Maximum Persistency via Iterative Relaxed Inference with Graphical Models

We consider the NP-hard problem of MAP-inference for undirected discrete graphical models. We propose a polynomial time and practically efficient algorithm for finding a part of its optimal solution. Specifically, our algorithm marks some labels of the considered graphical model either as (i) optimal, meaning that they belong to all optimal solutions of the inference problem; (ii) non-optimal if they provably do not belong to any solution. With access to an exact solver of a linear programming relaxation to the MAP-inference problem, our algorithm marks the maximal possible (in a specified sense) number of labels. We also present a version of the algorithm, which has access to a suboptimal dual solver only and still can ensure the (non-)optimality for the marked labels, although the overall number of the marked labels may decrease. We propose an efficient implementation, which runs in time comparable to a single run of a suboptimal dual solver. Our method is well-scalable and shows state-of-the-art results on computational benchmarks from machine learning and computer vision.

==> edit/diff_preamble.tex <==
\RequirePackage[normalem,normalbf]{ulem} %highlight changes
\newcommand\xoutpars[1]{\let\helpcmd\xout\parhelp#1\par\relax\relax}
\newcommand\soutpars[1]{\let\helpcmd\sout\parhelp#1\par\relax\relax}
\long\def\parhelp#1\par#2\relax{%
  \helpcmd{#1}\ifx\relax#2\else\par\parhelp#2\relax\fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{endnotes}
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE

\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFaddtex}[1]{{\protect\color{blue}{#1}}} %DIF PREAMBLE
\providecommand{\DIFdeltex}[1]{}                      %DIF PREAMBLE
%\providecommand{\DIFdeltex}[1]{{\protect\color{red}{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{\relax} %DIF PREAMBLE
\providecommand{\DIFaddend}{\relax} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{\relax} %DIF PREAMBLE
\providecommand{\DIFdelend}{\relax} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF HYPERREF PREAMBLE %DIF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
%\providecommand{\DIFdel}[1]{} %DIF PREAMBLE
%
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
%\RequirePackage[normalem]{ulem} %DIF PREAMBLE
%\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
%\providecommand{\DIFaddtex}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
%\providecommand{\DIFdeltex}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%%DIF SAFE PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
%\providecommand{\DIFaddend}{} %DIF PREAMBLE
%\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
%\providecommand{\DIFdelend}{} %DIF PREAMBLE
%%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
%\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
%\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
%\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
%\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
%\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%%DIF HYPERREF PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
%\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

==> style/diff_preamble.tex <==
\RequirePackage[normalem,normalbf]{ulem} %highlight changes
\newcommand\xoutpars[1]{\let\helpcmd\xout\parhelp#1\par\relax\relax}
\newcommand\soutpars[1]{\let\helpcmd\sout\parhelp#1\par\relax\relax}
\long\def\parhelp#1\par#2\relax{%
  \helpcmd{#1}\ifx\relax#2\else\par\parhelp#2\relax\fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{endnotes}
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE

\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFaddtex}[1]{{\protect\color{blue}{#1}}} %DIF PREAMBLE
%\providecommand{\DIFdeltex}[1]{}                      %DIF PREAMBLE
\providecommand{\DIFdeltex}[1]{{\protect\color{red}{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{\relax} %DIF PREAMBLE
\providecommand{\DIFaddend}{\relax} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{\relax} %DIF PREAMBLE
\providecommand{\DIFdelend}{\relax} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\def\DIFaddFL#1{\protect\DIFadd{#1}} %DIF PREAMBLE
\def\DIFdelFL#1{\protect\DIFdel{#1}} %DIF PREAMBLE
%
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF HYPERREF PREAMBLE %DIF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
%\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{} %DIF PREAMBLE
%
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
%\RequirePackage[normalem]{ulem} %DIF PREAMBLE
%\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
%\providecommand{\DIFaddtex}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
%\providecommand{\DIFdeltex}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%%DIF SAFE PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
%\providecommand{\DIFaddend}{} %DIF PREAMBLE
%\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
%\providecommand{\DIFdelend}{} %DIF PREAMBLE
%%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
%\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
%\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
%\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
%\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
%\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%%DIF HYPERREF PREAMBLE %DIF PREAMBLE
%\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
%\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
%%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

==> tcbbreakable.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbbreakable.code.tex: Code for breakable colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\let\tcb@parboxrestore@true=\tcb@parboxrestore
\let\tcb@parboxrestore@false\tcb@parbox@false@settings

% total height for boxes smaller than 0.4375\maxdimen and 0.4375\maxdimen else (ca 2.5m)
\def\tcb@defToTotalHeightBreakable#1#2{%
  \ifnum\ht#2<0 %
    \edef#1{7168pt}%
  \else\ifnum\ht#2<469762048 %
    \tcbdimto#1{\ht#2+\dp#2}%
  \else%
    \edef#1{7168pt}%
  \fi\fi%
}

\newbox\tcb@testbox

% for oversized boxes height is detected as \textheight or larger
\def\tcb@defToTotalHeightUnlimited#1#2{%
  \tcb@defToTotalHeightBreakable#1#2%
  \ifdim\dimexpr#1<\textheight\relax%
    \edef\tcb@thevfuzz{\the\vfuzz}%
    \edef\tcb@thevbadness{\the\vbadness}%
    \vfuzz=\maxdimen\vbadness=10000%
    \splittopskip=0pt%
    \splitmaxdepth=0pt%
    \savingvdiscards=1%
    \setbox\tcb@testbox=\vsplit#2 to \textheight%
    \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
    \ifdim\wd#2=0pt\relax%
      \tcb@swap{#2}{\tcb@testbox}%
      \tcbdimto#1{\ht#2+\dp#2}%
    \else%
      \setbox#2=\vbox{%
        \unvbox\tcb@testbox%
        \splitdiscards%
        \unvbox#2}%
      \edef#1{7168pt}%
    \fi%
    \savingvdiscards=0%
  \fi%
}


\def\tcb@vbox#1#2{%
  \edef\reserved@a{%
    \endgroup%
    \setbox#1\vbox{\hsize=#2%
      \begingroup\aftergroup}%
      \def\noexpand\@currenvir{\@currenvir}%
      \def\noexpand\@currenvline{\on@line}}%
  \reserved@a%
  \@endpefalse%
  \color@begingroup%
  \textwidth\hsize%
  \columnwidth\hsize%
  \csname tcb@parboxrestore@\kvtcb@parbox\endcsname%
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@%
  \let\@footnotetext\@mpfootnotetext%
  \let\@listdepth\@mplistdepth \@mplistdepth\z@%
  \@setminipage\tcb@hyph@fix%
  \let\tcb@drawcolorbox\tcb@drawcolorbox@standalone%
  \let\FN@pp@footnote\@empty% disable perpage mode of 'footmisc' package
  \ignorespaces%
}

\def\endtcb@vbox{%
  \par%
  \unskip%
  \ifvoid\@mpfootins\else%
    \vskip\skip\@mpfootins%
    \normalcolor%
    \footnoterule%
    \unvbox\@mpfootins%
  \fi%
  \@minipagefalse%
  \color@endgroup}

% remaining height
\def\tcb@comp@h@page{%
  \tcb@breakat@next%
  \ifdim\tcb@breakat@dim>0pt\relax%
    \tcbdimto\tcb@h@page{\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \else%
    \ifx\kvtcb@float\@empty%
      \iftcb@multicol%
        \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
      \else%
        \ifdim\pagegoal=16383.99998pt
          \tcbdimto\tcb@h@page{\vsize-\kvtcb@shrinkbreakgoal}% detects floating objects
        \else%
          \tcb@comp@compress%
          \tcbdimto\tcb@h@page{\pagegoal-\pagetotal+\tcb@compress@height-\kvtcb@shrinkbreakgoal}%
        \fi%
      \fi%
    \else%
      \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
    \fi%
  \fi%
}

\def\tcb@comp@h@total@standalone{%
  \tcbdimto\tcb@h@padding{\kvtcb@bbtop@stand+\kvtcb@bbbottom@stand+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@stand+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@total{\tcb@h@padding+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
}


\newif\iftcb@final@box

\def\tcb@check@for@final@box{%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \iftcb@multicol%
      \tcb@final@boxfalse%
    \else%
      \ifdim\tcb@h@total>\dimexpr\tcb@h@page+\kvtcb@enlargepage@flex\relax%
        \tcb@final@boxfalse%
      \else%
        \tcbdimto\tcb@temp{\tcb@h@total-\tcb@h@page}%
        \enlargethispage*{\tcb@temp}%
        \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@temp}%
        \tcb@final@boxtrue%
      \fi%
    \fi%
  \else%
    \tcb@final@boxtrue%
  \fi%
}

\def\tcb@following@title{%
  \ifx\kvtcb@followingtitle\@empty%
    \tcb@hasTitlefalse%
    \let\tcb@h@title=\tcb@zpt%
    \let\tcb@h@padtitle=\tcb@zpt%
  \else%
    \tcb@hasTitletrue%
    \tcbdimto\tcb@w@title{\tcb@innerwidth-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@followingtitle\end{tcb@savebox}%
    \tcbdimto\tcb@h@title{\ht\tcb@titlebox+\dp\tcb@titlebox}%
    \tcbdimto\tcb@h@padtitle{\kvtcb@title@rule+\kvtcb@boxsep*2+\kvtcb@toptitle+\kvtcb@bottomtitle+\tcb@h@title}%
  \fi%
}

\newbox\tcb@totalupperbox
\newbox\tcb@totallowerbox
\newif\iftcb@break@allowed

\def\tcb@enlbreak@next@final{%
  \ifdim\dimexpr\tcb@enlbreak@dim=0pt\relax
  \else%
    \iftcb@multicol\else\enlargethispage{\tcb@enlbreak@dim}\fi%
  \fi%
}

\def\tcb@enlbreak@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@enlbreak@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@enlbreak@next=\tcb@enlbreak@next@final%
  \else%
     \edef\tcb@enlbreak@seq{\temp@a @}%
  \fi%
  \tcb@enlbreak@next@final%
}

\def\tcb@enlbreak@next@step{%
  \edef\tcb@temp{\noexpand\tcb@enlbreak@next@scan\tcb@enlbreak@seq}%
  \tcb@temp%
}

\def\tcb@enlbreak@init{%
  \edef\tcb@enlbreak@seq{\kvtcb@enlargepage/@}%
  \let\tcb@enlbreak@next=\tcb@enlbreak@next@step%
  \tcb@enlbreak@next%
}


\def\tcb@breakat@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@breakat@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@breakat@next=\@empty%
  \else%
     \edef\tcb@breakat@seq{\temp@a @}%
  \fi%
}

\def\tcb@breakat@next@step{%
  \edef\tcb@temp{\noexpand\tcb@breakat@next@scan\tcb@breakat@seq}%
  \tcb@temp%
}

\def\tcb@breakat@init{%
  \edef\tcb@breakat@seq{\kvtcb@breakatdim/@}%
  \let\tcb@breakat@next=\tcb@breakat@next@step%
}


\newif\iftcb@multicol
\newif\iftcb@vfillbeforefirst

\def\tcb@do@nobreak@warning{%
  \iftcb@ignorenobreak%
    \tcb@warning{Using nobreak failed. You should set `ignore nobreak=false' to avoid this}%
  \else%
    \tcb@warning{Using nobreak failed. Try to enlarge `lines before break' or set page breaks manually}%
  \fi%
}

\def\tcb@handle@nobreak{%
  \tcb@enlbreak@init%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  \tcbdimto\tcb@h@page{\tcb@h@page-1.5\baselineskip-\parskip-\lineskip}% security surcharge
  \tcb@comp@h@total@standalone%
  \tcb@check@for@final@box%
  \iftcb@final@box%
  \else%
    \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
      \tcbdimto\tcb@h@page{\tcb@h@page+3.5\baselineskip+\parskip+\lineskip}%
      \vspace{\tcb@h@page}%
      {\parskip\z@\nointerlineskip\noindent}%
      \vspace{-\tcb@h@page}%
      \par%
    \fi%
  \fi%
}

\def\tcb@prepare@break@operation{%
  \setcounter{tcbbreakpart}{0}%
  \let\tcb@nobreak@warning\@empty%
  \@ifundefined{columnbreak}{\tcb@multicolfalse}{%
    \ifnum\doublecol@number>\z@ %
      \tcb@multicoltrue%
    \else%
      \tcb@multicolfalse%
    \fi}%
  \ifx\kvtcb@float\@empty%
    \iftcb@nobreak{%
      \let\tcb@nobreak@warning\tcb@do@nobreak@warning%
      \iftcb@ignorenobreak%
        \kvtcb@beforebox%
      \else%
        \tcb@handle@nobreak%
      \fi%
    }{\kvtcb@beforebox}%
    \def\kvtcb@beforebox{\parskip\z@\nointerlineskip\noindent}%
    \noindent% applies parskip
    \vskip\lineskip{\parskip\z@\par\vskip\z@}\bgroup\@nobreakfalse\addpenalty\z@\egroup% force update vertical list
    \tcb@break@allowedtrue%
    \tcb@enlbreak@init%
  \else%
    \tcb@break@allowedfalse%
  \fi%
}

\def\tcb@height@fill@unbroken#1{%
  \tcb@prepare@break@operation%
  \tcb@breakat@init%
  \tcbset{compress page=#1}%
  \tcb@comp@h@page%
  \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand,after=\eject}%
}

\def\tcb@height@fill@unbroken@normal{\tcb@height@fill@unbroken{none}}
\def\tcb@height@fill@unbroken@compressed{\tcb@height@fill@unbroken{all}}

\def\tcb@use@after@lastbox{\bgroup\tcb@after@lastbox\egroup}

\def\tcb@drawcolorbox@breakable{%
  \tcb@prepare@break@operation%
  \global\let\tcb@after@lastbox=\kvtcb@afterbox%
  \let\kvtcb@afterbox=\@empty%
  \begingroup%
    \parskip\z@%
    \parindent\z@%
    \lineskip\z@%
    \topskip\z@%
    \tcb@split@start%
  \endgroup%
  \color{.}% hack for some special cases
  \ifx\kvtcb@float\@empty%
    \aftergroup\tcb@use@after@lastbox%
  \fi%
}

\def\tcb@split@start{%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  % height calculation
  \tcb@comp@h@total@standalone%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@drawcolorbox@standalone%
  \else%
    \iftcb@break@allowed%
      \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
        \iftcb@multicol\columnbreak\else\pagebreak\fi%
        \tcb@nobreak@warning%
        \tcb@enlbreak@init\tcb@break@allowedfalse%
        \tcb@comp@h@page%
        \tcb@check@for@final@box%
        \iftcb@final@box%
          \tcb@drawcolorbox@standalone%
        \else%
          \let\tcb@split@next=\tcb@split@first%
        \fi%
      \else%
        \let\tcb@split@next=\tcb@split@first%
      \fi%
    \else%
      \let\tcb@split@next=\tcb@split@first%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@setbox#1#2#3{%
  \setbox#1=\vbox{\unvbox#3}%
  \ifdim\dimexpr\ht#1+\dp#1>#2\relax%
    %\tcb@warning{Splitted box part too large by \the\dimexpr\ht#1+\dp#1-#2\relax}% switched off (99% useless/annoying)
    \setbox#1=\vbox to\the\dimexpr#2-\dp#1\relax{\unvbox#1}%
  \fi%
}


\def\tcb@setbox@upper#1#2{%
  \tcb@setbox\tcb@upperbox{#1}{#2}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}


\def\tcb@split@upper@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \setbox\tcb@totalupperbox=\vbox{%
      \unvbox\tcb@upperbox%
      \splitdiscards%
      \unvbox\tcb@totalupperbox}%
  \else%
    \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@upper@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \tcb@warning{The upper box part has become overfull}%
  \fi%
  \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@setbox@lower#1#2{%
  \tcb@setbox\tcb@lowerbox{#1}{#2}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
}

\def\tcb@split@lower@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \setbox\tcb@totallowerbox=\vbox{%
      \unvbox\tcb@lowerbox%
      \splitdiscards%
      \unvbox\tcb@totallowerbox}%
  \else%
    \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@lower@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \tcb@warning{The lower box part has become overfull}%
  \fi%
  \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@split@setstate@first{%
  \edef\tcb@split@state{first}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@stand%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@stand%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\tcb@zpt%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@middle{%
  \edef\tcb@split@state{middle}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@last{%
  \edef\tcb@split@state{last}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@stand%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@stand%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\tcb@zpt%
}


\def\tcb@split@force@standalone{%
  \tcb@comp@h@total@standalone%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcb@h@page-\tcb@h@total}%
  \fi%
}


\def\tcb@split@break@to@start{%
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
  \iftcb@multicol\columnbreak\else\pagebreak\fi%
  \tcb@nobreak@warning%
  \tcb@enlbreak@init\tcb@break@allowedfalse%
  \let\tcb@split@next=\tcb@split@start%
}

\def\tcb@split@first{%
  \setcounter{tcbbreakpart}{1}%
  \ifx\kvtcb@float\@empty%
    \iftcb@vfillbeforefirst%
      \let\tcb@before@first=\vfill%
    \else%
    \let\tcb@before@first=\@empty%
    \fi%
    \let\tcb@before@middle=\@empty%
    \let\tcb@before@last=\@empty%
    \iftcb@multicol%
      \long\def\tcb@after@first{\par}% using \columnbreak here kills multicols' algortihm sometimes
      \long\def\tcb@after@middle{\par\vfill}%
    \else%
      \long\def\tcb@after@first{\par\pagebreak\tcb@enlbreak@next}%
      \long\def\tcb@after@middle{\par\vfill\eject\tcb@enlbreak@next}%
    \fi%
    \let\tcb@after@last=\par%
  \else%
    \edef\tcb@before@first{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]\noexpand\kvtcb@everyfloat}%
    \let\tcb@before@middle=\tcb@before@first%
    \let\tcb@before@last=\tcb@before@first%
    \let\tcb@after@first=\tcb@float@env@end%
    \let\tcb@after@middle=\tcb@float@env@end%
    \let\tcb@after@last=\tcb@float@env@end%
  \fi%
  %
  \edef\kvtcb@skin@@first{\kvtcb@skin@first}%
  \edef\kvtcb@skin@@middle{\kvtcb@skin@middle}%
  \edef\kvtcb@skin@@last{\kvtcb@skin@last}%
  %
  \let\tcb@h@breaksep@first=\kvtcb@bottomsep%
  \tcbdimto\tcb@h@breaksep@middle{\kvtcb@bottomsep+\kvtcb@topsep}%
  \let\tcb@h@breaksep@last=\kvtcb@topsep%
  \tcbdimto\tcb@h@padding@first{\kvtcb@bbtop@stand+\kvtcb@bbbottom@break+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@break+\tcb@h@breaksep@first+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@middle{\kvtcb@bbtop@break+\kvtcb@bbbottom@break+\kvtcb@top@rule@break+\kvtcb@bottom@rule@break+\tcb@h@breaksep@middle+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@last{\kvtcb@bbtop@break+\kvtcb@bbbottom@stand+\kvtcb@top@rule@break+\kvtcb@bottom@rule@stand+\tcb@h@breaksep@last+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  %
  \tcb@split@setstate@first%
  %
  \splittopskip=0pt%
  \splitmaxdepth=0pt%
  \edef\tcb@thevfuzz{\the\vfuzz}%
  \edef\tcb@thevbadness{\the\vbadness}%
  %
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  %
  \let\tcb@split@next=\relax%
  \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@first-\tcb@h@padtitle}%
  \ifdim\tcb@split@dim<\tcb@h@upper\relax%
    %
    %
    \iftcb@break@allowed%
      \tcb@split@upper@box@and@assemble%
      \ifnum\tcb@upper@box@badness=1000000\relax%
        \tcb@split@break@to@start%
      \else%
        \ifdim\wd\tcb@totalupperbox=0pt\relax%
          \iftcb@lowerspace%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \fi%
        \else%
          \ifdim\dimexpr\tcb@h@upper=0pt\relax%
            \tcb@split@break@to@start%
          \else%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@USL%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@standalone%
          \tcb@drawcolorbox@standalone%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \fi%
  \else%
    \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
    \iftcb@lowerspace%
      \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}%
      \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@SL%
      \else
        \tcb@split@lower@box@and@assemble%
        \ifnum\tcb@lower@box@badness=1000000\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \ifdim\wd\tcb@totallowerbox=0pt\relax%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \else%
            \tcb@sdraw@USL%
            \let\tcb@split@next=\tcb@split@L%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@force@standalone%
      \tcb@drawcolorbox@standalone%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@force@last{%
  \tcb@split@setstate@last%
  \ifdim\tcb@h@total>\tcb@h@page%
    \tcbdimto\kvtcb@bbbottom{\kvtcb@bbbottom+\tcb@h@page-\tcb@h@total}%
  \fi%
}

\def\tcb@nextbreakpart{%
  \stepcounter{tcbbreakpart}%
  \tcb@count@boxes%
  \iftcb@checkpage%
    \tcb@phantom@savepage%
    \tcb@hasPhantomtrue%
    \sbox\tcb@phantombox{\kvtcb@phantom}%
    \let\kvtcb@phantom\@empty%
  \fi%
  \tcb@following@title%
}


\def\tcb@split@USL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \tcb@defToTotalHeight\tcb@h@upper{\tcb@totalupperbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
    \iftcb@lowerspace%
      \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
      \tcb@sdraw@USL%
    \else
      \tcb@sdraw@U%
    \fi%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \ifdim\tcb@split@dim<\tcb@h@upper\relax%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@last%
          \tcb@sdraw@U%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \else%
      \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
      \iftcb@lowerspace%
        \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}
        \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else
          \tcb@split@lower@box@and@assemble%
          \ifnum\tcb@lower@box@badness=1000000\relax%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \ifdim\wd\tcb@totallowerbox=0pt\relax%
              \tcb@split@force@last%
              \tcb@sdraw@USL%
            \else%
              \tcb@sdraw@USL%
              \let\tcb@split@next=\tcb@split@L%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@split@force@last%
        \tcb@sdraw@U%
      \fi%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@SL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last-\kvtcb@top-\kvtcb@boxsep+\tcb@h@padtitle+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@SL%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle+\kvtcb@top+\kvtcb@boxsep-\tcb@h@padtitle-\tcb@h@segment}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@SL%
    \else
      \tcb@sdraw@SL%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@L{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@L%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@L%
    \else
      \tcb@sdraw@L%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@break@ch@fixed{%
  \ifdim\tcb@natheight<\tcb@h@page\relax%
    \tcbdimto\kvtcb@height@fixed{\tcb@h@page-\kvtcb@bbtop-\kvtcb@bbbottom}%
    \tcb@ch@fixed%
  \else%
    \tcb@ch@natural%
  \fi%
}


\def\tcb@sdraw@USL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
     % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@U{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{0}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@SL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@bottom+\kvtcb@boxsep+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@L{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{2}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\ht\tcb@lowerbox+\dp\tcb@lowerbox+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}



\tcbset{%
  breakable@true/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable@unlimited/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightUnlimited%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable/.style={breakable@#1},
  breakable/.default=true,%
  unbreakable/.style={breakable=false},%
  enforce breakable/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  title after break/.store in=\kvtcb@followingtitle,%
  notitle after break/.style={title after break=},%
  adjusted title after break/.style={title after break={#1\vphantom{\kvtcb@adjusttext}}},%
  lines before break/.store in=\kvtcb@breakminlines,%
  shrink break goal/.store in=\kvtcb@shrinkbreakgoal,%
  toprule at break/.store in=\kvtcb@top@rule@break,
  bottomrule at break/.store in=\kvtcb@bottom@rule@break,
  topsep at break/.store in=\kvtcb@topsep,%
  bottomsep at break/.store in=\kvtcb@bottomsep,%
  pad before break/.code={\let\kvtcb@bottom@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@bottomsep{#1-\kvtcb@bottom-\kvtcb@boxsep}},%
  pad before break*/.style={pad before break={#1},%
    code={\tcbdimto\tcb@temp{\kvtcb@bottom@rule@stand-\kvtcb@bottomsep}%
      \ifdim\tcb@temp>0pt\relax%
        \tcbdimto\kvtcb@enlargepage@flex{\kvtcb@enlargepage@flex+\tcb@temp}\fi}},%
  pad after break/.code={\let\kvtcb@top@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@topsep{#1-\kvtcb@top-\kvtcb@boxsep}},%
  pad at break/.style={pad before break={#1},pad after break={#1}},%
  pad at break*/.style={pad before break*={#1},pad after break={#1}},%
  enlargepage/.store in=\kvtcb@enlargepage,%
  enlargepage flexible/.store in=\kvtcb@enlargepage@flex,%
  break at/.store in=\kvtcb@breakatdim,%
  height fixed for/.is choice,%
  height fixed for/none/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/first/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/first and middle/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle and last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/all/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  vfill before first/.is if=tcb@vfillbeforefirst,%
  height fill/true/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@normal},%
  height fill/maximum/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@compressed},%
  height fill/.default=true,%
  compress page/.is choice,%
  compress page/all/.code={\def\tcb@comp@compress{\def\tcb@compress@height{\pageshrink-1sp}}},%
  compress page/none/.code={\def\tcb@comp@compress{\let\tcb@compress@height\tcb@zpt}},%
  compress page/baselineskip/.code={\def\tcb@comp@compress{%
    \ifdim\pageshrink>\baselineskip%
      \let\tcb@compress@height\baselineskip%
    \else%
      \def\tcb@compress@height{\pageshrink-1sp}%
    \fi}},%
  compress page/.default=all,%
  compress page=baselineskip,% global setting
  extras unbroken/.code={\appto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first/.code={\appto\tcb@extras@first{\tcbset{#1}}},%
  extras middle/.code={\appto\tcb@extras@middle{\tcbset{#1}}},%
  extras last/.code={\appto\tcb@extras@last{\tcbset{#1}}},%
  extras/.style={extras unbroken={#1},extras first={#1},extras middle={#1},extras last={#1}},%
  extras broken/.style={extras first={#1},extras middle={#1},extras last={#1}},%
  extras unbroken and first/.style={extras unbroken={#1},extras first={#1}},%
  extras unbroken and last/.style={extras unbroken={#1},extras last={#1}},%
  extras middle and last/.style={extras middle={#1},extras last={#1}},%
  extras first and middle/.style={extras first={#1},extras middle={#1}},%
  no extras unbroken/.code={\let\tcb@extras@unbroken\@empty},%
  no extras first/.code={\let\tcb@extras@first\@empty},%
  no extras middle/.code={\let\tcb@extras@middle\@empty},%
  no extras last/.code={\let\tcb@extras@last\@empty},%
  no extras/.code={\let\tcb@extras@unbroken\@empty\let\tcb@extras@first\@empty\let\tcb@extras@middle\@empty\let\tcb@extras@last\@empty},%
  if odd page*/.style 2 args={check odd page,extras={if odd page={#1}{#2}}},%
}


\tcbset{%
  reset@breakable/.style={%
    unbreakable,notitle after break,
    shrink break goal=0pt,
    lines before break=2,
    topsep at break=0pt,
    bottomsep at break=0pt,
    enlargepage=0pt,enlargepage flexible=0pt,
    break at=0pt,
    height fixed for=none,
    vfill before first=false,
    no extras,
  },
  initialize@reset=reset@breakable,
}


==> tcbdocumentation.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbdocumentation.code.tex: Code for LaTeX documentations
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{listings,skins,xparse,external}

\RequirePackage{pifont}[2005/04/12]
\RequirePackage{marvosym}[2011/07/20]
\ifdefined\printindex\else\RequirePackage{makeidx}[2000/03/29]\fi
\RequirePackage{refcount}[2011/10/16]
\RequirePackage{hyperref}[2012/02/06]
\ifdefined\marginnote\else\RequirePackage{marginnote}[2012/03/29]\fi

\definecolor{Option}{rgb}{0.118,0.546,0.222}
\definecolor{Definition}{rgb}{0.784,0.06,0.176}
\definecolor{ExampleFrame}{rgb}{0.628,0.705,0.942}
\definecolor{ExampleBack}{rgb}{0.963,0.971,0.994}
\definecolor{Hyperlink}{rgb}{0.281,0.275,0.485}

\def\colDef#1{\textcolor{\kvtcb@col@command}{#1}}
\def\colOpt#1{\textcolor{\kvtcb@col@opt}{#1}}

\lstdefinestyle{tcbdocumentation}{language={[LaTeX]TeX},
    aboveskip={0\p@ \@plus 6\p@},
    belowskip={0\p@ \@plus 6\p@},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    prebreak={\Righttorque},
    postbreak={\space\Lefttorque},
    breakatwhitespace=true,
    basicstyle=\ttfamily\footnotesize,
    extendedchars=true,
    moredelim={[is][\itshape\rmfamily]{^^a7}{^^a7}},
    nolol,inputencoding=\kvtcb@listingencoding}

% The following macros are taken from ltxdoc
\DeclareRobustCommand\cs[1]{\texttt{\char`\\#1}}
\def\meta@font@select{\rmfamily\itshape}

\AtEndPreamble{%
  \@ifpackageloaded{doc}{%
  }{% code taken from doc.sty
    \ifx\l@nohyphenation\undefined
      \newlanguage\l@nohyphenation
    \fi
    \DeclareRobustCommand\meta[1]{%
         \ensuremath\langle
         \ifmmode \expandafter \nfss@text \fi
         {%
          \meta@font@select
          \edef\meta@hyphen@restore
            {\hyphenchar\the\font\the\hyphenchar\font}%
          \hyphenchar\font\m@ne
          \language\l@nohyphenation
          #1\/%
          \meta@hyphen@restore
         }\ensuremath\rangle
    }%
  }%
}%

\def\marg#1{%
  {\ttfamily\char`\{}\meta{#1}{\ttfamily\char`\}}}
\def\oarg#1{%
  \colOpt{{\ttfamily[}\meta{#1}{\ttfamily]}}}

\newrobustcmd\tcb@cs[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\char`\\\scantokens{#1}\unskip}}
\newrobustcmd\tcb@scantokens[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\scantokens{#1}\unskip}}

\newif\iftcb@doc@toindex
\newif\iftcb@doc@colorize
\newif\iftcb@doc@annotate

% language specific texts
\tcbset{
  doclang/.cd,
  color/.store in=\kvtcb@text@color,
  colors/.store in=\kvtcb@text@colors,
  counter/.store in=\kvtcb@text@counter,
  counters/.store in=\kvtcb@text@counters,
  environment content/.store in=\kvtcb@text@envcontent,
  environment/.store in=\kvtcb@text@env,
  environments/.store in=\kvtcb@text@envs,
  index/.store in=\kvtcb@text@index,
  key/.store in=\kvtcb@text@key,
  keys/.store in=\kvtcb@text@keys,
  length/.store in=\kvtcb@text@length,
  lengths/.store in=\kvtcb@text@lengths,
  new/.store in=\kvtcb@text@new,
  pageshort/.store in=\kvtcb@text@pageshort,
  updated/.store in=\kvtcb@text@updated,
  value/.store in=\kvtcb@text@value,
  values/.store in=\kvtcb@text@values,
}

% documentation options
\tcbset{
  documentation listing options/.store in=\kvtcb@doclistingoptions,%
  documentation listing style/.style={documentation listing options={style=#1}},%
  documentation minted style/.store in=\kvtcb@docmintstyle,
  documentation minted options/.store in=\kvtcb@docmintoptions,
  color command/.store in=\kvtcb@col@command,
  color environment/.store in=\kvtcb@col@environment,
  color key/.store in=\kvtcb@col@key,
  color value/.store in=\kvtcb@col@value,
  color counter/.store in=\kvtcb@col@counter,
  color length/.store in=\kvtcb@col@length,
  color color/.store in=\kvtcb@col@color,
  color definition/.style={color command={#1},color environment={#1},color key={#1},
    color value={#1},color color={#1},color counter={#1},color length={#1}},
  color option/.store in=\kvtcb@col@opt,
  color hyperlink/.store in=\kvtcb@colhyper,
  color frame/.store in=\kvtcb@colhyper,
  index actual/.store in=\idx@actual,
  index quote/.store in=\idx@quote,
  index level/.store in=\idx@level,
  index format/.store in=\idx@format,
  index colorize/.is if=tcb@doc@colorize,%
  index annotate/.is if=tcb@doc@annotate,%
  index command/.code={\def\kvtcb@index@command##1{#1{##1}}},%
  index command name/.code={\def\kvtcb@index@command##1{\index[#1]{##1}}},%
  doc left/.dimstore in=\kvtcb@doc@left,
  doc right/.dimstore in=\kvtcb@doc@right,
  doc left indent/.dimstore in=\kvtcb@doc@indentleft,
  doc right indent/.dimstore in=\kvtcb@doc@indentright,
  doc head command/.style={doc@head@command/.style={#1}},
  doc head environment/.style={doc@head@environment/.style={#1}},
  doc head key/.style={doc@head@key/.style={#1}},
  doc head/.style={doc head command={#1},doc head environment={#1},doc head key={#1}},
  before doc body command/.store in=\kvtcb@doc@body@command@before,
  after doc body command/.store in=\kvtcb@doc@body@command@after,
  before doc body environment/.store in=\kvtcb@doc@body@environment@before,
  after doc body environment/.store in=\kvtcb@doc@body@environment@after,
  before doc body key/.store in=\kvtcb@doc@body@key@before,
  after doc body key/.store in=\kvtcb@doc@body@key@after,
  before doc body/.style={before doc body command={#1},before doc body environment={#1},before doc body key={#1}},
  after doc body/.style={after doc body command={#1},after doc body environment={#1},after doc body key={#1}},
  doc description/.store in=\kvtcb@doc@description,%
  doc into index/.is if=tcb@doc@toindex,%
  doc updated/.style={before upper={\tcbdocmarginnote{\tcbdocupdated{#1}}}},
  doc new/.style={before upper={\tcbdocmarginnote{\tcbdocnew{#1}}}},
  doc new and updated/.style 2 args={before upper={\tcbdocmarginnote{\tcbdocnew{#1}\\\tcbdocupdated{#2}}}},
  doc marginnote/.style={doc@marginnote/.style={#1}},
}


% styles
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize},
  documentation minted style=,
  documentation minted options={tabsize=2,fontsize=\small},
  index default settings/.style={index actual={@},index quote={"},index level={!}},
  index german settings/.style={index actual={=},index quote={!},index level={>}},
  english language/.code={\tcbset{doclang/.cd,
    color=color,colors=Colors,
    counter=counter,counters=Counters,
    environment content=environment content,
    environment=environment,environments=Environments,
    index=Index,
    key=key,keys=Keys,
    length=length,lengths=Lengths,
    new=New,
    pageshort={P.},
    updated=Updated,
    value=value,values=Values}},
}

\AtBeginDocument{%
  \csname tcb@doc@index@\idx@format\endcsname%
  \hypersetup{
  citecolor=\kvtcb@colhyper,
  linkcolor=\kvtcb@colhyper,
  urlcolor=\kvtcb@colhyper,
  filecolor=\kvtcb@colhyper,
  menucolor=\kvtcb@colhyper
}}

\def\dispExample{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispExample{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \tcblower%
  \tcbusetemp%
  \end{tcolorbox}%
}

\newenvironment{dispExample*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispExample}

\def\dispListing{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispListing{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \end{tcolorbox}%
}

\newenvironment{dispListing*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispListing}

% index auxiliary macros
\def\tcb@Index@Print@CA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@C#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
}

\def\tcb@Index@Print@ComCA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@ComC#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
}

\newrobustcmd{\tcbIndexPrintComC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@command}}
\def\tcb@Print@Com#1{\textcolor{\kvtcb@col@command}{\bfseries\tcb@cs{#1}}}

\newrobustcmd{\tcbIndexPrintEnvCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@environment}{\kvtcb@text@env}}
\newrobustcmd{\tcbIndexPrintEnvC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@environment}}
\def\tcb@Print@Env#1{\textcolor{\kvtcb@col@environment}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintKeyCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@key}{\kvtcb@text@key}}
\newrobustcmd{\tcbIndexPrintKeyC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@key}}
\def\tcb@Print@Key#1{\textcolor{\kvtcb@col@key}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintValCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@value}{\kvtcb@text@value}}
\newrobustcmd{\tcbIndexPrintValC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@value}}
\def\tcb@Print@Val#1{\textcolor{\kvtcb@col@value}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintColCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@color}{\kvtcb@text@color}}
\newrobustcmd{\tcbIndexPrintColC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@color}}
\def\tcb@Print@Col#1{\textcolor{\kvtcb@col@color}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintCountCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@counter}{\kvtcb@text@counter}}
\newrobustcmd{\tcbIndexPrintCountC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@counter}}
\def\tcb@Print@Count#1{\textcolor{\kvtcb@col@counter}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintLenCA}[1]{\tcb@Index@Print@ComCA{#1}{\kvtcb@col@length}{\kvtcb@text@length}}
\newrobustcmd{\tcbIndexPrintLenC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@length}}
\def\tcb@Print@Len#1{\textcolor{\kvtcb@col@length}{\bfseries\tcb@cs{#1}}}

\def\tcb@index@Com#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintComC{#1}}\fi}
\def\tcb@index@Env#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintEnvCA{#1}}\kvtcb@index@command{\kvtcb@text@envs\idx@level#1\idx@actual\tcbIndexPrintEnvC{#1}}\fi}
\def\tcb@index@Key#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintKeyCA{#1}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{#1}}\fi}%
\def\tcb@index@KeyPath#1#2{\iftcb@doc@toindex\kvtcb@index@command{#2\idx@actual\tcbIndexPrintKeyCA{#2}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{/#1/}\idx@level#2\idx@actual\tcbIndexPrintKeyC{#2}}\fi}%
\def\tcb@index@Val#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintValCA{#1}}\kvtcb@index@command{\kvtcb@text@values\idx@level#1\idx@actual\tcbIndexPrintValC{#1}}\fi}
\def\tcb@index@Col#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintColCA{#1}}\kvtcb@index@command{\kvtcb@text@colors\idx@level#1\idx@actual\tcbIndexPrintColC{#1}}\fi}
\def\tcb@index@Count#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintCountCA{#1}}\kvtcb@index@command{\kvtcb@text@counters\idx@level#1\idx@actual\tcbIndexPrintCountC{#1}}\fi}
\def\tcb@index@Len#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintLenCA{#1}}\kvtcb@index@command{\kvtcb@text@lengths\idx@level#1\idx@actual\tcbIndexPrintLenC{#1}}\fi}

\def\brackets#1{{\ttfamily\char`\{}#1{\ttfamily\char`\}}}

\newenvironment{tcb@manual@entry}{\begin{list}{}{%
  \setlength{\leftmargin}{\kvtcb@doc@left}%
  \setlength{\itemindent}{0pt}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parsep}{0pt}%
  \setlength{\rightmargin}{\kvtcb@doc@right}%
  }\item}{\end{list}}

\def\tcb@manual@top#1{\itemsep=0pt\parskip=0pt\item\strut{#1}\par\topsep=0pt}

\def\tcb@doc@do@description{%
  \ifx\kvtcb@doc@description\@empty\else\tcblower\raggedleft(\kvtcb@doc@description)\fi%
}

\newtcolorbox{tcb@doc@head}[1]{blank,colback=white,colframe=white,
  code={\tcbdimto\tcb@temp@grow@left{-\kvtcb@doc@indentleft}%
        \tcbdimto\tcb@temp@grow@right{-\kvtcb@doc@indentright}},
  grow to left by=\tcb@temp@grow@left,%
  grow to right by=\tcb@temp@grow@right,
  sidebyside,sidebyside align=top,
  sidebyside gap=-\tcb@w@upper@real,
  phantom=\phantomsection,%
  enlarge bottom by=-0.2\baselineskip,#1}

% main documentation environments
\newenvironment{docCommand}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@command}%
  \tcb@Print@Com{#2}\tcb@index@Com{#2}\protected@edef\@currentlabel{\noexpand\tcb@cs{#2}}\label{com:#2}{\ttfamily #3}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@command@before}%
  {\kvtcb@doc@body@command@after\end{tcb@manual@entry}}

\newenvironment{docCommand*}{\bgroup\tcb@doc@toindexfalse\begin{docCommand}}{\end{docCommand}\egroup}

\newenvironment{docEnvironment}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@environment}%
  \strut\cs{begin}\brackets{\tcb@Print@Env{#2}}\tcb@index@Env{#2}\protected@edef\@currentlabel{#2}\label{env:#2}{\ttfamily #3}\par%
  \strut~~\meta{\kvtcb@text@envcontent}\par%
  \strut\cs{end}\brackets{\tcb@Print@Env{#2}}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@environment@before}%
  {\kvtcb@doc@body@environment@after\end{tcb@manual@entry}}

\newenvironment{docEnvironment*}{\bgroup\tcb@doc@toindexfalse\begin{docEnvironment}}{\end{docEnvironment}\egroup}

\NewDocumentEnvironment{docKey}{ O{} +O{} m m +m }{\tcbset{#2,doc description={#5}}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@key}%
  \ifblank{#1}{%
    \tcb@Print@Key{#3}\tcb@index@Key{#3}\protected@edef\@currentlabel{#3}\label{key:#3}{\ttfamily #4}%
  }{%
    \tcb@Print@Key{/#1/#3}%
    \tcb@index@KeyPath{#1}{#3}\protected@edef\@currentlabel{/#1/#3}\label{key:/#1/#3}{\ttfamily #4}%
  }%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@key@before}%
  {\kvtcb@doc@body@key@after\end{tcb@manual@entry}}

\newenvironment{docKey*}{\bgroup\tcb@doc@toindexfalse\begin{docKey}}{\end{docKey}\egroup}

\def\tcbmakedocSubKey#1#2{%
  \NewDocumentEnvironment{#1}{ O{} +O{} m m +m }{%
    \ifblank{##1}{\def\tcb@key@path{#2}}{\def\tcb@key@path{#2/##1}}%
    \begin{docKey}[\tcb@key@path][##2]{##3}{##4}{##5}}%
      {\end{docKey}}%
  \newenvironment{#1*}{\bgroup\tcb@doc@toindexfalse\begin{#1}}{\end{#1}\egroup}%
}

\DeclareDocumentCommand\docAuxCommand{sm}{%
  \tcb@Print@Com{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Com{#2}}%
}

\DeclareDocumentCommand\docAuxEnvironment{sm}{%
  \tcb@Print@Env{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Env{#2}}%
}

\DeclareDocumentCommand\docAuxKey{sO{}m}{%
  \ifblank{#2}{%
    \tcb@Print@Key{#3}%
    \IfBooleanTF{#1}{}{\tcb@index@Key{#3}}%
  }{%
    \tcb@Print@Key{/#2/#3}%
    \IfBooleanTF{#1}{}{\tcb@index@KeyPath{#2}{#3}}%
}}

\DeclareDocumentCommand\docColor{sm}{%
  \tcb@Print@Col{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Col{#2}}%
}

\DeclareDocumentCommand\docCounter{sm}{%
  \tcb@Print@Count{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Count{#2}}%
}

\DeclareDocumentCommand\docLength{sm}{%
  \tcb@Print@Len{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Len{#2}}%
}

\DeclareDocumentCommand\docValue{sm}{%
  \tcb@Print@Val{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Val{#2}}%
}

\setrefcountdefault{-1}
\DeclareDocumentCommand\tcb@ref@doc{msm}{%
  \hyperref[#1:#3]{\texttt{\ref*{#1:#3}}%
  \IfBooleanTF{#2}{}{%
    \ifnum\getpagerefnumber{#1:#3}=\thepage%
    \else%
      \textsuperscript{\ding{213}\,\kvtcb@text@pageshort\,\pageref*{#1:#3}}%
    \fi}}%
}

\def\refCom{\tcb@ref@doc{com}}
\def\refEnv{\tcb@ref@doc{env}}
\def\refKey{\tcb@ref@doc{key}}

\def\refAux#1{\textcolor{\kvtcb@colhyper}{\tcb@scantokens{#1}}}
\def\refAuxcs#1{\textcolor{\kvtcb@colhyper}{\tcb@cs{#1}}}

\newenvironment{absquote}
               {\list{}{\leftmargin2cm\rightmargin\leftmargin}%
                \item\relax\footnotesize}
               {\endlist}

\newcommand{\tcbdocmarginnote}[2][]{%
  \marginnote{%
  \begin{tcolorbox}[enhanced jigsaw,size=fbox,boxrule=1pt,leftrule=0pt,rightrule=0pt,
    arc=0pt,outer arc=1pt,boxsep=1pt,top=1pt,bottom=1pt,
    nobeforeafter,width=\marginparwidth,
    colframe=red!50!white,colback=red!25!yellow!5!white,fontupper=\scriptsize,before upper=\flushright,
    doc@marginnote,#1]#2\end{tcolorbox}}}

\newcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}
\newcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}

%--- index macros taken from pgfmanual-en-macros
\def\tcb@doc@index@pgf@{%
  \ifdefined\c@IndexColumns%
    \c@IndexColumns=2%
  \fi%
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
    \parindent -30pt%
    \columnsep 15pt%
    \parskip 0pt plus 1pt%
    \leftskip 30pt%
    \rightskip 0pt plus 2cm%
    \small%
    \def\@idxitem{\par}%
    \let\item\@idxitem\ignorespaces}
  \def\endtheindex{\onecolumn}%
  \def\noindexing{\let\index=\@gobble}%
}

\def\tcb@doc@index@pgfsection{%
  \def\index@prologue{\section*{\kvtcb@text@index}\addcontentsline{toc}{section}{\kvtcb@text@index}%
    \par\noindent%
  }%
  \tcb@doc@index@pgf@%
}

\def\tcb@doc@index@pgfchapter{%
  \def\index@prologue{\ifdefined\phantomsection\phantomsection\fi\@makeschapterhead{\kvtcb@text@index}\addcontentsline{toc}{chapter}{\kvtcb@text@index}}%
  \tcb@doc@index@pgf@%
}

\let\tcb@doc@index@pgf=\tcb@doc@index@pgfsection%

\def\tcb@doc@index@doc{%
  \let\tcb@index@Com=\SpecialMainIndex%%
  \let\tcb@index@Env=\SpecialMainEnvIndex%
  \tcbset{index german settings}%
  \EnableCrossrefs%
  \PageIndex%
}

\def\tcb@doc@index@off{}%

\tcbset{%
  reset@documentation/.style={%
    index command=\index,%
    index format=pgf,
    english language,
    documentation listing style=tcbdocumentation,
    index default settings,
    color option=Option,
    color definition=Definition,
    color hyperlink=Hyperlink,
    doc left=2em,
    doc right=0pt,
    doc left indent=-2em,
    doc right indent=0pt,
    doc head=,
    before doc body=,
    after doc body=,
    doc description=,
    doc into index=true,
    index colorize=false,
    index annotate=true,
    doc marginnote=,
    },
  initialize@reset=reset@documentation,
}

% deprecated
\tcbset{
  before example/.store in=\kvtcb@beforeexample,
  after example/.store in=\kvtcb@afterexample,
    before example=\par\smallskip,
    after example=,
}


==> tcbexternal.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbexternal.code.tex: Code for externalization
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

{
\catcode`\"=12
\xdef\tcbexternal@normal@dq{"}
\catcode`\"=13
\gdef\tcbexternal@activate@normal@dq{\let"=\tcbexternal@normal@dq}
}

\long\def\tcbifexternal#1#2{%
  \ifdefined\TCBEXTERNALINPUT%
    #1%
  \else%
    #2%
  \fi%
}

\tcbifexternal{%
  \def\tcbEXTERNALIZE{%
    \RequirePackage{incgraph}%
    \TCBEXTERNALPREAMBLE%
    \begin{document}%
    \begin{inctext}[border=\TCBEXTERNALSAFETY]%
    \input{\TCBEXTERNALINPUT}%
    \end{inctext}%
    \end{document}%
  }%
}{%
  \def\tcbEXTERNALIZE{%
    \tcbset{
      external/.cd,
      externalize/.is if=tcb@externalize,
      externalize=true,
    }%
  }%
}

\@onlypreamble\tcbEXTERNALIZE

\def\tcbexternal@setbasename#1{%
  \edef\tcbexternal@job@name{\expandonce{\tcbexternal@prefix}\expandonce{#1}}%
  \edef\tcbexternal@job@mdfive{\expandonce{\tcbexternal@job@name.md5}}%
  \edef\tcbexternal@job@source{\expandonce{\tcbexternal@job@name.tex}}%
  \edef\tcbexternal@job@pdf{\expandonce{\tcbexternal@job@name.pdf}}%
}

\def\tcbexternal@corecompile{%
  \begingroup%
  \ifnum\the\catcode`\"=13 \tcbexternal@activate@normal@dq\fi%
  \message{=== Compile external '\tcbexternal@job@name': }%
  \immediate\openout\tcb@out="\tcbexternal@run@tex"
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALINPUT{"\tcbexternal@job@source"}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALSAFETY{\tcbexternal@safety}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALPREAMBLE{\expandonce{\tcbexternal@preamble}}}%
  \ifdefempty{\tcbexternal@preclass}{}{\immediate\write\tcb@out{\expandonce{\tcbexternal@preclass}}}%
  \immediate\write\tcb@out{\string\input{"\jobname.tex"}}%
  \immediate\closeout\tcb@out%
  \foreach \n in {1,...,\tcbexternal@runs}
  {%
    \immediate\write18{%
      \tcbexternal@compiler\space
      -shell-escape
      -halt-on-error
      -interaction=batchmode
      -jobname="\tcbexternal@job@name"
      "\tcbexternal@run@tex"
    }%
  }%
  \endgroup%
}

\def\tcbexternal@inputsource{%
  \IfFileExists{\tcbexternal@job@source}%
    {\input{\tcbexternal@job@source}}%
    {\tcb@error{File '\tcbexternal@job@source' missing.}{}}%
}

\def\tcbexternal@pdfmissing@warning{%
  \tcb@warning{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}%
  \message{Load '\tcbexternal@job@source' instead}%
  \tcbexternal@inputsource%
}

\def\tcbexternal@pdfmissing@error{%
  \tcb@error{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}{}%
}

\def\tcbexternal@inputpdf{%
  \IfFileExists{\tcbexternal@job@pdf}%
    {%
      \begingroup\edef\x{\endgroup%
        \noexpand\includegraphics[trim=\tcbexternal@safety\space\tcbexternal@safety%
        \space\tcbexternal@safety\space\tcbexternal@safety]{\expandonce{\tcbexternal@job@pdf}}}%
      \x%
    }%
    {\tcbexternal@pdfmissing}%
}

\newif\iftcb@externalize
\tcb@externalizefalse

\def\tcbexternal@generatemdivesum{%
  \iftcb@externalize%
    \def\tcbexternallastmdfivesum{}%
    \IfFileExists{\tcbexternal@job@mdfive}{\input{\tcbexternal@job@mdfive}}{}%
    \edef\tcbexternalmdfivesum{\pdfmdfivesum file {\tcbexternal@job@source}}%
  \else%
    \def\tcbexternallastmdfivesum{x}%
    \edef\tcbexternalmdfivesum{}%
  \fi%
  \immediate\openout\tcb@out=\tcbexternal@job@mdfive%
  \immediate\write\tcb@out{\string\def\string\tcbexternallastmdfivesum{\tcbexternalmdfivesum}\@percentchar}%
  \immediate\closeout\tcb@out%
}

\def\tcbexternal@conditionalcompile{%
  \IfFileExists{\tcbexternal@job@pdf}{%
    \ifdefstrequal{\tcbexternallastmdfivesum}{\tcbexternalmdfivesum}{%
    }{%
      \tcbexternal@corecompile%
    }%
  }{%
    \tcbexternal@corecompile%
  }%
}

\def\tcb@useexternal{%
  \tcbexternal@generatemdivesum%
  \iftcb@externalize%
    \tcbexternal@compile%
    \tcbexternal@inputpdf%
  \else%
    \tcbexternal@inputsource%
  \fi%
}

\newenvironment{tcbexternal}[2][]{%
  \tcbset{external/.cd,#1,name=#2}%
  \@ifundefined{@tcbexternal@JN@\tcbexternal@job@name}{%
      \global\@namedef{@tcbexternal@JN@\tcbexternal@job@name}{}%
    }{%
      \tcb@error{External job name '\tcbexternal@job@name' already used}%
        {Give a new unique name to the current external job.}%
    }%
  \begingroup%
  \let\tcb@verbatim@begin@hook=\tcbexternal@out@begin%
  \let\tcb@verbatim@end@hook=\tcbexternal@out@end%
  \tcbverbatimwrite{\tcbexternal@job@source}}%
{%
  \endtcbverbatimwrite\endgroup%
  \tcb@useexternal%
}

\long\def\new@tcb@externalizeenvironment#1#2#3#4#5{%
  \tcb@newenvironment{#1}[2][]{%
    #4%
    \begingroup%
    \tcbexternal[#3,##1,environment=#2]{##2}%
  }{%
    \endtcbexternal%
    \endgroup%
    #5%
  }%
}

\def\newtcbexternalizeenvironment{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizeenvironment%
}

\def\renewtcbexternalizeenvironment{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizeenvironment%
}

\long\def\new@tcb@externalizetcolorbox#1#2#3#4{%
  \new@tcb@externalizeenvironment{#1}{#2}%
    {preamble tcbset={force nobeforeafter},#3}%
    {\tcb@layer@pushup\tcb@apply@box@options{#4}\tcb@set@normal@unbroken@beforeafter\tcb@before@unbroken}%
    {\tcb@after@unbroken}%
}

\def\newtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizetcolorbox%
}

\def\renewtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizetcolorbox%
}


\newtcbexternalizeenvironment{extikzpicture}{tikzpicture}{}{}{}

\newtcbexternalizetcolorbox{extcolorbox}{tcolorbox}{}{}


\tcbset{
  external/.cd,
  %
  runner/.code={%
    \edef\tcbexternal@run@tex{\expandonce{#1}}%
  },
  %
  prefix/.store in=\tcbexternal@prefix,
  compiler/.store in=\tcbexternal@compiler,
  runs/.code={\numdef\tcbexternal@runs{#1}},
  name/.code={\tcbexternal@setbasename{#1}},
  safety/.store in=\tcbexternal@safety,
  preamble/.code={\appto\tcbexternal@preamble{#1}},
  preamble tcbset/.code={\appto\tcbexternal@preamble{\tcbset{#1}}},
  clear preamble/.code={\def\tcbexternal@preamble{}},
  preclass/.code={\appto\tcbexternal@preclass{#1}},
  clear preclass/.code={\def\tcbexternal@preclass{}},
  PassOptionsToPackage/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToPackage{#1}{#2}}},
  PassOptionsToClass/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToClass{#1}{#2}}},
  externalize/.code={},
  -/.style={externalize=false},
  %
  force remake/.is choice,
  force remake/true/.code={\let\tcbexternal@compile=\tcbexternal@corecompile},
  force remake/false/.code={\let\tcbexternal@compile=\tcbexternal@conditionalcompile},
  force remake/.default=true,
  !/.style=force remake,
  %
  input source on error/.is choice,
  input source on error/true/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@warning},
  input source on error/false/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@error},
  input source on error/.default=true,
  %
  plain/.code={%
    \let\tcbexternal@out@begin=\@empty%
    \let\tcbexternal@out@end=\@empty%
  },
  minipage/.code={%
    \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{minipage}{\the\dimexpr#1\relax}\string\ignorespaces\@percentchar}}%
    \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{minipage}\@percentchar}}%
  },
  minipage/.default=\linewidth,
  %
  environment with percent/.is choice,
  environment with percent/true/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}\@percentchar}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}\@percentchar}}%
    }
  },
  environment with percent/false/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}}}%
    }
  },
  environment with percent/.default=true,
  %
  runner=\jobname_run.tex,
  prefix={external/},
  compiler=pdflatex,
  runs=1,
  name=unnamed,
  safety=2mm,
  clear preamble,
  clear preclass,
  force remake=false,
  input source on error,
  environment with percent,
  plain
}

\tcbset{%
  externalize example/.style={%
    external/name=#1,tempfile=\tcbexternal@job@source,
    code={\let\tcbusetemp=\tcb@useexternal}%
  },
  externalize example!/.style={externalize example=#1,external/force remake},
  externalize listing/.style={%
    external/name=#1,listing file=\tcbexternal@job@source,
    code={\let\tcbuselistingtext@input=\tcb@useexternal}%
  },
  externalize listing!/.style={externalize listing=#1,external/force remake},
}


==> tcbfitting.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbfitting.code.tex: Code for fit boxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\newdimen\tcbfitdim
\newdimen\tcb@lowerfitdim
\newdimen\tcb@upperfitdim
\newif\iftcb@continue

\tcbset{%
  fit/.style={capture=fitbox},%
  fit to/.style args={#1 and #2}{capture=fitbox,width=#1,height=#2},%
  fit to height/.style={capture=fitbox,height=#1},%
  fit basedim/.code={\def\kvtcb@fit@basedim{#1}\tcbfitdim\kvtcb@fit@basedim},%
  fit skip/.store in=\kvtcb@fit@skip,%
  fit fontsize macros/.code={%
    \renewcommand\tiny{\tcb@setfontsize\tiny{0.5}}%
    \renewcommand\scriptsize{\tcb@setfontsize\scriptsize{0.7}}%
    \renewcommand\footnotesize{\tcb@setfontsize\footnotesize{0.8}}%
    \renewcommand\small{\tcb@setfontsize\small{0.9}}%
    \renewcommand\normalsize{\tcb@setfontsize\normalsize{1}}%
    \renewcommand\large{\tcb@setfontsize\large{1.2}}%
    \renewcommand\Large{\tcb@setfontsize\Large{1.44}}%
    \renewcommand\LARGE{\tcb@setfontsize\LARGE{1.728}}%
    \renewcommand\huge{\tcb@setfontsize\huge{2.0736}}%
    \renewcommand\Huge{\tcb@setfontsize\Huge{2.48832}}},%
  fit height plus/.style={fit,height plus=#1},%
  fit width plus/.dimstore in=\kvtcb@fit@plus@width,%
  fit height from/.style args={#1 to #2}{fit,height from={#1} to {#2}},
  fit width from/.style args={#1 to #2}{fit,width={#1},fit width plus={#2-#1}},
  fit maxstep/.store in=\kvtcb@fit@maxstep,%
  fit maxfontdiff/.store in=\kvtcb@fit@maxfontdiff,%
  fit maxfontdiffgap/.store in=\kvtcb@fit@maxfontdiffgap,%
  fit maxwidthdiff/.store in=\kvtcb@fit@maxwidthdiff,%
  fit maxwidthdiffgap/.store in=\kvtcb@fit@maxwidthdiffgap,%
  fit warning/.is choice,
  fit warning/on/.code={\let\tcb@fit@warn@begin=\@empty%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/off/.code={\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/final/.code={\tcb@cur@hbadness=\hbadness\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \def\tcb@fit@warn@end{\hbadness=\tcb@cur@hbadness\relax\tcb@fit@@box}},
  fit algorithm/.is choice,
  fit algorithm/fontsize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize},
  fit algorithm/fontsize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize@star},
  fit algorithm/areasize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize},
  fit algorithm/areasize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize@star},
  fit algorithm/hybrid/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid},
  fit algorithm/hybrid*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid@star},
  fit algorithm/squeeze/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@squeeze},
  spartan@fit/.style={fit algorithm=squeeze},
}

\def\tcb@@capture@fitbox{%
  \let\endtcolorbox=\relax%
  \Collect@Body\tcbox@inner@fitbox@collected%
}

\def\tcbfontsize#1{\fontsize{#1\tcbfitdim}{#1\dimexpr\kvtcb@fit@skip\tcbfitdim}\selectfont}

\def\tcb@setfontsize#1#2{\@setfontsize#1{#2\tcbfitdim}{#2\dimexpr\kvtcb@fit@skip\tcbfitdim}}

\long\def\tcbox@inner@fitbox@collected#1{%
  \tcbox@inner@fitbox{#1}%
  \tcb@finalize@environment%
}

\newcount\tcb@cur@hbadness

\def\tcbox@fitalgorithm@fontsize{%
  \tcb@continuetrue%
  \loop%
    \tcbfitdim.5\tcbfitdim%
    \tcb@fit@@box%
    \ifnum\count@=\kvtcb@fit@maxstep\relax%
      \tcb@continuefalse%
    \else%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \ifdim\tcbfitdim<18000sp\relax%
          \count@\kvtcb@fit@maxstep\relax%
          \tcb@continuefalse%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
    \fi%
  \iftcb@continue \repeat%
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
    \tcb@lowerfitdim\tcbfitdim%
    \tcb@upperfitdim2\tcbfitdim%
    \tcbfitdim1.5\tcbfitdim%
    \loop%
      \tcb@fit@@box%
      \tcb@continuetrue%
      \ifnum\count@<\kvtcb@fit@maxstep\relax%
        \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiff\relax%
          \tcb@continuefalse%
        \else%
          \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiffgap\relax%
            \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
              \tcb@continuefalse%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
      \iftcb@continue%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcb@upperfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@lowerfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \else%
          \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
          \tcb@lowerfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@upperfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \fi%
      \else%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcbfitdim\tcb@lowerfitdim%
          \tcb@fit@@box%
        \fi%
      \fi%
    \iftcb@continue \repeat%
  \fi%
}

\def\tcbox@fitalgorithm@fontsize@star{%
  \tcbox@fitalgorithm@fontsize%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@core{%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathsqrt{\pgfmathresult}%
  \let\tcb@temp=\pgfmathresult%
  \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper}%
  \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathdivide{\pgfmathresult}{\tcb@temp}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.98pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \else\ifdim\dimexpr\pgfmathresult pt>1.02pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \fi\fi%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize{%
  \tcbox@fitalgorithm@areasize@core%
  \pgfmathdivide{\tcb@w@upper}{\tcb@w@upper@temp}%
  \tcbdimto\tcb@fit@@h{\pgfmathresult\dimexpr\tcb@fit@@h}%
  \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \let\tcb@fit@@h=\tcb@fit@@target%
  \fi
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@h}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@star{%
  \tcbox@fitalgorithm@areasize@core%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@squeeze{%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@hybrid@core{%
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \tcbfitdim=\pgfmathresult\tcbfitdim%
  \tcb@fit@@box%
  %
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.85pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \else\ifdim\dimexpr\pgfmathresult pt>1.15pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \fi\fi%
}

\def\tcbox@fitalgorithm@hybrid{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize%
}

\def\tcbox@fitalgorithm@hybrid@star{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize@star%
}

\def\tcb@fit@@box{%
  \iftcb@hasTitle%
    \tcbdimto\tcb@w@title{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@title\kvtcb@title\kvtcb@after@title\end{tcb@savebox}%
    \tcbdimto\tcb@h@titletotal{\ht\tcb@titlebox+\dp\tcb@titlebox+\kvtcb@title@rule+(\kvtcb@boxsep)*2+\kvtcb@toptitle+\kvtcb@bottomtitle}%
  \else%
    \let\tcb@h@titletotal=\tcb@zpt%
  \fi%
  \tcbdimto\tcb@fit@@line{\kvtcb@fit@skip\tcbfitdim}%
  \tcbdimto\tcb@w@upper{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@leftupper)-(\kvtcb@rightupper)}%
  \tcb@fit@@boxsave{\tcb@w@upper}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@fit@@target{\kvtcb@height@fixed-(\kvtcb@top@rule@stand)-(\kvtcb@bottom@rule@stand)-(\kvtcb@top)-(\kvtcb@bottom)-(\kvtcb@boxsep)*2-\tcb@h@titletotal}%
}%

\long\def\tcbox@inner@fitbox#1{%
  \tcbset{breakable@false,sidebyside=false}%
  \let\tcb@val@raisebase=\tcb@zpt%
  \unless\ifdefined\kvtcb@height@fixed%
    \tcbset{height=\kvtcb@width}%
  \fi%
  \tcb@hasLowerfalse%
  %
  \count@\z@%
  \tcbfitdim\kvtcb@fit@basedim%
  \tcb@fit@warn@begin%
  %
  \def\tcb@fit@@boxsave##1{%
    \tcbdimto\tcb@innerwidth{\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
    \colorlet{tcbcol@origin}{.}%
    \tcb@set@color{tcbcol@upper}%
    \begin{tcb@savebox}{\tcb@upperbox}{##1}%
      \kvtcb@fontupper\fontsize{\tcbfitdim}{\tcb@fit@@line}\selectfont%
%      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\unskip\kvtcb@after@upper%
      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\kvtcb@after@upper%
    \end{tcb@savebox}%
    \tcb@reset@color%
    \advance\count@ 1\relax%
  }%
  %
  \tcb@set@@phantom%
  \tcb@set@@title%
  \tcb@fit@@box%
  %
  % height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \let\tcb@fit@@minheight=\kvtcb@height@fixed%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
      \ifdim\dimexpr\tcb@fit@@h>\dimexpr\tcb@fit@@target+\kvtcb@height@fixed@plus\relax%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\kvtcb@height@fixed@plus}%
        \tcbdimto\tcb@fit@@target{\tcb@fit@@target+\kvtcb@height@fixed@plus}%
      \else%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
        \let\tcb@fit@@target=\tcb@fit@@h%
      \fi%
    \fi%
  \fi%
  %
  % width fit
  \ifdim\kvtcb@fit@plus@width>0pt\relax%
    \ifnum\count@<\kvtcb@fit@maxstep\relax%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
        \tcb@upperfitdim\dimexpr\kvtcb@width+\kvtcb@fit@plus@width\relax%
        \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
        \tcb@fit@@box%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \else%
          \ifnum\count@<\kvtcb@fit@maxstep\relax%
            \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
            \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
            \loop%
              \tcb@fit@@box%
              \tcb@continuetrue%
              \ifnum\count@<\kvtcb@fit@maxstep\relax%
                \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiff\relax%
                  \tcb@continuefalse%
                \else%
                  \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiffgap\relax%
                    \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
                      \tcb@continuefalse%
                    \fi%
                  \fi%
                \fi%
              \else%
                \tcb@continuefalse%
              \fi%
              \iftcb@continue%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \else%
                  \tcb@upperfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \fi%
              \else%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
                  \tcb@fit@@box%
                \fi%
              \fi%
            \iftcb@continue \repeat%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  %
  % (font) fit
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \tcbox@fitalgorithm%
    \fi%
  \fi%
  %
  \tcb@fit@warn@end%
  %
  % last height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \ifdim\dimexpr\tcb@fit@@h<\tcb@fit@@target\relax%
      \tcbdimto\tcb@temp{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
      \ifdim\dimexpr\tcb@temp<\tcb@fit@@minheight\relax%
      \else%
        \let\kvtcb@height@fixed=\tcb@temp%
      \fi%
    \fi%
  \fi%
  %
  \edef\tcbfitsteps{\the\count@}%
  \tcb@set@@dimensions%
  \tcb@draw@color@box%
}

\newcommand{\tcboxfit}[2][]{%
  \tcb@ox{capture=fitbox,#1}{#2}%
}

\long\def\tcb@newtcboxfit#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcboxfit[#2,options@for=#1]}}

\long\def\tcb@newtcboxfit@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcboxfit[#3,options@for=#1]}}

\long\def\tcb@newtcboxfit@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcboxfit[#4,options@for=#1]}}

\long\def\tcb@new@tcboxfit@#1[#2]{%
  \@ifnextchar[{\tcb@newtcboxfit@@{#1}[#2]}{\tcb@newtcboxfit@{#1}[#2]}}

\long\def\tcb@new@tcboxfit#1{%
  \@ifnextchar[{\tcb@new@tcboxfit@{#1}}{\tcb@newtcboxfit{#1}}}

\def\newtcboxfit{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\def\renewtcboxfit{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\tcbset{%
  reset@fitting/.style={%
    fit algorithm=fontsize,%
    fit basedim=10pt,fit skip=1.2,
    height plus=0pt,fit width plus=0pt,
    fit maxstep=20,fit maxfontdiff=0.1pt,fit maxfontdiffgap=1pt,
    fit maxwidthdiff=1pt,fit maxwidthdiffgap=10pt,
    fit warning=off
  },
  initialize@reset=reset@fitting,
}



==> tcbhooks.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbhooks.code.tex: Code for adding hooks
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\tcbset{%
  before upper app/.code={\appto\kvtcb@before@upper{#1}},%
  before upper pre/.code={\preto\kvtcb@before@upper{#1}},%
  after upper app/.code={\appto\kvtcb@after@upper{#1}},%
  after upper pre/.code={\preto\kvtcb@after@upper{#1}},%
  before lower app/.code={\appto\kvtcb@before@lower{#1}},%
  before lower pre/.code={\preto\kvtcb@before@lower{#1}},%
  after lower app/.code={\appto\kvtcb@after@lower{#1}},%
  after lower pre/.code={\preto\kvtcb@after@lower{#1}},%
  before title app/.code={\appto\kvtcb@before@title{#1}},%
  before title pre/.code={\preto\kvtcb@before@title{#1}},%
  after title app/.code={\appto\kvtcb@after@title{#1}},%
  after title pre/.code={\preto\kvtcb@after@title{#1}},%
  %
  % usable inside the document or in the preamble after setting before / after
  before app/.code={\appto\kvtcb@beforebox{#1}},%
  before pre/.code={\preto\kvtcb@beforebox{#1}},%
  after app/.code={\appto\kvtcb@afterbox{#1}},%
  after pre/.code={\preto\kvtcb@afterbox{#1}},%
  %
  overlay unbroken app/.code={\appto\tcb@overlay@unbroken{#1}},%
  overlay unbroken pre/.code={\preto\tcb@overlay@unbroken{#1}},%
  overlay first app/.code={\appto\tcb@overlay@first{#1}},%
  overlay first pre/.code={\preto\tcb@overlay@first{#1}},%
  overlay middle app/.code={\appto\tcb@overlay@middle{#1}},%
  overlay middle pre/.code={\preto\tcb@overlay@middle{#1}},%
  overlay last app/.code={\appto\tcb@overlay@last{#1}},%
  overlay last pre/.code={\preto\tcb@overlay@last{#1}},%
  %
  overlay app/.style={overlay unbroken app={#1},overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay pre/.style={overlay unbroken pre={#1},overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay broken app/.style={overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay broken pre/.style={overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay unbroken and first app/.style={overlay unbroken app={#1},overlay first app={#1}},%
  overlay unbroken and first pre/.style={overlay unbroken pre={#1},overlay first pre={#1}},%
  overlay unbroken and last app/.style={overlay unbroken app={#1},overlay last app={#1}},%
  overlay unbroken and last pre/.style={overlay unbroken pre={#1},overlay last pre={#1}},%
  overlay middle and last app/.style={overlay middle app={#1},overlay last app={#1}},%
  overlay middle and last pre/.style={overlay middle pre={#1},overlay last pre={#1}},%
  overlay first and middle app/.style={overlay first app={#1},overlay middle app={#1}},%
  overlay first and middle pre/.style={overlay first pre={#1},overlay middle pre={#1}},%
  %
  % skins:
  frame code app/.code={\appto\tcb@frame@code{#1}},%
  frame code pre/.code={\preto\tcb@frame@code{#1}},%
  interior titled code app/.code={\appto\tcb@interiortitled@code{#1}},%
  interior titled code pre/.code={\preto\tcb@interiortitled@code{#1}},%
  interior code app/.code={\appto\tcb@interior@code{#1}},%
  interior code pre/.code={\preto\tcb@interior@code{#1}},%
  segmentation code app/.code={\appto\tcb@segmentation@code{#1}},%
  segmentation code pre/.code={\preto\tcb@segmentation@code{#1}},%
  title code app/.code={\appto\tcb@title@code{#1}},%
  title code pre/.code={\preto\tcb@title@code{#1}},%
  %
  extras unbroken pre/.code={\preto\tcb@extras@unbroken{#1}},%
  extras first pre/.code={\preto\tcb@extras@first{#1}},%
  extras middle pre/.code={\preto\tcb@extras@middle{#1}},%
  extras last pre/.code={\preto\tcb@extras@last{#1}},%
  extras pre/.style={extras unbroken pre={#1},extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras broken pre/.style={extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras unbroken and first pre/.style={extras unbroken pre={#1},extras first pre={#1}},%
  extras unbroken and last pre/.style={extras unbroken pre={#1},extras last pre={#1}},%
  extras middle and last pre/.style={extras middle pre={#1},extras last pre={#1}},%
  extras first and middle pre/.style={extras first pre={#1},extras middle pre={#1}},%
  %
  underlay unbroken pre/.code={\preto\tcb@underlay@unbroken{#1}},%
  underlay first pre/.code={\preto\tcb@underlay@first{#1}},%
  underlay middle pre/.code={\preto\tcb@underlay@middle{#1}},%
  underlay last pre/.code={\preto\tcb@underlay@last{#1}},%
  underlay boxed title pre/.code={\preto\tcb@underlay@boxedtitle{#1}},%
  underlay pre/.style={underlay unbroken pre={#1},underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay broken pre/.style={underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay unbroken and first pre/.style={underlay unbroken pre={#1},underlay first pre={#1}},%
  underlay unbroken and last pre/.style={underlay unbroken pre={#1},underlay last pre={#1}},%
  underlay middle and last pre/.style={underlay middle pre={#1},underlay last pre={#1}},%
  underlay first and middle pre/.style={underlay first pre={#1},underlay middle pre={#1}},%
  finish unbroken pre/.code={\preto\tcb@finish@unbroken{#1}},%
  finish first pre/.code={\preto\tcb@finish@first{#1}},%
  finish middle pre/.code={\preto\tcb@finish@middle{#1}},%
  finish last pre/.code={\preto\tcb@finish@last{#1}},%
  finish pre/.style={finish unbroken pre={#1},finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish broken pre/.style={finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish unbroken and first pre/.style={finish unbroken pre={#1},finish first pre={#1}},%
  finish unbroken and last pre/.style={finish unbroken pre={#1},finish last pre={#1}},%
  finish middle and last pre/.style={finish middle pre={#1},finish last pre={#1}},%
  finish first and middle pre/.style={finish first pre={#1},finish middle pre={#1}},%
  %
  watermark tikz app/.style={overlay app={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz pre/.style={overlay pre={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark tikz pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics app/.style={overlay app={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics pre/.style={overlay pre={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@graphics{#2}}},
  watermark graphics pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text app/.style={overlay app={\tcb@drawspec@watermark@text{#1}}},
  watermark text pre/.style={overlay pre={\tcb@drawspec@watermark@text{#1}}},
  watermark text app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@text{#2}}},
  watermark text pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@text{#2}}},
}



==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
  every listing line/.code={%
    \def\lst@NewLine{%
      \ifx\lst@OutputBox\@gobble\else
          \par\noindent \hbox{}#1%
      \fi
      \global\advance\lst@newlines\m@ne
      \lst@newlinetrue}},%
  every listing line*/.style={every listing line={#1},%
    code={\setbox\z@=\hbox{#1}\tcbdimto\kvtcb@rightupper{\kvtcb@rightupper+\wd\z@}}},%
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{pdftexcmds}

\def\tcbuselistingtext@input{\input{\kvtcb@listingfile}}%
\def\tcbuselistingtext{\tcbuselistingtext@input}%
\def\tcbuselistingcomment{\kvtcb@listingcomment}%
\def\tcb@listing@listing{\tcbuselistinglisting}

\def\tcb@listing@listingAndOther{%
   \tcbuselistinglisting%
   \tcblower%
   \tcb@use@listing@other%
}

\def\tcb@listing@otherAndListing{%
   \tcb@use@listing@other%
   \tcblower%
   \tcbuselistinglisting%
}

\newenvironment{tcb@lower@outside}[1]{%
  \tcbset{savedelimiter=tcb@lower@outside}\tcb@minipage{#1}%
  \color{tcbcol@lower}\kvtcb@fontlower\kvtcb@halignlower\kvtcb@before@lower\ignorespaces}%
%  {\unskip\kvtcb@after@lower\endminipage}
  {\kvtcb@after@lower\endminipage}

\def\tcb@use@listing@other@reset{%
  \tcbset{every box on layer 1/.style={reset,every box}}%
  \tcb@use@listing@other}

\def\tcb@use@lower@outside#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@otherAboveListing{%
  {\kvtcb@beforebox}\noindent%
  \iftcb@lowervisible%
    \tcb@use@lower@outside{\kvtcb@width}%
    \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
  \fi%
  \begin{tcolorbox}[before=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@otherAboveListing@Decoupled{%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveOther{%
  \begin{tcolorbox}[after=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@use@lower@outside{\kvtcb@width}%
  \fi%
  {\kvtcb@afterbox}%
}

\def\tcb@inputlisting@out@listingAboveOther@Decoupled{%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
}


\newenvironment{tcb@outside@environment}{%
  \tcb@before@unbroken%
  \begin{minipage}{\tcb@width}}%
{%
  \end{minipage}%
  \tcb@after@unbroken}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \let\tcb@before@unbroken=\kvtcb@beforebox%
    \let\tcb@after@unbroken=\kvtcb@afterbox%
  \else%
    \edef\tcb@before@unbroken{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]}%
    \let\tcb@after@unbroken=\tcb@float@env@end%
  \fi%
}

\def\tcb@use@lower@outside@side#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcb@box@align\z@%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@listingAndOther{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \kern\kvtcb@sbs@gap%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
  \fi%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@out@otherAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside-\tcb@temp@wd+\kvtcb@sbs@gap}%
  \else%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside+\kvtcb@sbs@gap}%
  \fi%
  \kern\tcb@temp@wd%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture,savedelimiter=tcolorbox]\tcb@listing@process\end{tcolorbox}%
}

\long\def\tcb@run@system@command#1{%
  \ifcase\pdf@shellescape\relax
    \tcb@error{You must invoke LaTeX with the -shell-escape flag}{Pass the -shell-escape flag to LaTeX.}%
  \or\or
    \tcb@warning{System call with restricted shell escape may fail}%
  \fi%
  \filename@parse{\kvtcb@listingfile}\immediate\write18{#1}%
  \relax%
}


\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing@process@inside/.code 2 args={%
    \let\tcb@inputlisting\tcb@inputlisting@inside%
    \let\tcb@listing@process=#1%
    \let\tcb@use@listing@other=#2},%
  listing@process@outside/.code 2 args={%
    \let\tcb@inputlisting=#1%
    \let\tcb@use@listing@other=#2},%
  listing only/.style={listing@process@inside={\tcb@listing@listing}{\tcbuselistingtext}},%
  text only/.style={listing@process@inside={\tcbuselistingtext}{\tcbuselistingtext}},%
  comment only/.style={listing@process@inside={\tcbuselistingcomment}{\tcbuselistingcomment}},%
  listing and text/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingtext}},%
  text and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingtext}},%
  text above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingtext}},%
  text above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingtext}},%
  listing above text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingtext}},%
  listing above* text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingtext}},%
  text outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingtext}},%
  listing outside text/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingtext}},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  listing and comment/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingcomment}},%
  comment and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingcomment}},%
  comment above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingcomment}},%
  comment above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingcomment}},%
  listing above comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingcomment}},%
  listing above* comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingcomment}},%
  comment outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingcomment}},%
  listing outside comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingcomment}},%
  comment side listing/.style={sidebyside,comment and listing},%
  listing side comment/.style={sidebyside,listing and comment},%
  listing engine/.is choice,%
  image comment/.style 2 args={comment={\includegraphics[#1]{#2}}},%
  comment style/.store in=\kvtcb@commentstyle,%
  tcbimage comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\tcbincludegraphics[code={\pgfkeysalsofrom\tcb@trans@commentstyle}]{#1}}},
  pdf extension/.store in=\kvtcb@pdf@extension,%
  pdf comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\filename@parse{#1}\edef\tcb@trans@commentfile{\filename@area\filename@base.\kvtcb@pdf@extension}%
    \begin{tcbraster}[raster halign=center,sharp corners,size=tight,colback=white,code={\pgfkeysalsofrom\tcb@trans@commentstyle}]\tcbincludepdf{\tcb@trans@commentfile}\end{tcbraster}}},
  pdf comment/.default={\kvtcb@listingfile},
  process code/.code={\appto\tcb@listing@process@hook{#1}},%
  no process/.code={\def\tcb@listing@process@hook{}},%
  compilable listing/.style={listing file={\jobname-listing-\thetcblistingcount}},
  run system command/.style={process code={\tcb@run@system@command{#1}}},%
  run@system@command/.style 2 args={run system command={#1\space#2\space\filename@area\filename@base}},%
  run pdflatex/.style={run@system@command={pdflatex}{#1}},%
  run xelatex/.style={run@system@command={xelatex}{#1}},%
  run lualatex/.style={run@system@command={lualatex}{#1}},%
  run makeindex/.style={run@system@command={makeindex}{#1}},%
  run bibtex/.style={run@system@command={bibtex}{#1}},%
  run biber/.style={run@system@command={biber}{#1}},%
  run arara/.style={run@system@command={arara}{#1}},%
  run latex/.style={run@system@command={latex}{#1}},%
  run dvips/.style={run@system@command={dvips}{#1}},%
  run ps2pdf/.style={run system command={ps2pdf\space#1\space\filename@area\filename@base.ps}},%
}

\def\tcbinputlisting@core{%
  \tcb@listing@process@hook%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting%
}

\newcounter{tcblisting}

\newenvironment{tcblisting}[1]{%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcbinputlisting@core%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \tcbinputlisting@core%
  \endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}

\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\def\tcb@new@tcblisting#1{%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\def\tcb@new@tcbinputlisting#1{%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}

\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=, listing and text,
    no process,comment style=,pdf extension=pdf,
  },
  initialize@reset=reset@listingscore,
}



==> tcblistingsutf8.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistingsutf8.code.tex: Code for colorboxes with listings in UTF-8
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\RequirePackage{listingsutf8}[2011/11/10]
\tcbuselibrary{listings}

\tcbset{
  listing utf8/.style={listing inputencoding=utf8/#1},
}

\tcbset{%
  reset@listingsutf8/.style={listing utf8=latin1},
  initialize@reset=reset@listingsutf8,
}



==> tcbmagazine.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbmagazine.code.tex: Code for box sets and magazine styles
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{breakable}

\def\newboxarray#1{%
  \ifcsdef{tcb@boxarray@#1@allocated}{%
    \tcb@warning{box array '#1' is allocated again by \string\newboxarray. Memory and registers are wasted}%
  }{}%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \global\csdef{tcb@boxarray@#1@allocated}{0}%
}

\newboxarray{default}

\newrobustcmd*{\boxarraygetsize}[2][default]{%
  \letcs#2{tcb@boxarray@#1@size}%
  \ifdef{#2}{}{%
    \tcb@error{undefined box array '#1'}%
    {You have to say \string\newboxarray{#1}, before '#1' can be used as box array.}%
  }%
}

\newrobustcmd*{\boxarrayreset}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
}

\newrobustcmd*{\boxarrayclear}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \begingroup%
    \count@=0%
    \loop%
    \ifnum\count@<\tcb@box@array@allocated\relax%
      \advance\count@ 1\relax%
      \letcs\tcb@box@array@box{tcb@boxarray@#1@\number\count@ @box}%
      \setbox0=\box\tcb@box@array@box%
    \repeat%
  \endgroup%
}

\newrobustcmd*{\boxarraygetbox}[3][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \let#2\@undefined%
  \ifnum\numexpr#3>0\relax%
    \ifnum\numexpr#3>\tcb@box@array@size\relax%
    \else%
      \letcs#2{tcb@boxarray@#1@#3@box}%
    \fi%
  \fi%
}

\newrobustcmd*{\boxarraygetwidth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\wd\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetdepth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygettotalheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box+\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\useboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \usebox{\tcb@box@array@box}%
  \fi%
}

\newrobustcmd{\usetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\usebox{\tcb@box@array@box}}%
  \fi%
}

\newrobustcmd*{\consumeboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \leavevmode\box\tcb@box@array@box\relax%
  \fi%
}

\newrobustcmd{\consumetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\leavevmode\box\tcb@box@array@box\relax}%
  \fi%
}

\def\boxarraystore#1{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \numdef\tcb@box@array@size{\tcb@box@array@size+1}%
  \global\cslet{tcb@boxarray@#1@size}{\tcb@box@array@size}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \ifnum\tcb@box@array@allocated<\tcb@box@array@size\relax%
    \newbox\tcb@box@array@box\csxdef{tcb@boxarray@#1@\tcb@box@array@size @box}{\the\tcb@box@array@box}%
    \global\cslet{tcb@boxarray@#1@allocated}{\tcb@box@array@size}%
  \else%
    \letcs\tcb@box@array@box{tcb@boxarray@#1@\tcb@box@array@size @box}%
  \fi%
  \edef\reserved@a{%
    \endgroup
    \global\setbox\tcb@box@array@box\hbox{%
      \begingroup\aftergroup}%
        \def\noexpand\@currenvir{\@currenvir}%
        \def\noexpand\@currenvline{\on@line}}%
  \reserved@a
    \@endpefalse
    \color@setgroup
      \ignorespaces}

\def\endboxarraystore{\unskip\color@endgroup}

\def\tcb@storetoboxarray@begin#1#2[#3]{\begin{boxarraystore}{#1}}
\def\tcb@storetoboxarray@end{\end{boxarraystore}}

\tcbset{
  store to box array/.code={%
    \def\kvtcb@float{S}\def\tcb@float@env@begin{\tcb@storetoboxarray@begin{#1}}\def\tcb@float@env@end{\tcb@storetoboxarray@end}},
  store to box array/.default=default,
  reset box array/.code={\boxarrayreset[#1]},
  reset box array/.default=default,
  reset and store to box array/.style={reset box array={#1},store to box array={#1}},%
  reset and store to box array/.default=default,
  do not store to box array/.style={nofloat},
}



==> tcbminted.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbminted.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{minted}[2011/09/17]

\tcbuselibrary{listings@core}

\def\tcb@minted@input@listing#1#2#3#4{%
  \edef\temp@a{#4}%
  \ifx\temp@a\@empty%
  \else
    %\usemintedstyle{\temp@a}%
    \toks@=\expandafter{#4}%
    \edef\tcb@temp{\noexpand\usemintedstyle{\the\toks@}}%
    \tcb@temp%
  \fi%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\inputminted[\the\toks@]}%
  \tcb@temp{#2}{#3}%
}

\def\tcb@minted@uselistinglisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@listingfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@tempfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@doc@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@docmintoptions}{latex}{\kvtcb@tempfile}{\kvtcb@docmintstyle}%
}

\tcbset{%
  minted language/.store in=\kvtcb@minted@language,
  minted options/.store in=\kvtcb@minted@options,
  minted style/.store in=\kvtcb@minted@style,
  listing engine/minted/.code={\let\tcbuselistinglisting\tcb@minted@uselistinglisting%
    \let\tcbusetemplisting\tcb@minted@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@minted@doc@usetemplisting},
}


\tcbset{%
  reset@minted/.style={%
    minted language=latex,
    minted options={tabsize=2,fontsize=\small},
    minted style=,
    listing engine=minted,
  },
  initialize@reset=reset@minted,
}



==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@start\@empty%
    \let\tcb@raster@ehg@continue\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@row%
    \let\tcb@raster@ehg@continue\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@all%
    \let\tcb@raster@ehg@continue\@empty},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\kvtcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\kvtcb@raster@yskip\relax}\noindent\fi%
      \kern\kvtcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\kvtcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
        \aftergroup\tcb@raster@ehg@continue%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\kvtcb@raster@width+\kvtcb@raster@xskip-\kvtcb@raster@skip@left-\kvtcb@raster@skip@right)/\kvtcb@raster@columns-\kvtcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\kvtcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\kvtcb@raster@height+\kvtcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\kvtcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \tcb@raster@ehg@start%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\kvtcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
  \fi%
  \kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\kvtcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\kvtcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}


==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcb@segment@state=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcol@frame,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcol@back,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcol@backtitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcol@frame,bottom color=tcbcol@back,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcol@frame}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@backtitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcol@frame}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcol@backlower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}


\tikzset{beamer@color/.style={fill=none,top color=tcbcol@back,bottom color=tcbcol@back!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcb@segment@state
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}


\tcbset{%
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.store in=\kvtcb@style@boxedtitle,%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \colorlet{tcbtranscol@frame}{tcbcol@frame}%
      \colorlet{tcbtranscol@back}{tcbcol@backtitle}%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@boxedtitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[colframe=tcbtranscol@frame,colback=tcbtranscol@back,size=title,code={\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}}\endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}};
  }},
  fill plain picture/.style={path picture={%
    \tcb@set@waterbox@to@picture{#1}%
    \node at (path picture bounding box.center) {\box\tcb@waterbox};
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]{#1}};
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcol@frame,bottom color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  title style={left color=tcbcol@frame,right color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options]}%
      \tcb@temp{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}[underlay={%
        \begin{tcbclipinterior}%
        \edef\tcb@temp{\noexpand\tikzset{fill image options={\expandonce\kvtcb@graphics@options}}}%
        \tcb@temp%
        \path[fill zoom image={\imagepath}]
          ([xshift=\kvtcb@boxsep+\kvtcb@leftupper,yshift=\kvtcb@boxsep+\kvtcb@bottom]interior.south west) rectangle
          ([xshift=-\kvtcb@boxsep-\kvtcb@rightupper,yshift=-\kvtcb@boxsep-\kvtcb@top]interior.north east);
        \end{tcbclipinterior}%
        }]%
      \end{tcolorbox}%
    \else%
      \begin{tcolorbox}%
        \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth]}%
        \tcb@temp{\imagepath}%
      \end{tcolorbox}%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
}


\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcol@back!85!tcbcol@frame,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title style=,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1:#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5:##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,%
  },
  initialize@reset=reset@theorems,
}



==> tcbxparse.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbxparse.code.tex: Code for xparse features
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{xparse}[2013/12/31]

\tcbset{%
  IfNoValueTF/.code args={#1#2#3}{\IfNoValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfValueTF/.code args={#1#2#3}{\IfValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfBooleanTF/.code args={#1#2#3}{\IfBooleanTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  verbatim/.style={fontupper=\ttfamily,nobeforeafter,tcbox raise base,top=0pt,bottom=0pt,left=1mm,right=1mm,boxrule=0.3mm}
}

%-- tcolorbox --
\long\def\tcb@New@TColorBox#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcolorbox[#3,options@for=#1]}{\endtcolorbox}}

\def\DeclareTColorBox{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\NewTColorBox{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\RenewTColorBox{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\ProvideTColorBox{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

%-- tcolorbox (total) --
\long\def\tcb@New@TotalTColorBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\begin{tcolorbox}[#3,options@for=#1]#4\end{tcolorbox}}}

\def\DeclareTotalTColorBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\NewTotalTColorBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\RenewTotalTColorBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\ProvideTotalTColorBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

%-- tcbox --
\long\def\tcb@New@TCBox#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]}}

\def\DeclareTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\NewTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\RenewTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\ProvideTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

%-- tcbox (total) --
\long\def\tcb@New@TotalTCBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\NewTotalTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\RenewTotalTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\ProvideTotalTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\DeclareTotalTCBox{\tcboxverb}{ O{} v }{verbatim,#1}{#2}

%-- tcboxfit --
\long\def\tcb@New@TCBoxFit#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]}}

\def\DeclareTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\NewTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\RenewTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\long\def\tcb@New@TotalTCBoxFit#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\NewTotalTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\RenewTotalTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTotalTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}


%-- tcblisting --
\long\def\tcb@New@TCBListing#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\def\DeclareTCBListing{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\NewTCBListing{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\RenewTCBListing{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\ProvideTCBListing{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

%-- tcbinputlisting --
\long\def\tcb@New@TCBInputListing#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbinputlisting{#3,options@for=#1}}%
}

\def\DeclareTCBInputListing{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\NewTCBInputListing{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\RenewTCBInputListing{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\ProvideTCBInputListing{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}


%-- sidebyside --

\def\tcb@sbs@content@none{\tcb@sbs@text@left\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@left{\box\tcb@upperbox\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@right{\tcb@sbs@text@left\tcblower\box\tcb@lowerbox}
\def\tcb@sbs@content@both{\box\tcb@upperbox\tcblower\box\tcb@lowerbox}

\tcbset{%
  sidebyside adapt/.is choice,
  sidebyside adapt/none/.style={%
    sidebyside@adapt@process/.style={%
      code={\let\tcb@sbs@content\tcb@sbs@content@none},
    }%
  },
  sidebyside adapt/left/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\let\tcb@sbs@content\tcb@sbs@content@left},
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  sidebyside adapt/right/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@right},
      righthand width=\wd\tcb@lowerbox,
    }%
  },
  sidebyside adapt/both/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@both},
      text width=\wd\tcb@upperbox+\kvtcb@sbs@gap+\wd\tcb@lowerbox,
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  %
  sidebyside switch/.is choice,
  sidebyside switch/true/.style={%
    sidebyside@switch/.code={%
      \tcb@swap{\tcb@sbs@text@left}{\tcb@sbs@text@right}
    }%
  },
  sidebyside switch/false/.style={%
    sidebyside@switch/.style=%
  },
  sidebyside switch/.default=true
}


\DeclareTotalTColorBox{\tcbsidebyside}{ +O{} +m +m }{%
  code={\long\def\tcb@sbs@text@left{#2}\long\def\tcb@sbs@text@right{#3}},%
  #1,%
  sidebyside,%
  sidebyside@switch,sidebyside@adapt@process%
}{\tcb@sbs@content}


\tcbset{%
  reset@xparse/.style={%
    sidebyside adapt=none,sidebyside switch=false,%
  },
  initialize@reset=reset@xparse,
}


==> tex/experiments_generated_supplement1.tex <==
\onecolumn
{
\footnotesize
\centering
\clearpage
\begin{longtable}{lllllllllll}
\toprule
dataset &
algorithm & 
\parbox{1.5cm}{time\\needed\\overall} & \parbox{1.5cm}{time for\\initial\\ solution} & \parbox{1.5cm}{\#iterations\\Algorithm~\ref{alg:iterative-LP},\ref{alg:iterative-DualLP}} & \parbox{1.5cm}{\#iterations\\TRWS} & \parbox{1.5cm}{logarithmic\\percentage\\partial\\optimality} & \parbox{1.5cm}{percentage\\exluded\\labels}\\
\hline
\endhead%

\hline
 \multicolumn{ 8 }{c}{ ProteinFolding } \\\hline
1CKK & IRI\_CPLEX & 2757.62 & 1177.62 & 5 & $\dagger$ & 14.24\% & 27.04\%\\
1CKK & IRI\_SHEKHOVTSOV & 15.00 & 13.42 & 3 & 1000+60 & 14.25\% & 29.19\%\\
1CKK & IRI\_TRWS & 156.53 & 30.27 & 6 & 288+32 & 13.93\% & 26.90\%\\
1CKK & MQPBO & 825.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
1CKK & MQPBO\_10 & 5670.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
1CKK & PBP\_CPLEX & 2502.69 & 2493.65 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
1CKK & PBP\_TRWS & 47.57 & 30.19 & 2 & 288+185 & 0.00\% & 0.00\%\\
1CM1 & IRI\_CPLEX & 4070.00 & 992.15 & 7 & $\dagger$ & 8.38\% & 34.28\%\\
1CM1 & IRI\_SHEKHOVTSOV & 15.00 & 12.71 & 4 & 1000+105 & 8.07\% & 29.98\%\\
1CM1 & IRI\_TRWS & 159.33 & 21.58 & 8 & 242+173 & 8.01\% & 29.79\%\\
1CM1 & MQPBO & 723.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
1CM1 & MQPBO\_10 & 5520.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
1CM1 & PBP\_CPLEX & 2388.46 & 2198.04 & 3 & $\dagger$ & 0.00\% & 0.00\%\\
1CM1 & PBP\_TRWS & 51.33 & 21.60 & 3 & 242+358 & 0.00\% & 0.00\%\\
1SY9 & IRI\_CPLEX & 2628.72 & 416.74 & 5 & $\dagger$ & 25.34\% & 51.30\%\\
1SY9 & IRI\_SHEKHOVTSOV & 16.00 & 14.72 & 4 & 1000+20 & 28.11\% & 58.09\%\\
1SY9 & IRI\_TRWS & 116.34 & 46.74 & 7 & 400+30 & 27.10\% & 56.56\%\\
1SY9 & MQPBO & 2112.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.11\%\\
1SY9 & MQPBO\_10 & 7494.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
1SY9 & PBP\_CPLEX & 1067.46 & 910.90 & 4 & $\dagger$ & 0.00\% & 0.00\%\\
1SY9 & PBP\_TRWS & 66.73 & 46.77 & 5 & 400+174 & 0.00\% & 0.00\%\\
2BBN & IRI\_CPLEX & 9677.42 & 5476.81 & 5 & $\dagger$ & 2.12\% & 8.58\%\\
2BBN & IRI\_SHEKHOVTSOV & 24.00 & 23.01 & 3 & 1000+10 & 2.32\% & 11.52\%\\
2BBN & IRI\_TRWS & 370.43 & 42.99 & 5 & 242+16 & 1.45\% & 7.21\%\\
2BBN & MQPBO & 2429.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2BBN & MQPBO\_10 & 1736.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2BBN & PBP\_CPLEX & 9776.60 & 9771.18 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2BBN & PBP\_TRWS & 54.21 & 42.90 & 2 & 242+146 & 0.00\% & 0.00\%\\
2BCX & IRI\_CPLEX & 36222.90 & 6998.66 & 5 & $\dagger$ & 4.81\% & 15.66\%\\
2BCX & IRI\_SHEKHOVTSOV & 23.00 & 20.90 & 3 & 1000+55 & 4.43\% & 14.45\%\\
2BCX & IRI\_TRWS & 303.15 & 40.08 & 5 & 252+16 & 3.88\% & 14.63\%\\
2BCX & MQPBO & 1288.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2BCX & MQPBO\_10 & 1008.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2BCX & PBP\_CPLEX & 11419.60 & 11409.90 & 2 & $\dagger$ & 0.00\% & 0.00\%\\
2BCX & PBP\_TRWS & 55.26 & 39.60 & 2 & 252+194 & 0.00\% & 0.00\%\\
2BE6 & IRI\_CPLEX & 1381.60 & 765.84 & 4 & $\dagger$ & 9.14\% & 17.68\%\\
2BE6 & IRI\_SHEKHOVTSOV & 12.00 & 10.72 & 4 & 1000+60 & 9.03\% & 17.52\%\\
2BE6 & IRI\_TRWS & 132.24 & 28.19 & 4 & 363+10 & 7.88\% & 18.07\%\\
2BE6 & MQPBO & 540.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2BE6 & MQPBO\_10 & 3728.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.05\%\\
2BE6 & PBP\_CPLEX & 1552.95 & 1552.88 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2BE6 & PBP\_TRWS & 40.12 & 28.12 & 2 & 363+230 & 0.00\% & 0.00\%\\
2F3Y & IRI\_CPLEX & 3628.90 & 2546.68 & 5 & $\dagger$ & 6.22\% & 10.66\%\\
2F3Y & IRI\_SHEKHOVTSOV & 15.00 & 13.88 & 3 & 1000+55 & 8.50\% & 13.87\%\\
2F3Y & IRI\_TRWS & 182.90 & 32.58 & 5 & 321+15 & 8.90\% & 15.81\%\\
2F3Y & MQPBO & 928.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.05\%\\
2F3Y & MQPBO\_10 & 5138.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2F3Y & PBP\_CPLEX & 4618.78 & 4618.76 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2F3Y & PBP\_TRWS & 41.87 & 33.03 & 3 & 321+164 & 0.00\% & 0.00\%\\
2FOT & IRI\_CPLEX & 7458.75 & 1996.55 & 5 & $\dagger$ & 4.10\% & 11.64\%\\
2FOT & IRI\_SHEKHOVTSOV & 16.00 & 14.02 & 4 & 1000+60 & 3.63\% & 10.72\%\\
2FOT & IRI\_TRWS & 218.88 & 44.37 & 6 & 398+15 & 4.07\% & 11.35\%\\
2FOT & MQPBO & 1054.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.07\%\\
2FOT & MQPBO\_10 & 4961.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.09\%\\
2FOT & PBP\_CPLEX & 4473.58 & 4440.51 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2FOT & PBP\_TRWS & 61.92 & 44.42 & 2 & 398+222 & 0.00\% & 0.00\%\\
2HQW & IRI\_CPLEX & 5721.95 & 1946.20 & 6 & $\dagger$ & 10.30\% & 17.30\%\\
2HQW & IRI\_SHEKHOVTSOV & 16.00 & 13.00 & 6 & 1000+150 & 8.33\% & 18.18\%\\
2HQW & IRI\_TRWS & 188.79 & 35.54 & 7 & 382+44 & 10.31\% & 17.35\%\\
2HQW & MQPBO & 1193.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2HQW & MQPBO\_10 & 7228.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2HQW & PBP\_CPLEX & 2163.98 & 2161.07 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2HQW & PBP\_TRWS & 44.07 & 35.46 & 2 & 382+121 & 0.00\% & 0.00\%\\
2O60 & IRI\_CPLEX & 12085.40 & 3007.95 & 6 & $\dagger$ & 4.22\% & 12.81\%\\
2O60 & IRI\_SHEKHOVTSOV & 19.00 & 17.21 & 3 & 1000+55 & 4.17\% & 13.26\%\\
2O60 & IRI\_TRWS & 263.64 & 46.35 & 6 & 352+20 & 4.43\% & 13.57\%\\
2O60 & MQPBO & 1997.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2O60 & MQPBO\_10 & 7516.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
2O60 & PBP\_CPLEX & 6137.07 & 6128.14 & 1 & $\dagger$ & 0.00\% & 0.00\%\\
2O60 & PBP\_TRWS & 93.87 & 46.42 & 2 & 352+369 & 0.00\% & 0.00\%\\
3BXL & IRI\_CPLEX & 3247.11 & 915.86 & 7 & $\dagger$ & 4.97\% & 17.18\%\\
3BXL & IRI\_SHEKHOVTSOV & 17.00 & 15.63 & 4 & 1000+65 & 4.66\% & 12.35\%\\
3BXL & IRI\_TRWS & 212.02 & 25.44 & 7 & 227+26 & 4.65\% & 12.33\%\\
3BXL & MQPBO & 1291.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
3BXL & MQPBO\_10 & 6709.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
3BXL & PBP\_CPLEX & 1776.23 & 1598.07 & 2 & $\dagger$ & 0.00\% & 0.00\%\\
3BXL & PBP\_TRWS & 44.71 & 25.52 & 2 & 227+216 & 0.00\% & 0.00\%\\
pdb1b25 & IRI\_CPLEX & 1599.67 & 55.01 & 28 & $\dagger$ & 76.76\% & 84.05\%\\
pdb1b25 & IRI\_SHEKHOVTSOV & 15.00 & 12.82 & 13 & 1000+155 & 82.92\% & 87.84\%\\
pdb1b25 & IRI\_TRWS & 96.29 & 27.72 & 28 & 443+481 & 38.73\% & 58.27\%\\
pdb1b25 & MQPBO & 2.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 1.99\%\\
pdb1b25 & MQPBO\_10 & 27.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.53\%\\
pdb1b25 & PBP\_CPLEX & 324.64 & 72.11 & 14 & $\dagger$ & 18.84\% & 22.32\%\\
pdb1b25 & PBP\_TRWS & 119.71 & 27.62 & 14 & 443+1238 & 18.92\% & 22.34\%\\
pdb1d2e & IRI\_CPLEX & 154.76 & 25.44 & 5 & $\dagger$ & 97.30\% & 97.98\%\\
pdb1d2e & IRI\_SHEKHOVTSOV & 7.00 & 6.76 & 6 & 1000+80 & 97.00\% & 98.26\%\\
pdb1d2e & IRI\_TRWS & 9.20 & 6.14 & 7 & 190+30 & 97.63\% & 98.35\%\\
pdb1d2e & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.74\%\\
pdb1d2e & MQPBO\_10 & 12.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.61\%\\
pdb1d2e & PBP\_CPLEX & 483.55 & 34.59 & 25 & $\dagger$ & 55.53\% & 58.94\%\\
pdb1d2e & PBP\_TRWS & 83.82 & 6.16 & 47 & 190+2775 & 55.69\% & 58.98\%\\
pdb1fmj & IRI\_CPLEX & 99.33 & 12.35 & 7 & $\dagger$ & 92.58\% & 94.90\%\\
pdb1fmj & IRI\_SHEKHOVTSOV & 3.00 & 3.17 & 6 & 1000+40 & 89.94\% & 92.54\%\\
pdb1fmj & IRI\_TRWS & 7.85 & 2.96 & 11 & 186+98 & 89.92\% & 93.34\%\\
pdb1fmj & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.04\%\\
pdb1fmj & MQPBO\_10 & 6.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.92\%\\
pdb1fmj & PBP\_CPLEX & 77.30 & 16.97 & 11 & $\dagger$ & 15.94\% & 18.83\%\\
pdb1fmj & PBP\_TRWS & 16.67 & 3.10 & 11 & 186+677 & 16.18\% & 18.91\%\\
pdb1i24 & IRI\_SHEKHOVTSOV & 0.00 & 0.08 & 2 & 60+5 & 99.73\% & 99.94\%\\
pdb1i24 & IRI\_TRWS & 1.00 & 0.89 & 0 & 115+-115 & 100.00\% & 100.00\%\\
pdb1i24 & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.43\%\\
pdb1i24 & MQPBO\_10 & 3.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.85\%\\
pdb1i24 & PBP\_CPLEX & 5.66 & 5.66 & 0 & $\dagger$ & 100.00\% & 100.00\%\\
pdb1i24 & PBP\_TRWS & 0.82 & 0.82 & 0 & 115+-115 & 100.00\% & 100.00\%\\
pdb1iqc & IRI\_CPLEX & 111.58 & 18.51 & 5 & $\dagger$ & 99.10\% & 99.63\%\\
pdb1iqc & IRI\_SHEKHOVTSOV & 3.00 & 2.80 & 8 & 560+70 & 96.34\% & 97.09\%\\
pdb1iqc & IRI\_TRWS & 11.00 & 4.06 & 10 & 169+40 & 97.31\% & 98.08\%\\
pdb1iqc & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.90\%\\
pdb1iqc & MQPBO\_10 & 8.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 6.06\%\\
pdb1iqc & PBP\_CPLEX & 229.09 & 24.36 & 20 & $\dagger$ & 35.32\% & 41.15\%\\
pdb1iqc & PBP\_TRWS & 36.03 & 4.06 & 28 & 169+2058 & 40.50\% & 45.56\%\\
pdb1jmx & IRI\_CPLEX & 142.20 & 15.52 & 9 & $\dagger$ & 97.24\% & 98.69\%\\
pdb1jmx & IRI\_SHEKHOVTSOV & 2.00 & 1.71 & 5 & 450+95 & 96.66\% & 98.20\%\\
pdb1jmx & IRI\_TRWS & 13.95 & 3.60 & 13 & 188+202 & 35.80\% & 58.70\%\\
pdb1jmx & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.73\%\\
pdb1jmx & MQPBO\_10 & 8.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.76\%\\
pdb1jmx & PBP\_CPLEX & 121.71 & 16.21 & 19 & $\dagger$ & 35.86\% & 39.98\%\\
pdb1jmx & PBP\_TRWS & 20.02 & 3.59 & 24 & 188+1098 & 35.26\% & 39.12\%\\
pdb1kgn & IRI\_CPLEX & 196.03 & 17.97 & 10 & $\dagger$ & 89.22\% & 93.23\%\\
pdb1kgn & IRI\_SHEKHOVTSOV & 5.00 & 4.41 & 10 & 940+140 & 88.03\% & 92.42\%\\
pdb1kgn & IRI\_TRWS & 25.24 & 6.40 & 14 & 268+342 & 36.13\% & 58.54\%\\
pdb1kgn & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.27\%\\
pdb1kgn & MQPBO\_10 & 9.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.24\%\\
pdb1kgn & PBP\_CPLEX & 161.57 & 24.37 & 12 & $\dagger$ & 39.42\% & 39.67\%\\
pdb1kgn & PBP\_TRWS & 53.49 & 6.45 & 17 & 268+1824 & 13.20\% & 13.36\%\\
pdb1kwh & IRI\_CPLEX & 105.77 & 9.63 & 10 & $\dagger$ & 79.09\% & 85.64\%\\
pdb1kwh & IRI\_SHEKHOVTSOV & 2.00 & 1.99 & 8 & 930+70 & 76.53\% & 83.26\%\\
pdb1kwh & IRI\_TRWS & 5.85 & 2.44 & 15 & 208+84 & 78.93\% & 85.67\%\\
pdb1kwh & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.43\%\\
pdb1kwh & MQPBO\_10 & 5.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.99\%\\
pdb1kwh & PBP\_CPLEX & 51.33 & 12.89 & 9 & $\dagger$ & 25.54\% & 31.15\%\\
pdb1kwh & PBP\_TRWS & 9.15 & 2.43 & 8 & 208+401 & 25.43\% & 31.13\%\\
pdb1m3y & IRI\_CPLEX & 73.60 & 18.58 & 3 & $\dagger$ & 98.54\% & 99.47\%\\
pdb1m3y & IRI\_SHEKHOVTSOV & 6.00 & 5.38 & 8 & 1000+105 & 89.55\% & 92.87\%\\
pdb1m3y & IRI\_TRWS & 15.17 & 4.84 & 8 & 200+190 & 46.64\% & 66.91\%\\
pdb1m3y & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 5.72\%\\
pdb1m3y & MQPBO\_10 & 8.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 6.38\%\\
pdb1m3y & PBP\_CPLEX & 120.60 & 25.18 & 14 & $\dagger$ & 31.05\% & 27.97\%\\
pdb1m3y & PBP\_TRWS & 28.19 & 4.82 & 12 & 200+1135 & 31.08\% & 27.98\%\\
pdb1qks & IRI\_CPLEX & 138.12 & 15.19 & 8 & $\dagger$ & 98.30\% & 98.93\%\\
pdb1qks & IRI\_SHEKHOVTSOV & 3.00 & 2.75 & 3 & 670+60 & 98.57\% & 99.38\%\\
pdb1qks & IRI\_TRWS & 4.05 & 3.25 & 3 & 161+6 & 99.74\% & 99.89\%\\
pdb1qks & MQPBO & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 3.68\%\\
pdb1qks & MQPBO\_10 & 9.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 5.09\%\\
pdb1qks & PBP\_CPLEX & 96.77 & 15.82 & 12 & $\dagger$ & 28.18\% & 26.37\%\\
pdb1qks & PBP\_TRWS & 27.99 & 3.24 & 15 & 161+1154 & 30.63\% & 28.46\%\\

\hline
 \multicolumn{ 8 }{c}{ color-seg } \\\hline
colseg-cow3 & IRI\_SHEKHOVTSOV & 550.00 & 353.53 & 11 & 1000+360 & 99.94\% & 99.95\%\\
colseg-cow3 & IRI\_TRWS & 830.22 & 665.31 & 1 & 826+0 & 100.00\% & 100.00\%\\
colseg-cow3 & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 99.89\%\\
colseg-cow3 & MQPBO & 24.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 32.06\%\\
colseg-cow3 & MQPBO\_10 & 206.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 43.55\%\\
colseg-cow3 & PBP\_TRWS & 7530.72 & 690.55 & 14 & 826+6056 & 99.95\% & 99.95\%\\
colseg-cow4 & IRI\_SHEKHOVTSOV & 555.00 & 370.12 & 8 & 1000+305 & 99.91\% & 99.92\%\\
colseg-cow4 & IRI\_TRWS & 1271.03 & 751.09 & 18 & 848+314 & 99.93\% & 99.94\%\\
colseg-cow4 & Kovtun & 2.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 99.90\%\\
colseg-cow4 & MQPBO & 40.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.37\%\\
colseg-cow4 & MQPBO\_10 & 46.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.56\%\\
colseg-cow4 & PBP\_TRWS & 7395.03 & 742.58 & 10 & 848+6349 & 99.80\% & 99.80\%\\
colseg-garden4 & IRI\_SHEKHOVTSOV & 19.00 & 17.59 & 3 & 1000+55 & 99.91\% & 99.94\%\\
colseg-garden4 & IRI\_TRWS & 7.28 & 6.88 & 1 & 167+0 & 100.00\% & 100.00\%\\
colseg-garden4 & Kovtun & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 94.96\%\\
colseg-garden4 & MQPBO & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.21\%\\
colseg-garden4 & MQPBO\_10 & 14.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.27\%\\
colseg-garden4 & PBP\_TRWS & 33.68 & 6.75 & 5 & 167+488 & 99.89\% & 99.89\%\\

\hline
 \multicolumn{ 8 }{c}{ color-seg-n4 } \\\hline
clownfish-small & IRI\_SHEKHOVTSOV & 38.00 & 32.23 & 3 & 370+45 & 100.00\% & 100.00\%\\
clownfish-small & IRI\_TRWS & 70.85 & 30.08 & 3 & 223+104 & 99.98\% & 99.99\%\\
clownfish-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 74.11\%\\
clownfish-small & MQPBO & 41.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.67\%\\
clownfish-small & MQPBO\_10 & 536.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 15.83\%\\
clownfish-small & PBP\_TRWS & 151.98 & 30.01 & 6 & 223+610 & 99.97\% & 99.97\%\\
crops-small & IRI\_SHEKHOVTSOV & 33.00 & 30.97 & 3 & 350+10 & 100.00\% & 100.00\%\\
crops-small & IRI\_TRWS & 69.88 & 35.04 & 8 & 260+52 & 99.92\% & 99.97\%\\
crops-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 64.70\%\\
crops-small & MQPBO & 33.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.71\%\\
crops-small & MQPBO\_10 & 577.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 14.32\%\\
crops-small & PBP\_TRWS & 677.08 & 34.88 & 40 & 260+3578 & 99.00\% & 99.00\%\\
fourcolors & IRI\_SHEKHOVTSOV & 1.00 & 0.92 & 2 & 20+5 & 99.96\% & 99.97\%\\
fourcolors & IRI\_TRWS & 3.27 & 2.52 & 1 & 34+0 & 100.00\% & 100.00\%\\
fourcolors & Kovtun & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 69.52\%\\
fourcolors & MQPBO & 3.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
fourcolors & MQPBO\_10 & 37.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
fourcolors & PBP\_TRWS & 31.28 & 2.60 & 8 & 34+238 & 99.92\% & 99.92\%\\
lake-small & IRI\_SHEKHOVTSOV & 6.00 & 4.49 & 2 & 50+5 & 100.00\% & 100.00\%\\
lake-small & IRI\_TRWS & 14.66 & 14.61 & 0 & 95+-95 & 100.00\% & 100.00\%\\
lake-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 74.87\%\\
lake-small & MQPBO & 31.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 6.65\%\\
lake-small & MQPBO\_10 & 607.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 15.31\%\\
lake-small & PBP\_TRWS & 13.75 & 13.75 & 0 & 95+-95 & 100.00\% & 100.00\%\\
palm-small & IRI\_SHEKHOVTSOV & 16.00 & 14.36 & 2 & 160+5 & 100.00\% & 100.00\%\\
palm-small & IRI\_TRWS & 44.46 & 40.44 & 1 & 291+0 & 100.00\% & 100.00\%\\
palm-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 68.65\%\\
palm-small & MQPBO & 19.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
palm-small & MQPBO\_10 & 510.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.48\%\\
palm-small & PBP\_TRWS & 846.27 & 39.97 & 19 & 291+4582 & 98.20\% & 98.20\%\\
penguin-small & IRI\_SHEKHOVTSOV & 7.00 & 6.43 & 2 & 90+5 & 100.00\% & 100.00\%\\
penguin-small & IRI\_TRWS & 15.82 & 15.78 & 0 & 152+-152 & 100.00\% & 100.00\%\\
penguin-small & Kovtun & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 91.99\%\\
penguin-small & MQPBO & 13.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 1.03\%\\
penguin-small & MQPBO\_10 & 193.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 1.42\%\\
penguin-small & PBP\_TRWS & 15.67 & 15.67 & 0 & 152+-152 & 100.00\% & 100.00\%\\
pfau-small & IRI\_SHEKHOVTSOV & 170.00 & 80.04 & 51 & 1000+755 & 89.43\% & 93.41\%\\
pfau-small & IRI\_TRWS & 892.47 & 77.85 & 152 & 654+1341 & 73.55\% & 83.58\%\\
pfau-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 5.59\%\\
pfau-small & MQPBO & 16.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
pfau-small & MQPBO\_10 & 591.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.70\%\\
pfau-small & PBP\_TRWS & 799.08 & 79.34 & 44 & 654+10857 & 10.43\% & 10.43\%\\
snail & IRI\_SHEKHOVTSOV & 3.00 & 2.46 & 2 & 50+5 & 99.99\% & 99.99\%\\
snail & IRI\_TRWS & 7.24 & 6.46 & 1 & 83+0 & 100.00\% & 100.00\%\\
snail & Kovtun & 0.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 97.77\%\\
snail & MQPBO & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 58.35\%\\
snail & MQPBO\_10 & 7.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 77.91\%\\
snail & PBP\_TRWS & 46.20 & 6.47 & 5 & 83+332 & 99.98\% & 99.98\%\\
strawberry-glass-2-small & IRI\_SHEKHOVTSOV & 7.00 & 6.20 & 2 & 80+5 & 100.00\% & 100.00\%\\
strawberry-glass-2-small & IRI\_TRWS & 121.36 & 31.42 & 23 & 259+187 & 99.52\% & 99.71\%\\
strawberry-glass-2-small & Kovtun & 1.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 54.99\%\\
strawberry-glass-2-small & MQPBO & 39.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 0.00\%\\
strawberry-glass-2-small & MQPBO\_10 & 528.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 2.78\%\\
strawberry-glass-2-small & PBP\_TRWS & 311.54 & 31.00 & 11 & 259+1721 & 99.31\% & 99.31\%\\

\hline
 \multicolumn{ 8 }{c}{ mrf-photomontage } \\\hline
family-gm & IRI\_SHEKHOVTSOV & 1141.00 & 472.59 & 69 & 1000+1515 & 4.75\% & 4.80\%\\
family-gm & IRI\_TRWS & 4012.16 & 1302.21 & 184 & 1015+1668 & 4.75\% & 4.80\%\\
family-gm & MQPBO & 90.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.34\%\\
family-gm & MQPBO\_10 & 1087.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 4.41\%\\
family-gm & PBP\_TRWS & 12726.45 & 1291.11 & 50 & 1015+22483 & 4.41\% & 4.41\%\\
pano-gm & IRI\_SHEKHOVTSOV & 1336.00 & 695.05 & 45 & 1000+1015 & 65.78\% & 78.06\%\\
pano-gm & IRI\_TRWS & 8812.30 & 1513.88 & 62 & 911+1531 & 68.37\% & 79.52\%\\
pano-gm & MQPBO & 97.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 40.37\%\\
pano-gm & MQPBO\_10 & 646.00 & 0.00 & 0 & $\dagger$ & 0.00\% & 28.06\%\\
pano-gm & PBP\_TRWS & 14360.45 & 1871.14 & 33 & 911+11193 & 27.55\% & 27.55\%\\

\hline
 \multicolumn{ 8 }{c}{ mrf-stereo } \\\hline
ted-gm & IRI\_SHEKHOVTSOV & 1049.00 & 407.01 & 53 & 1000+1010 & 67.81\% & 72.40\%\\
ted-gm & IRI\_TRWS & 23962.01 & 389.13 & 212 & 689+1552 & 63.11\% & 68.16\%\\
ted-gm & PBP\_TRWS & 3837.51 & 436.30 & 28 & 689+10383 & 38.13\% & 38.13\%\\
tsu-gm & IRI\_SHEKHOVTSOV & 261.00 & 237.86 & 6 & 1000+80 & 99.91\% & 99.94\%\\
tsu-gm & IRI\_TRWS & 737.86 & 223.14 & 4 & 377+266 & 99.97\% & 99.99\%\\
tsu-gm & PBP\_TRWS & 9277.99 & 267.55 & 54 & 377+17421 & 0.39\% & 0.39\%\\
ven-gm & IRI\_SHEKHOVTSOV & 489.00 & 424.80 & 10 & 1000+130 & 0.01\% & 0.02\%\\
ven-gm & IRI\_TRWS & 3191.05 & 1201.52 & 92 & 993+467 & 0.01\% & 0.02\%\\
ven-gm & PBP\_TRWS & 14737.47 & 1451.83 & 55 & 993+16592 & 0.00\% & 0.00\%\\
\bottomrule
\caption{Detailed experimental evaluation for Algorithm~\ref{alg:iterative-LP} utilising CPLEX~\cite{CPLEX} as a subsolver, denoted as IRI\_CPLEX, Algorithm~\ref{alg:iterative-DualLP} utilising TRWS~\cite{TRWSKolmogorov} as a subsolver, denoted as IRI\_TRWS,
   and their counterparts from~\cite{SwobodaPersistencyCVPR2014} denoted by PBP\_CPLEX and PBP\_TRWS.}
\label{tab:DetailedExperimentalEvaluation}
\end{longtable}
}
\twocolumn


==> tex/extra/cuts.tex <==
\subsection{Pruning Cuts}\label{sec:cuts}
By design of \Algorithm{alg:iterative-LP} we have to solve a series of problems, which were simplified to~\eqref{test-problem-r1}. Some further simplification will be possible for the specific class of maps but the problem will generally retain the complexity of a general LP with $\{0,1,-1\}$ matrix. By taking polytopes $\Lambda'$ that do not provide characterization but satisfy requirements of \Theorem{T:nested++}, we obtain necessary conditions that may (but need not) simplify the problem. One simple choice is a ``single node'' polytope:
\begin{equation}
\begin{aligned}
\Lambda_{v,i} = \{\mu\in\Lambda \mid & \mu_{v}(i)+\mu_{v}(y_v) = 1;\\
&(\forall u\neq v)\ \mu_{u}(y_{u}) = 1 \}.
\end{aligned}
\end{equation}
%Minimizing over this polytope gives condition
Minimizing $g$ over this polytope yields expression
\begin{equation}\label{dee-mark}
\min\Big\{ 0,\ g_v(i) + \sum_{u\in\N(v)} g_{vu}(i,y_u)\Big\}.
\end{equation}
If~\eqref{dee-mark} is negative, label $(v,i)$ must be removed from $\Y_v$. %marked as immovable. %After we mark some labels as immovable with the general condition, we can check this local condition %These conditions, checked after 
In \Algorithm{alg:iterative-LP}, after some labels were removed from $\Y_v$  by a general condition, some more labels can be removed quickly by evaluating~\eqref{dee-mark} for every node-label.
\par
We can also chose $\Lambda'$ to be a "move polytope" between test labeling $y$ and any other labeling $x$.
\begin{equation}
\Lambda_{x} = \{\mu\in\Lambda \mid (\forall v\in\V)\ \mu_{v}(y_v)+\mu_{v}(x_v) = 1\}.
\end{equation}
It can be verified that for class $\SP^{2,y}$, there holds $[p](\Lambda_{x}) \subset \Lambda_{x}$. Minimization over $\Lambda_{x}$ reduces to QPBO, and with some additional simplification below to just a submodular problem. 
%Now suppose that during iterations of TRW-S for solving the general characterization problem we happened to obtain a primal integral solution $x$ with $\SE_{g}(x) < 0$. It is clear that the optimal lower bound will be negative and hence some labels will have to be marked. But is is not clear which ones, as only optimal solutions provide a necessary condition. At this point rather than waiting for convergence we can solve the cut problem with $\Lambda_x$. Since $g(x)<0$ the optimal cut will as well be negative. There is therefore a guarantee to remove a non-empty set of labels from sets $\Y_v$.%mark a non-empty set of labels as immovable.
%For example, assume we found a labeling $x$ such that $$

==> tex/extra/integer.tex <==
\subsection{Integer Costs}
%Work with integer energy. 
%This is a very useful paradigm. 
%In practice, the algorithm is cleaner if we work with integer costs $f$. First, we have a limited machine precision any
%If you
We found several good arguments in favor of working with integer costs $f$. If the costs were decimal numbers, it is much harder to claim global optimality. Some tolerance thresholds (\eg on the gap between lower bound and best integer solution (hereafter {\em bound gap})) would have to be introduced and the optimality could be claimed {\em approximately} with this threshold. In contrast, when the input costs are integer the energy of any labeling is integer and we have an optimality guarantee as soon as the bound gap is less than 1. In the case when the integrality gap is $0$, a converging method is guaranteed to achieve a bound gap of, \eg, $1/2$ in a finite number of iterations.
\par
Let us now discuss the relaxed-improving condition~\eqref{equ:linearStrictLPImprovingMapping}. Because even for the integer cost model the optimal value of the relaxation need not be integer, \eqref{equ:linearStrictLPImprovingMapping} may be violated by an arbitrary small margin. However, it is sufficient to require a weaker condition
\begin{equation}\label{L-improving-int}
(\forall \mu\in\Lambda)\tab \<f,(I-[p])\mu\> > -1
\end{equation}
in order to claim that $p$ is an improving map. Such map may increase the energy of some fractional labellings, but it is guaranteed to not increase it for all integer labelings. Again, when the minimization of ~\eqref{L-improving-int} is performed by maximizing the lower bound, we can stop with a robust condition $LB > -1/2$. Note if $f$ is integer, then so is $g = (I-[p]\T)f$ for any idempotent map $p$. This argument however does not apply when a map in $\BS_f$ is to be found. In this case we will use a different, discrete, condition of termination (see step~\ref{trws-return-step} of \Algorithm{Alg:iterative-trws}). %It is therefore more robust 
\par
The difference to introducing a tolerance threshold is that we compute with more precision than that of the input data. (It would be the same to truncate the input data at a predefined precision and carry this precision to the stopping conditions. Working with integer costs establishes a convenient global scale).
%


==> tex/extra/reduction.tex <==
\subsection{Reduced Cost Vector}\label{sec:reduction}
%Problem~\eqref{test-problem-r1}, which we showed to be equivalent to the verification LP is not .
We have shown that problem~\eqref{test-problem-r1} is equivalent to the verification LP in the sense of properties of its optimal solutions needed for \Algorithm{alg:iterative-LP} and is somewhat simpler, because it has fewer marginalization constraints. %This property can in turn be translated into modification of the cost vector
% (its value is negative iff the value ).
%has fewer marginalization constraint. 
%We can exploit this property to eliminate some of the variables in the problem. Expressing some variables explicitly can be cast as making modifications to the energy itself. 
%Absent marginalization in turn decouple some of variables and possibility to 
The absent marginalization constraints, by duality arguments can be translated into a reduction of the cost vector. Another way to see this is as follows. Due to fewer constraints some variables decouple and can be expressed via the remaining variables and their expressions substituted to the objective. The resulting objective will be the new cost vector.
It is the idea of the reduction theorem that we have formulated in \Section{sec:problemReduction} and prove now.
%The end result of the construction is as follows.
\par
\begin{figure}
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cc}
\begin{tabular}{c}\includegraphics[width=0.49\linewidth]{fig/reduction_1-crop.pdf}\end{tabular}\ \ \ \ & 
\begin{tabular}{c}\includegraphics[width=0.49\linewidth]{fig/reduction_2-crop.pdf}\end{tabular}\\
(b) & (d)
\end{tabular}
\caption{Illustration for the proof of problem reduction. Cases (b) and (d) of the proof. In case (b) minimum of the two indicated pairwise costs is assigned to both. In case (d) value of $g_{uv}(i,j)$ can be decreased, assuming all reductions of type (b) and (c) are already performed. }
\end{figure}
%
%
%
\begin{theorem}[Reduction with $\Lambda_P$]\label{T:reduction-L_P}
The support sets of optimal solutions to the reduced verification LP~\eqref{test-problem-r1} are preserved if the cost vector $g$ is replaced in~\eqref{test-problem-r1} with $\bar g$ defined as follows:
%Vector $g = (I -P\T)f$ for the verification LP can be reduced to
\begin{subequations}\label{equ:reductionTheorem-copy}
 \begin{align}
%\notag
	&\bar g_v(x_v) = g_v(x_v),\ v \in\SV;\\
	\label{bar-g-uv}
  &\overline g_{uv}(x_u,x_v)= \\
	\notag
	& \left\{
	%\hskip-5pt
	\setlength{\arraycolsep}{0pt}
  \begin{array}{ll}
   0, & x_u\notin \Y_u, x_v\notin \Y_v\,,\\
   \Delta_{vu}(x_v):=\min\limits_{x_u\notin \Y_u} g_{uv}(x_u,x_v), & x_u\notin \Y_u, x_v\in \Y_v\,,\\
   \Delta_{uv}(x_u):=\min\limits_{x_v\notin \Y_v} g_{uv}(x_u,x_v), & x_u\in \Y_u, x_v\notin \Y_v\,,\\
	\begin{aligned}
   \min\{& \Delta_{vu}(x_v)\cr
	& +\Delta_{uv}(x_u), g_{uv}(x_u,x_v)\},
	\end{aligned} &
	\begin{aligned}
		\vphantom{\min\{\Delta_{vu}(x_v)}\cr
		x_u\in \Y_u, x_v\in \Y_v\,.
	\end{aligned}
  \end{array}
\right.
 \end{align}
\end{subequations}
\end{theorem}
 %``Mapping $p\in\SP^{2,y}$ is strictly $\Lambda$- improving for the cost vector $f$ if and only if for ${\O^* := \argmin_{\mu\in\Lambda} \<\bar g, \mu\>}$ and ${\O_v^* := \{ i\in\X_v \mid (\exists \mu\in\O^*)\ \ \mu_{v}(i)>0 \}}$ there holds ${(\forall v\in\SV) \ \ \O^*_v \cap \Y_v = \emptyset}$. The vector $\bar g$ is defined via $g:=(I-[p])^\top f$ as
%\begin{equation}\label{equ:reductionTheorem-copy}
 %\begin{aligned}
%%\notag
	%&\bar g_v(x_v) = g_v(x_v),\ v \in\SV;\\
  %&\overline g_{uv}(x_u,x_v)=\left\{
  %\begin{array}{ll}
   %0, & x_u\notin \Y_u, x_v\notin \Y_v\,,\\
   %\Delta_{vu}(x_v):=\min_{x_u\notin \Y_u} g_{uv}(x_u,x_v), & x_u\notin \Y_u, x_v\in \Y_v\,,\\
   %\Delta_{uv}(x_u):=\min_{x_v\notin \Y_v} g_{uv}(x_u,x_v), & x_u\in \Y_u, x_v\notin \Y_v\,,\\
   %\min\{\Delta_{vu}(x_v)+\Delta_{uv}(x_u), g_{uv}(x_u,x_v)\}, & x_u\in \Y_u, x_v\in \Y_v\,.\\
  %\end{array}
%\right.
 %\end{aligned}
%\end{equation}
%''.
%\begin{theorem}\label{T:reduction}
%Let $q_{v}(i) = y_v \xi_{v,i} + i(1-\xi_{v,i})$. Let $g = (I-Q\T) f$. Then the value and set of minimizers for problem~\eqref{test-problem-r1} is retained for reduction $\bar g$ with components 
%\begin{equation}\label{test-problem-r2}
 %\begin{aligned}
%%\notag
	%&\bar g_v(x_v) = g_v(x_v),\ v \in\SV;\\
  %&\overline g_{uv}(x_u,x_v)=\left\{
  %\begin{array}{ll}
   %0, & x_u\notin \Y_u, x_v\notin \Y_v\,,\\
   %\Delta_{vu}(x_v):=\min_{x_u\notin \Y_u} g_{uv}(x_u,x_v), & x_u\notin \Y_u, x_v\in \Y_v\,,\\
   %\Delta_{uv}(x_u):=\min_{x_v\notin \Y_v} g_{uv}(x_u,x_v), & x_u\in \Y_u, x_v\notin \Y_v\,,\\
   %\min\{\Delta_{vu}(x_v)+\Delta_{uv}(x_u), g_{uv}(x_u,x_v)\}, & x_u\in \Y_u, x_v\in \Y_v\,.\\
  %\end{array}
%\right.
 %\end{aligned}
%\end{equation}
%\end{theorem}
\begin{proof}
Recall from \Lemma{lambda-p-q} that $\Lambda_{P}$ has only non-negativity constraints, part of the marginalization constraints~\eqref{marg-r1-1-a} associated to labels $i\in \Y_u$ and unary normalization constraints $1\T \mu_u = 1$.
%\begin{align}
%
%\end{align} 
%Let us expand the meaning of constraints $A(I-Q) \mu = 0$.
%We already have expression~\eqref{marg-r1} for node-wise map $Q$ and will specify it now for the map $q_{v}(i) = y_v \leftbb i\in \Y_v \rightbb + i \leftbb i \not\in \Y_v \rightbb$. The linear extension expresses as
%\begin{equation}
%Q_v \mu_v = \mu_v \leftbb i\not\in \Y_v \rightbb + \leftbb i{=}y_v\rightbb \sum_{i'}\mu_{v}(i') \leftbb i' \in \Y_v \rightbb.
%\end{equation}
%The constraint $(I-Q_v)\mu_v = (I-Q_v)(\mu_{vu} \bone)$ expands now as following cases:
%\begin{subequations}
%\begin{align}
%i\in \Y_v: &\tab \mu_v(i) = \sum_{j}\mu_{vu}(i,j)\\
%i\notin \Y_v,\ i\neq y_v: &\tab  0 = 0\\
%\notag
%i = y_v: &\tab \sum_{i'\in \Y_v}\mu_v(i') = \sum_{i'\in \Y_v}\sum_{j}\mu_{vu}(i,j).
%\end{align}
%\end{subequations}
%Note, the constraint in the last case is a combination of constraints from the first case and is therefore redundant.
%The net result is that only marginalization constraints for $i\in \Y_v$ are retained in the reduced problem.
\par
Let $vu\in\SE$. Consider a fourtuple of labels $i\in \X_v$, $i'\in \X_v\backslash{\Y_v}$, $j\in\X_u$, $j'\in\X_u\backslash{\Y_u}$ in the following cases:
\begin{itemize}
\item[(a)] $i\in \X_v\backslash{\Y_v}$, $j \in \X_u\backslash{\Y_u}$. In this case $\mu_{vu}(i,j)$ is unconstrained but also $g_{vu}(i,j) = 0$ so $\mu_{vu}(i,j)$ has no effect on the problem.
\item[(b)]  $i\in \Y_v$, $j\in \X_u\backslash{\Y_u}$. In this case there is only one marginalization constraint where $\mu_{vu}(i,j)$ and $\mu_{vu}(i,j')$ appear, the constraint:
\begin{equation}
\mu_v(i) = \sum_{j''}\mu_{vu}(i,j'').
\end{equation}
Assume $g_{vu}(i,j) < g_{vu}(i,j')$ and assume $\mu$ is a minimizer. If $\mu_{vu}(i,j')>0$ then decreasing it and increasing $\mu_{vu}(i,j)$ preserves feasibility and decreases the objective. It follows that the optimal value for $\mu_{vu}(i,j')$ is $0$. If we decrease the cost $g_{vu}(i,j')$ slightly, preserving the condition $g_{vu}(i,j') > g_{vu}(i,j)$, the optimal value of $\mu_{vu}(i,j')$ remains zero. It follows that we can decrease $g_{vu}(i,j')$ down to $g_{vu}(i,j)$ without affecting the minimizer. More specifically, unary components of any minimizer $(\mu_v(i) \mid v\in\V,\ \in\X_v)$ are preserved. Applying this reasoning iteratively for all pairs $j,j'\in \X_u\backslash{\Y_u}$ we conclude that $g_{vu}(i,j)$ can be set to $\Delta_{vu}(i) = \min_{j\in \X_u\backslash{\Y_u}}g_{vu}(i,j)$ for all $j\in \X_u\backslash{\Y_u}$.
%
\item[(c)] $i\in \X_v\backslash{\Y_v}$, $j\not\in \X_u\backslash{\Y_u}$. This case is symmetric to (b), we can set $g_{vu}(i,j)$ to  $\Delta_{uv}(j) = \min_{i\in \X_v\backslash{\Y_v}}g_{vu}(i,j)$ for all $i\in \X_v\backslash{\Y_v}$ while retaining all optimal unary components of $\mu$, and thus the support sets $(\O_u \mid u\in\V)$.
\item[(d)]  $i\in \Y_v$, $j\in \Y_u$. In this case we have 3 unknowns constrained by 2 marginalization constraints:
\begin{subequations}
\begin{align}
&\mu_{vu}(i,j) + \mu_{vu}(i,j')  = \bar \mu_v(i),\\
&\mu_{vu}(i,j) + \mu_{vu}(i',j)  = \bar \mu_u(j),
\end{align}
\end{subequations}
where $\bar \mu_v(i) = \mu_v(i)-\sum_{j''\neq j,j'}\mu_{vu}(i,j'')$ temporary denotes the contribution of other variables and similarly $\bar \mu_u(j)$. Assume that $g_{vu}(i,j)>g_{vu}(i,j')+g_{vu}(i',j)$. %Assume for contradiction that $\mu_{vu}(i,j)>0$ in the optimal solution. 
%In this case we can decrease $\mu_{vu}(i,j)$ and $\mu_{vu}(i',j')$ by $\varepsilon < \mu_{vu}(i,j)$ and increase $\mu_{vu}(i',j)$ and $\mu_{vu}(i,j')$ by $\varepsilon$. This transformation preserves feasibility and decreases the objective by $\varepsilon(g_{vu}(i,j)-g_{vu}(i,j')-g_{vu}(i',j))$, which contradicts optimality of $\mu$.
In this case an optimal solution $\mu$ must have $\mu_{vu}(i,j)=0$ since otherwise $\mu_{vu}(i,j)$ can be decreased and both $\mu_{vu}(i,j')$ and $\mu_{vu}(i',j)$ increased by the same amount resulting in a feasible solution (since reduced marginalization and non-negativity are preserved) with strictly better objective. It follows that $g(i,j)$ can be set to $\min\big\{g_{vu}(i,j),g_{vu}(i,j')+g_{vu}(i',j) \big\}$ not affecting the  support sets of optimal solutions $(\O_u \mid u\in\V)$. By considering all choices of $i'\in \X_v\backslash{\Y_v}$ and $j'\in \X_u\backslash{\Y_u}$ we get the reduced cost vector as specified in~\eqref{equ:reductionTheorem-copy}.
\end{itemize}
\end{proof}

\par
{\noindent \bf Theorem~\ref{thm:reductionTheorem} (Reduction with $\Lambda$).} The theorem formulated in \Section{sec:problemReduction} states that we can use reduced cost vector $\bar g$ with the initial polytope $\Lambda$.
\begin{proof}
%We need to show that after changing the cost vector in the optimization over the reduced polytope $\Lambda_P$ we may switch back to the initial polytope $\Lambda$. 
%We will show that verification LP with cost vector $\bar g$ has the same support sets of optimal solutions as reduced verification LP.

By \Theorem{T:reduction-L_P}, solving the reduced verification LP~\eqref{test-problem-r1} with cost vector $\bar g$ gives the same support sets $O_v$ as with cost vector $g$. We will show now that for every optimal solution $\mu'\in \Lambda_P$ there is always an optimal solution $\mu\in\Lambda$ that has the same cost and same unary components. 
%Essentially, we need to construct a solution $\mu'$ that satisfies pairwise normalization constraint. 
\par
For simplicity and \Wlog, we will contract all labels $\X_v\backslash{\Y_v}$ into a single label $y_v$ for each node $v$. This can be done because all associated unary and pairwise terms of $\bar g$ are equal among these labels.
%Since all unary and pairwise terms of $\bar g$ associated with labels $i' \in \X_v\backslash{\Y_v}$ (resp. with pairs $i' \in \X_v\backslash{\Y_v}$, $j' \in \X_u\backslash{\Y_u}$) equal zero, we can consider for simplicity that the optimal solution has for all $i' \in \X_v\backslash{\Y_v}\backslash\{y_v\}$ all components $\mu_{v}(i') = 0$, and only $\mu_{v}(y_v)$ may be non-zero (label $y_v$ is chosen as representative). Similarly, among pairwise components $\mu_{vu}(i,j')$ for $j'\in\X_u\backslash{\Y_u}$ (as they have equal cost in $\bar g$) we chose the solution with weight concentrated on $\mu_{vu}(i,y_u)$.
%\par
%Let $vu\in\SE$. Let $i\in \Y_v$, $j, j'\in\X_u\backslash{\Y_u}$. Because $\bar g_vu(i,j') = g_vu(i,j')$
\par
Let $\mu'\in \Lambda_P$ be an optimal solution and let us initialize $\mu:=\mu'$.
Let $vu\in\SE$. Consider a pair of labels $i\in \Y_v$, $j\in\Y_u$. There holds $g_{vu}(i,j) \leq \bar g_{vu}(i,y_u)+g_{vu}(y_v,y_u)$. If $\mu_{vu}(i,y_u)>0$ and $\mu_{vu}(y_v,j)>0$ simultaneously, then we can decrease both and increase $\mu_{vu}(i,j)$. Feasibility to $\Lambda_P$ is preserved and the cost will not increase. Thus we can select optimal $\mu$ such that its pairwise components satisfy either
\begin{align}
(\forall j\in \Y_u)\ \mu_{vu}(y_v,j) = 0
\end{align}
or the symmetric expression
\begin{align}
(\forall i\in \Y_v)\ \mu_{vu}(i,y_u) = 0.
\end{align}
Let it be the first case.
Component $\mu_{vu}(y_v,y_v)$ is unconstrained in $\Lambda_P$ and has zero cost $\bar g_{vu}(y_v,y_u)$. Let us chose 
\begin{align}
\mu_{vu}(y_v,y_u) := \mu_v(y_v);
\end{align}
Such solution $\mu$ satisfies all marginalization constraints with node $u$. The only remaining marginalization constraint with node $v$ at label $y_v$ is implied. It can be verified as follows. From marginalization with $v$ and normalization at $u$ there holds $\sum_{i,j}\mu_{vu}(i,j) = 1$. Then using also normalization constraint at $u$:
%It follows that $\sum_{i,j}\mu_{vu}(i,j) = 1$.
%It remains to verify marginalization constraint with node $v$ at label $y_v$. %Let us calculate the sum of all pairwise terms but 
\begin{align}
\sum_{i\in\X_u} \mu_{vu}(i,y_u) = &1 - \sum_{i\in\X_u}\sum_{j\neq y_v} \mu_{vu}(i,j) \\
\notag
= & 1- \sum_{j\neq y_v} \mu_{u}(j) = \mu_{u}(y_v).
\end{align}
%For such solution $\mu$, using normalization and marginalization constraints of $\Lambda_P$, we have
%\begin{align}
%\sum\csub{i\in\X_v \\ j\in\Y_u} \mu_{vu}(i,j)
%\end{align}
It follows that $\mu\in\Lambda$, $\<\mu,\bar g\> = \<\mu',\bar g\>$. It is clear that the contracted labels may be expanded back preserving the distribution of unary weights assigned by $\mu'$. Thus unary components of $\mu$ match those of $\mu'$ also in the general case.
\end{proof}

\par
{\noindent \bf Lemma~\ref{lemma:LPrefinement}:}
 ``
%Let $p\in\BS_{f}\cap\SP^{2,y}$ and let $\Lambda'\subseteq\Lambda$. Then ${(\forall v\in\SV) \ \ \O^*_v \cap \Y_v = \emptyset}$ holds for ${\O^* := \argmin_{\mu\in\Lambda'} \<\bar g, \mu\>}$
Let $q\in\BS_{f}\cap\SP^{2,y}$, $Q=[q]$. Let $\Lambda'\subset\Lambda$ and $Q(\Lambda') \subset \Lambda'$. Then $(\forall v\in\SV) \ \ q_v(\O^*_v) =  \O^*_v$ holds for $\O^* := \argmin_{\mu\in\Lambda'} \<\bar g, \mu\>$
''.
\begin{proof}
We need to show that \Theorem{T:nested++} holds with the reduced cost vector. %The result will follow 
\revisit
\end{proof}

Note, taking into account that $g_{vu}(i',j') = 0$ for $i'\in \X_v\backslash{\Y_v}$, $j'\in \X_u\backslash{\Y_u}$, the reduction that we obtained in all cases\footnote{In case (c), for example, two zero edges in addition to the edges $g_{vu}(i,j)$ and $g_{vu}(i,j')$ are considered and the submodularity inequality reduces to $g_{vu}(i,j') -g_{vu}(i,j) \geq 0 $. Since $j$ and $j'$ appear in the reverse order as well, reductions of type (c) altogether enforce modularity of this fourtuple. Case (b) is interpreted similarly.} can be interpreted as forcing the mixed discrete derivative
\begin{equation}\label{partial-submodularity}
g_{vu}(i,j')+g_{vu}(i',j) - g_{vu}(i,j) - g_{vu}(i',j')
\end{equation}
to be non-negative.
Problem $\bar g$ is therefore a (partial) submodular {\em truncation} of $g$. One can notice certain similarity with construction of auxiliary problems by \cite{Kovtun-10}, where full submodularity is enforced. We essentially proved that in part Kovtun's construction is optimal.
\par
Since the reduction only decreases some edges of $g$, it trivially yields a sufficient condition for $\min_{\mu\in\Lambda}\<\mu,g\> < 0$. It is the necessity which is difficult and that we have shown.
\par
The practical aspect of the reduction is that, \eg, TRW-S is able to find a labeling with a negative cost much faster since we have decreased many edge costs. Additionally, minimization over polytope $\Lambda_x$ with reduced $g$ is a purely submodular problem (recall that $y_v\in \X_v\backslash{\Y_v}$). We thus can solve it with a regular minimum cut and not QPBO minimum cut.


==> tex/extra/refined_necessary.tex <==
\section{Proofs of the Reduction}\label{sec:reduction-p}
In this section we prove the reduction \Theorem{thm:reductionTheorem} and the correctness of heuristics (pruning of negative labelings and individual nodes) that are based on \Lemma{lemma:LPrefinement}. We revisit key elements on which \Algorithm{alg:iterative-LP} builds: the verification LP~\eqref{prop:linearStrictLPImprovingMapping}, \Proposition{SI-components} and \Lemma{A1-C1}, which either certifies $p\in\BS_f$ or allows to make pruning. %We generalize these statements in two directions:
%first, we are interested in more general necessary conditions for $p\in\BS_f$
We first generalize these key properties by solving the verification LP approximately. According to \Definition{def:linearStrictLPImprovingMapping}, mapping $p$ is strictly improving only if the value of the verification LP is zero. It is easy to see that solving the verification LP within a guaranteed approximation ratio provides an exact answer to the question whether the optimal value is zero. We then look at the set of optimal solutions of the approximation problem and prove that an analog of \Lemma{A1-C1} holds, \ie, this set can be used for pruning.
%
\par
The approximation is obtained by dropping some of the marginalization constraints of $\Lambda$ according to the current mapping $p$. Then we translate this change of the polytope to the change of the cost vector $g$. By the end of the section we are back to optimizing over standard polytope $\Lambda$, for which the inference algorithms are designed, but with a projected (reduced) cost vector $\bar g$, corresponding to solving the approximate verification LP.
%
%
\subsection{Reduced Polytope}\label{sec:refined_necessary}
%To this end we successfully avoided speaking of the non strictly $\Lambda$-improving mapping, but now we have to introduce it.
%\begin{definition}\cite{shekhovtsov-14} Mapping $p\colon \X \to \X$ is called (weakly) $\Lambda$-improving for $f$ if
%\begin{align}
%\min_{\mu\in\Lambda} \<(I-P)\T f, \mu \> \geq 0.
%\end{align}
%\end{definition}
%Clearly, a strictly $\Lambda$-improving mapping must be $\Lambda$-improving.
%%The optimality of \Algorithm{alg:iterative-LP} grounds on the local necessary conditions. % ~\citep[Theorem 3]{shekhovtsov-14}.
%%We now refine these conditions in order to prove optimality with the reduced problem~\eqref{equ:reductionTheorem}. 

The refined conditions and the reduction are based on the following result. Due to that $g = (I-P)\T f$ lies in the linear subspace $\Null (P\T)$, if we want to test whether the optimal value is zero or not we can arbitrarily scale the polytope in the directions in the range of $P$. \Ie, in all directions that are orthogonal to the objective cost vector $g$.
%
\par
Let $A$ be the matrix of marginalization constraints
\begin{subequations}
\begin{align}
(\forall uv\in\SE, \forall i\in\X_u)\ \sum_{j}\mu_{uv}(i,j) = \mu_u(i),\\
(\forall uv\in\SE, \forall j\in\X_v)\  \sum_{i}\mu_{uv}(i,j)  = \mu_{v}(j).
\end{align}
\end{subequations}
and $B$ the matrix on the unary normalization constraints
\begin{subequations}
\begin{align}
(\forall v\in\V)\ \sum_{i}\mu_{u}(i) = 1,\\
\mu_0 = 1.
\end{align}
\end{subequations}
%all homogenous equality constraints in the primal~\eqref{LP-big} so that 
Polytope $\Lambda$ may be expressed as
\begin{align}
\Lambda = \{ \mu\in\Real^\SI_+ \mid A\mu =0,\ B \mu = 1\}.
\end{align}
Let us introduce the following relaxed version of polytope $\Lambda$ corresponding to a mapping $P$:
\begin{equation}
\begin{aligned}
\Lambda_P = \{\mu\in\Real^\SI_+ \mid\ & A(I-P)\mu = 0,\ B \mu = 1\}.
\end{aligned}
\end{equation}
%
%
\begin{lemma}[Structure of $\Lambda_P$]\label{L:lambda_p-struct}
Let $P=[p]$ and $p$ be defined by~\eqref{equ:pixelWiseMapping}. Equalities $A(I-P)\mu$ reduce to 
\begin{align}
(\forall v\in\V,\ \forall i\in \Y_u): \tab \mu_u(i) - \sum_{j}\mu_{uv}(i,j) = 0,
\end{align}
\ie, only marginalization constraints for not yet pruned labels are retained in $\Lambda_P$.
\end{lemma}
\begin{proof}
We begin by expanding constraint $A(I-P)\mu = 0$.
The normalization constraints in $A(I-P) \mu = 0$ vanish as they are expressed as
\begin{align}
1\T (I-P_u)\mu_u = ((I-P)\mu)_0
\end{align}
and using the properties $1\T P_u = 1\T$ and $(P_\mu)_0 = \mu_0$ we obtain $0=0$. %simplify to $1\T P_u \mu_u = 1\T \mu_u$.
Marginalization constraints $A(I-P) \mu = 0$ express as
$(\forall vu\in\SE)$ 
\begin{equation}
\begin{aligned}\label{marg-r1-1}
& \mu_u-P_u \mu_u = (\mu_{uv}-P_v \mu_{uv} P_u\T)\T \bone,\\
& \mu_u-P_u \mu_u = \mu_{uv}\T \bone  -P_u \mu_{uv}\T P_v\T \bone,\\
& \mu_u-P_u \mu_u = \mu_{uv}\T \bone  -P_u \mu_{uv}\T \bone,\\
& \mu_u-\mu_{uv}\T \bone =   P_u \mu_u -P_u \mu_{uv}\T \bone,\\
& (I-P_u)(\mu_u-\mu_{uv}\T \bone) = 0.\\
\end{aligned}
\end{equation}
%Let us expand the meaning of constraints $A(I-Q) \mu = 0$.
%We already have expression~\eqref{marg-r1} for pixel-wise map $Q$ and 
Let us further detail this constraint for the map $p$ defined by means of sets $\Y_u$ in~\eqref{equ:pixelWiseMapping}. The linear extension expresses as
\begin{equation}
%P_u \mu_u = \mu_u (1-\xi_{u i}) + \leftbb i{=}y_u\rightbb \sum_{i'}\mu_{u}(i') \xi_{u i'}.
(P \mu)_u(i) = \begin{cases}
0, & i\in \Y_u,\\
\sum\limits_{i'\in\Y_u \cup\{y_u\}}\mu_{u}(i'), & i = y_u,\\
\mu_u(i), & i \notin \Y_u\ \cup\{y_u\}.
%\mu_u(i) \leftbb i{\notin}\Y_u \rightbb , & i\neq y_u\\
%\leftbb i{\notin}\Y_u \rightbb + \leftbb i{=}y_u\rightbb \sum_{i'\in\Y_u}\mu_{u}(i').
\end{cases}
\end{equation}
The constraint~\eqref{marg-r1-1} expands now as following cases:
\begin{subequations}
\begin{align}
\label{marg-r1-1-a}
& i\in \Y_u: \tab \mu_u(i) - \sum_{j}\mu_{uv}(i,j) = 0\\
\label{marg-r1-1-c}
& i\notin \Y_u\cup\{y_u\}: \tab  0 - 0 = 0\\
\notag
& i = y_u: \\
\notag
& \mu_{u}(y_u)-\sum_{j}\mu_{uv}(y_u,j)\\
\notag
&-\Big(\hskip-5pt\sum_{i'\in \Y_u \cup\{y_u\}}\hskip-5pt\mu_u(i') - \hskip-5pt \sum_{i'\in \Y_u \cup\{y_u\}}\sum_{j}\mu_{uv}(i,j)\Big) = 0.
\end{align}
\end{subequations}
In the expression~\eqref{marg-r1-1-c} values depending on $y_u$ cancel inside and outside the brackets and the reminder is nothing but a sum of constraints~\eqref{marg-r1-1-a} over $i\in\Y_s$. This constraint is therefore redundant. Only constraint~\eqref{marg-r1-1-a} remains, \ie, only marginalization constraints for not yet pruned labels are retained in $\Lambda_P$.
\end{proof}

Clearly, $\Lambda\subset \Lambda_P$ because from $\mu\in\Lambda$ follows $P\mu\in\Lambda$ and therefore $AP\mu =0$ and $A(I-P)\mu = A\mu - (A P\mu) = 0$. We have also the following property:
%
%
\begin{lemma}\label{L:PLambdaP}
Let $p\colon \X \to \X$ node-wise idempotent and $P = [p]$. Then $P(\Lambda_P) \subset \Lambda_P$.
\end{lemma}
\begin{proof}
Let $\mu\in\Lambda_P$ and $\mu' = P \mu$. 
Clearly, $\mu'\geq 0$ since $P$ has non-negative coefficients, \cf equation~\eqref{equ:PixelLinearExtension}.
Next, $A(I-P)\mu' = A(I-P)P\mu = A(P-P)\mu = 0$. Finally, normalization constraints are verified as $1\T\mu'_v = 1\T P_v\mu_v = 1\T \mu = 1$. Therefore $\mu'$ satisfies all constraints of $\Lambda_P$.
\end{proof}
%
%
The following theorem is a bounded version of statement that appeared in the Characterization Theorem of \citesuppl{shekhovtsov-14-TR}. %If we optimize with the cost vector $(I-P)\T f$, it allows to relax polytope $\Lambda$ to $\Lambda_P$.
It allows to approximate the verification LP with optimization over a simpler polytope $\Lambda_P$. %we optimize with the cost vector $(I-P)\T f$, it allows to relax polytope $\Lambda$ to $\Lambda_P$.
\begin{theorem}[Projection from $\Lambda_P$ to $\Lambda$]\label{T:proj}Let $p\colon \X \to \X$ node-wise idempotent and $P = [p]$. For any $\mu\in\Lambda_P$ there exists vector $\mu^*\in \Lambda$ and $\gamma>0$ such that 
\begin{align}
(I-P) \mu^* = \frac{1}{\gamma}(I-P) \mu.
\end{align}
%where $\gamma = \max_{st} |\X_{st}|$.
\end{theorem}
\begin{proof}We adopt a part of the proof of the characterization theorem~\citesuppl[Theorem 1]{shekhovtsov-14-TR} with slight modifications.
\par
Let $\mu=\mu_1 + \mu_2$, where
\begin{equation}
\begin{aligned}
\mu_1 = P \mu\,;\ \ \ \ \mu_2 = (I-P) \mu\,.
\end{aligned}
\end{equation}
There holds
\begin{equation}
\begin{aligned}
(I-P)\mu_1 & = (I-P)P \mu  = (P-P^2) \mu = 0\,,\\
P \mu_2 & = P (I-P) \mu = 0\,,
\end{aligned}
\end{equation}
\ie, $\mu_1 \in \Null(I-P)$ and $\mu_2 \in \Null(P)$. Let us construct $\mu_1'$ as follows. Let $\gamma = $
\begin{align}\label{gamma-mu1'}
\notag
 &\max\big\{ \max_{uv, ij} |\X_{uv}|(\mu_{1, uv}(i,j), \max_{u,i} |\X_u| \mu_{1,u}(i), \mu_{1,0} \big\}\,,\\
%\notag
& (\mu_1')_{uv} = \gamma / |\X_{uv}|\,,\\
\notag
& (\mu_1')_{u} = \gamma / |\X_{u}|\,,\\
\notag
& (\mu_1')_0 = \gamma\,.
\end{align}
%Let
%\begin{align}\label{eq:gamma}
%%\notag
%%& \gamma = \max_{st, ij} |\X_{st}|\,,\\
%%\notag
%& (\mu_1')_{st} = \gamma / |\X_{st}|\,,\\
%\notag
%& (\mu_1')_{s} = \gamma / |\X_{s}|\,,\\
%\notag
%& (\mu_1')_0 = \gamma\,.
%\end{align}
By construction, $A \mu_1' = 0$ and $B \mu'_1 = \gamma$. 
%By \Lemma{L:PLambdaP}, $\mu_1 \in\Lambda_P$ and therefore all its components are less than $1$ {\red *}. 
It is also clear that $(\mu_1') \geq \mu_1$.
%Because $\mu$ satisfies normalization constraints, there holds $\mu_{u}(i) \leq 1$ for all $u,\ i$ and therefore $(\mu_1') \geq \mu_1$.
%By construction, $(\mu_1') \geq \mu_1$ and $A \mu_1' = 0$.
%\begin{equation}
%(\mu_1') \geq \mu_1 \tab\tab \mbox{and} \tab\tab A \mu_1' = 0\,.
%\end{equation}
Let $\mu_1'' = P \mu_1'$. Because $P \geq 0$, we have
\begin{equation}
\mu_1'' = P \mu_1' \geq P \mu_1 = \mu_1\,.
\end{equation}
On the other hand, $A P \mu_1'' = A P P \mu_1' = A P \mu_1' = 0$ and $(I-P) \mu_1'' = (I-P)P \mu_1' = 0$.
Let
\begin{align}
\mu^* = \frac{1}{\gamma}(\mu_{1}''+\mu_{2}).
\end{align}
There holds
\begin{subequations}
\begin{align}
& \mu^* = \frac{1}{\gamma}(\mu_{1}''+\mu_{2}) \geq \frac{1}{\gamma}(\mu_1 + \mu_{2}) = \frac{1}{\gamma} \mu \geq 0\,,\\
& A(I-P)\mu^* = \frac{1}{\gamma} A(I-P)\mu_2 = \frac{1}{\gamma} A(I-P)\mu = 0\,,\\
& A P\mu^* = \frac{1}{\gamma} A P \mu_1'' = 0\,.
\end{align}
\end{subequations}
It follows that $A \mu^* =0$. Next, we verify normalization constraints for $\mu^*$ as follows: 
\begin{subequations}
\begin{align}
& \mu^*_0 = \frac{1}{\gamma}(\gamma + (\mu_2)_0) = \frac{1}{\gamma}(\gamma + \mu_0 - \mu_0) = 1,\\
\notag
& 1\T \mu^*_u = 1 + \frac{1}{\gamma}1\T(\mu_2)_u = 1 + \frac{1}{\gamma}1\T(I-P_u)\mu_u = 1.
%& 1\T \mu^*_{uv} 1 = 1 + \frac{1}{\gamma}1\T (\mu_{uv} - P_u \mu_{uv} P_v)\T 1 = 1.
\end{align}
\end{subequations}
Therefore, $B\mu^* = 1$. It follows that $\mu^*\in\Lambda$. Finally, $\mu^*$ satisfies the equality claimed by the theorem:
%\begin{equation}
\begin{align}
(I-P)\mu^* &= \frac{1}{\gamma}(I-P)(\mu_{1}''+\mu_{2}) \\
\notag
&= \frac{1}{\gamma}(I-P)\mu_{2} = \frac{1}{\gamma}(I-P)\mu\,.
\end{align}
%\end{equation}
\end{proof}
%Thus, if $\mu$ is a solution to the following {\em reduced verification LP}:
\begin{corollary}\label{C1:proj}
Let $g = (I-P)\T f$. There holds
% The value of the verification LP is negative iff
%\begin{align}
%\frac{1}{\gamma}\min_{\mu\in\Lambda} \<(I-P)\T f,\mu\> \leq \min_{\mu\in\Lambda_P} \<(I-P)\T f,\mu\> \leq \min_{\mu\in\Lambda} \<(I-P)\T f,\mu\>,
%\end{align}
\begin{align}\label{reduced-vLP}
\gamma\min_{\mu\in\Lambda} \<g,\mu\> \leq \min_{\mu\in\Lambda_P} \<g,\mu\> \leq \min_{\mu\in\Lambda} \<g,\mu\>,
\end{align}
where $\gamma = \max_{st} |\X_{st}|$.
\end{corollary}
\begin{proof}
The upper bound holds trivially, because $\Lambda\subset \Lambda_P$. Then, for any solution $\mu\in\Lambda_P$ of the approximation problem (in the middle of~\eqref{reduced-vLP}), \Theorem{T:proj} allows to construct $\mu^* \in\Lambda$ such that $(I-P)\T \mu^* = 1/\gamma (I-P)\T \mu$ with $\gamma$ defined by~\eqref{gamma-mu1'}. Let $\mu$ be an optimal solution.
\par
%Let us show $$
From normalization constraints and non-negativity of $\mu$ follows that unary components $\mu_{u}(i)$ are bounded from above by $1$.
From structure of $\Lambda_P$ given by \Lemma{L:lambda_p-struct} follows that when $p_u(i) \neq i$ the marginalization constraint is active for $i$ and therefore pairwise components $\mu_{uv}(i,j)$ are bounded by $1$ for all $uv\in\SE$ and all $j\in\X_v$. The only unbounded components are $\mu_{uv}(i,j)$ for $i,j$ such that $p_u(i) = i$ and $p_v(j) = j$. They are not constrained and the corresponding cost $g_{u,v}(i,j) = 0$. It is clear that the reduced verification LP is bounded. \Wlog, we may chose optimal $\mu$ with unbounded components set to zero. It follows that all components are bounded by $1$ and thus $\gamma$ can be selected as $\max_{st} |\X_{st}|$.
%An optimal solution $\mu$ may be selected such that 

%It follows that $\mu^*$ is feasible to the LHS and 
From \Theorem{T:proj}, $\gamma \<g, \mu^*\> = \gamma \<f, (I-P)\mu^*\> = \<f, (I-P)\mu\> = \<g,\mu\>$. Therefore the lower bound holds true.
\end{proof}
%
\begin{corollary}\label{C2:proj}
If $P\mu\neq \mu$ then for $\mu^*$ constructed by \Theorem{T:proj} there holds $P\mu^* \neq \mu^*$.
\end{corollary}
\begin{proof}
Let $\tilde \mu = \gamma \mu^*$.
We have $(I-P)\mu = (I-P)\tilde\mu$. Assume $P\mu \neq \mu$. Then $P\mu + (I-P)\mu \neq \mu + (I-P)\tilde\mu$, and opening brackets it gives $\mu \neq \mu +(I-P)\tilde \mu$ and $0 \neq \tilde \mu - P\tilde \mu$. We can now divide by $\gamma$ to obtain the claim.
\end{proof}
%


%The following theorem is a bounded and ``strict'' variant of the Characterization Theorem of \citesuppl{shekhovtsov-14-TR}.
In what follows we will refer to the problem
\begin{align}\label{test-problem-r1}
\min_{\mu\in\Lambda_P}\<(I-P)\T f,\mu\>
\end{align}
as {\em reduced verification LP}. We have shown that it is related to the (non-reduced) verification LP by~\eqref{reduced-vLP}, \ie, in terms of the objective value. We can now make a claim about the support sets of its optimal solutions.
%
%
\begin{theorem}\label{reduced-SI}
Let $P=[p]$ and $g=(I-P\T)f$. 
%Mapping $p$ is strictly $\Lambda$-improving for $f$ iff %Condition \eqref{L-improving-min} holds 
Let
\begin{subequations}
\begin{align}\label{reduced-char-a}
&\O = \argmin_{\mu\in\Lambda_P}\<g,\mu\>;\\
&\O_v = \{i\in\X_v \mid (\exists \mu\in\O)\ \mu_{v}(i) > 0 \}.
\end{align}
\end{subequations}
Then $p\in\BS_f$ iff $(\forall v\in\V,\ \forall i\in\O_v) p_v(i)=i$.
\end{theorem}
\begin{proof} Direction ``$\Leftarrow$''. We have $P(\O) = \O$. It follows that the value of the reduced verification LP~\eqref{reduced-char-a} is zero. By \Corollary{C1:proj} (lower bound), the value of the (non-reduced) verification LP is zero as well.
Let $\mu \in \Lambda$ such that $P\mu\neq \mu$. Because $\Lambda \subset \Lambda_P$, $\mu$ is feasible to~\eqref{reduced-char-a}. From $P\mu\neq \mu$ follows that $\mu\notin\O$, \ie $\mu$ is not a minimizer of~\eqref{reduced-char-a}, therefore it must be $\<g,\mu\> > 0$. Thus conditions of \Definition{def:linearStrictLPImprovingMapping} for $P\in\BS_f$ are satisfied.
%Assume for contradiction that $\<g,\mu\> = 0$. 
 %From $P\mu\neq \mu$ follows $\mu\notin \O$ and therefore $\<g,\mu\> > 0$. Let $\mu^*\in\Lambda$ be the vector provided by \Theorem{T:proj}. By \Corollary{C2:proj}, $P \mu^*\neq \mu^*$. By \Corollary{C1:proj}, $\<g,\mu^*\> = \<g,\mu\> > 0$ and .
%
%
\par
Direction ``$\Rightarrow$''. We have $p\in\BS_f$. By \Corollary{C1:proj} the value of the reduced verification LP is zero. %and so sets $O_v$ are well-defined. 
Assume for contradiction that $(\exists v\in\V,\ \exists i\in\O_v) p_v(i)\neq i$.
Then $(\exists \mu\in\O) P \mu \neq \mu$. Let $\mu^*\in\Lambda$ be the vector provided by \Theorem{T:proj} for $\mu$. By \Corollary{C2:proj}, $P \mu^*\neq \mu^*$. From $p$ strictly improving it follows that $\<f, (I-P)\mu^* \> > 0$. But $\<f, (I-P)\mu\>  = \gamma \<f, (I-P)\mu^* \> > 0$, \ie, cost of $\mu$ is positive, which contradicts to $\mu \in \O$.
\end{proof}

Recall that \Algorithm{alg:iterative-LP} verifies in every iteration whether $p$ is strictly $\Lambda$-improving for $f$ and if not it makes adjustments to $p$. \Theorem{reduced-SI} allows to certify termination based on the reduced verification LP, it can be seen as a relaxed version of \Proposition{SI-components}. In order to show that pruning based on the reduced verification LP is correct we need an analog of \Lemma{A1-C1}. We will extend \Theorem{reduced-SI} in two directions: to make claim about all strictly improving relaxed mappings $q\in\BS_f$ such that $q\leq p$ and to allow a weaker polytope to enable heuristics.

\par
We need first an auxiliary result.
%
%
\begin{lemma}\label{lambda-p-q}
For $q,p\in\SP^{2,y}$ and $q < p$ there holds $\Lambda_{[p]} \subset \Lambda_{[q]}$.
\end{lemma}
\begin{proof}
Let $P=[p]$ and $Q=[q]$. 
%The net result is that only marginalization constraints for $i\in \Y_u$ are retained in the reduced problem.
From \Lemma{L:lambda_p-struct} it is clear that for $q<p$, mapping $q$ retains fewer marginalization constraints than $p$ and therefore $\Lambda_P \subset \Lambda_Q$.
%{\red *}
\end{proof}
%
%
%
%First we show that $\Lambda_\Q \subset$
%use the reduced verification LP instead as it gives the same property for its set of optimal solution as~\eqref{SI-components} for the non-reduced version.
%\par
%We will extend \Theorem{reduced-SI} in one more direction to allow for heuristics.

%As the theorem states, verifying~\eqref{reduced-char} allows to decide whether $p$ is strictly $\Lambda$-improving as well. Problem~\eqref{reduced-char} appears to have fewer constraints than the verification LP~\eqref{equ:linearStrictLPImprovingMapping}, we therefore intend to use it in \Algorithm{alg:iterative-LP}. However, the set of optimal solutions to~\eqref{reduced-char} (assume that we make it bounded by retaining also normalization constraints) would generally differ from that of the initial verification LP~\eqref{equ:linearStrictLPImprovingMapping}. The question is: can we use the set of optimal solutions to~\eqref{reduced-char} for pruning?

%~\eqref{L-improving-min}. %$\min_{\mu\in\Lambda}\<(I-[q]\T)f,\mu\>$. 
%The refined necessary condition will prove that the solution to~\eqref{reduced-char} can as well be used to prune the set of maps without loss of optimality.
%{\gray
%The reduced problem will be a bit simpler to solve, in particular for TRW-S. In case of Potts model and all-to-one maps, the reduced problem is identical to the auxiliary problem of~\cite{Swoboda-13}, matching in this special case to result obtained above. Another implication of the refined necessary condition will be {\em pruning cuts} -- simpler auxiliary problems that can be employed as a heuristic to reduce {\sc max-wi} problem and solve it much faster.
%\par
%}
%Let us introduce the relaxed version of polytope $\Lambda$ that appears in characterization~\eqref{reduced-char} but with normalization constraints retained, $\Lambda_P = $
%\begin{equation}
%\{\mu\in\Real^\SI_+ \mid A(I-P)\mu = 0,\ 1\T\mu_v = 1,\ \mu\geq 0 \}.
%\end{equation}

\def\mapp{q}
\def\mapq{p}
\def\mapP{Q}
\def\mapQ{P}

%The next theorem show that if $p$ is an upper bound ($\geq$) of all $q\in\BS_f$ (as in Algorithm 1) and we solve reduced problem~\eqref{reduced-char} over the polytope $\Lambda_P$, then all $q\in\BS_f$ must preserve the set of the optimal solutions and therefore we can prune the maps that do not preserve it. We further generalize the claim to any polytope $\Lambda' \subset \Lambda_P$, which is used in heuristics (negative labeling and single node pruning).
%
%
%
\begin{theorem}[Refined Local Necessary Conditions]\label{T:nested++}
Let $\mapp, \mapq$ be node-wise, idempotent and $\mapp \leq \mapq$. Let $Q = [q]$ and $P = [p]$. Let $\Lambda'$ be a polytope such that $\Lambda' \subset \Lambda_{Q}$ and $Q (\Lambda') \subset \Lambda'$.
Let
\begin{subequations}
\begin{align}\label{test-problem++}
& \O' = \argmin\lsub{\mu\in\Lambda'} \<f,(I-\mapQ)\mu\>;\\
& \O'_v = \{i\in\X_v \mid (\exists \mu\in\O')\ \mu_{v}(i)>0 \}.
\end{align}
\end{subequations}
%Then  $\mapp\in\BS_f$ $\Rightarrow$ $(\forall \mu\in\O) \mapP\mu = \mu$.
Then  $q\in\BS_f$ $\Rightarrow$ $(\forall v\in\V,\ \forall i\in\O'_v) \mapp_v(i) = i$.
\end{theorem}
%Thus the solution to the auxiliary problem~\eqref{test-problem++} reveals some information about all strictly improving maps.
\begin{proof}
%{\bf (a)\ }
%
%Assume for contradiction $\mapP(\O) \nsubseteq \O$. Then there exists $\mu\in \O$ such that $\mapP\mu \notin\O$ and at the same time $\mapP\mu \in \Lambda'$. 
%%We need to show in addition to 
%%\par
%Because $\mu$ is optimal and $\mapP\mu$ is feasible but not optimal to~\eqref{test-problem++} we have 
%\begin{equation}
%\<f,(I-\mapQ) \mu\> < \<f, (I-\mapQ) \mapP \mu\>.
%\end{equation}
%Equivalently, $0 > \<f,((I-\mapQ) -(I-\mapQ)\mapP ) \mu\>  = \<f,(I-\mapP) \mu\>$.
%Because $\Lambda' \subseteq \Lambda_P$ it follows that
%%Because $\mu\in\Lambda_P$, we have that
%\begin{equation}
%\min\lsub{\mu\in\Lambda_P} \<f,(I-\mapP)\mu\> <0,
%\end{equation}
%which contradicts to $\mapp\in \BW_f$.
%%
%%
%\par{\bf (b)\ } 
%We first need to show that strict $\Lambda$-improving inequality extends to hold over $\Lambda_P$. 
%For $\mu\in\Lambda_P$, the proof of Characterization Theorem~\citesuppl[Theorem 1]{shekhovtsov-14-TR} constructs a vector $\mu^*\in \coni(\Lambda)$ (where $\coni(\Lambda)$ denotes a conic hull of $\Lambda$) such that $\<f, (I-\mapP) \mu \> = \<f, (I-\mapP) \mu^* \>$. Additionally, because $\mapP(\mu-\mu^*) = \mu-\mu^*$, we have $\mapP\mu\neq \mu$ iff $\mapP\mu^*\neq \mu^*$. It follows that for $\mapP\in\BS_f$ and $\mu\in\Lambda_P$ such that $\mapP \mu\neq \mu$ there holds $\<f, (I-\mapP)\mu\>  = \<f, (I-\mapP)\mu^* \> > 0$.
%\par

Assume for contradiction that $(\exists v\in\V,\ \exists i\in O'_v)\ q_v(i)\neq i$. Then $(\exists \mu\in\O')$ $Q \mu\neq \mu$.
%Assume for contradiction that $\mu\in\O$ and $\mapP\mu\neq \mu$.
Since $\O' \subset \Lambda' \subset \Lambda_Q$ we have $\mu\in\Lambda_Q$. By \Theorem{T:proj}, there exist $\mu^* \in \Lambda$ such that $(I-Q)\mu^* = 1/\gamma (I-Q)\mu$ and there holds $Q\mu^* \neq \mu^*$. From $q\in\BS_f$, $\mu^*\in\Lambda$ and $Q\mu^*\neq \mu^*$ we have $\<f, (I-Q) \mu^* \> > 0$. And therefore $\<f, (I-Q) \mu \> = \gamma \<f, (I-Q) \mu \> > 0$.
%Since $\O' \subset \Lambda' \subset \Lambda_P$ we have $\mu\in\Lambda_P$. 
%From $q\in\BS_f$ by \Theorem{reduced-SI}, there holds $q$
%By \Theorem{reduced-SI}, from $q\in\BS_f$ follows that $\mu$
%From $q\in\BS_f$ and $Q\mu\neq \mu$ we have {\red *} $\<f, Q \mu \> < \<f, \mu \>$. 
Using $P Q = P$, there holds $(I-Q) = ((I-P) -(I-P)Q )$ and we
obtain $\<f,((I-P) -(I-P)Q ) \mu \> > 0$, which implies $\<f,(I-P) \mu \> > \<f, (I-P) Q \mu \>$. Therefore solution $Q\mu \in\Lambda'$ is a better solution for problem~\eqref{test-problem++} than $\mu$, which contradicts $\mu\in \O'$.
%\qed
%We have shown that for $\mu\in\O$ there holds $\mapP\mu = \mu$. Since mapping $\mapp$ is idempotent and node-wise, the component-wise statement $(\forall v\in\V,\ \forall i\in\O_v) \mapp_v(i) = i$ follows.
\end{proof}
Note, for $q \leq p$ there holds $p(q(x)) = p(x)$ for all $x\in\X$, and for their extensions there holds $P Q = P$.
We can now pick freely a polytope $\Lambda'$ to get a necessary condition.
%Let us consider the polytope
%$\Lambda_Q = $
%\begin{equation}
%\{\mu\in\Real^\SI_+ \mid A(I-\mapQ)\mu = 0,\ 1\T\mu_v = 1,\ \mu\geq 0 \}.
%\end{equation}
%which appears in the bounded version of the characterization problem~\eqref{reduced-char}. 
%The inclusion $\Lambda_Q \subset \Lambda$ follows from properties of $[\mapq]$.  We show now that it also satisfies $\mapP (\Lambda_Q) \subset \Lambda_Q$ in two steps.
The next two lemmas show that polytope $\Lambda_P$ satisfies the requirements of the \Theorem{T:nested++}: $\Lambda_P \subset \Lambda_Q$ and $Q (\Lambda_P) \subset \Lambda_P$.

%\begin{lemma}
%If $\mu\in\Lambda_P$ and $P Q = P$ then $\mu\in\Lambda_Q$.
%\end{lemma}
%\begin{proof}
%%We now show $\mu\in\Lambda_P$ using $QP = \mapQ$ and $A(I-\mapQ)\mu=0$ in the following chain
%We use identities $P Q = P$ and $A (I-P) \mu = 0$ in the following chain {\red *}:
%\begin{equation}
%\begin{aligned}
%&A(I-P)Q\mu = 0\\
%&A(\mapP-P Q)\mu = 0\\
%&A(\mapP-\mapQ)\mu = 0\\
%&A(\mapP-I)\mu = 0.\\
%\end{aligned}
%\end{equation}
%Statement $\mu \in \Lambda_Q$ is proven.
%\end{proof}


\begin{lemma}
Let $p,q\in\SP^{2,y}$, $q<p$, $P=[p]$, $Q=[q]$. Then $Q(\Lambda_{P}) \subset \Lambda_{P}$.
\end{lemma}
\begin{proof}
Let $\mu\in\Lambda_P$. We need to show that $Q\mu \in\Lambda_P$ as well. 
Clearly, $Q\mu$ satisfies non-negativity and normalization constraints. Marginalization constraints are verified as follows.
From $\mu\in\Lambda_P$ we have $A\mu = A P \mu$.
By \Lemma{lambda-p-q} there holds $\Lambda_{[p]} \subset \Lambda_{[q]}$ and therefore $A\mu = A Q\mu$. 
Using the relation $PQ = P$, we express
\begin{equation}
\begin{aligned}
& A(I-P) Q \mu =  A(Q-P) \mu = \\
& A Q \mu - A P \mu = A \mu- A\mu = 0.
\end{aligned}
\end{equation}
It follows that $Q \mu$ satisfies constraints of $\Lambda_P$.
\end{proof}
%
%
%%By \Lemma{L:PLambdaP}, $[q](\Lambda_[q]) \subset \Lambda_[q]$
%Because mapping $\mapQ$ is node-wise, marginalization constraints $A(I-\mapQ)\mu = 0$ express as
%
%$(\forall vu\in\SE)$ 
%\begin{equation}
%\begin{aligned}\label{marg-r1}
%& \mu_u-Q_u \mu_u = (\mu_{vu}-Q_v \mu_{vu} Q_u\T)\T \bone,\\
%& \mu_u-Q_u \mu_u = \mu_{vu}\T \bone  -Q_u \mu_{vu}\T Q_v\T \bone,\\
%& \mu_u-Q_u \mu_u = \mu_{vu}\T \bone  -Q_u \mu_{vu}\T \bone,\\
%& \mu_u-\mu_{vu}\T \bone =   Q_u \mu_u -Q_u \mu_{vu}\T \bone,\\
%& (I-Q_u)(\mu_u-\mu_{vu}\T \bone) = 0.\\
%\end{aligned}
%\end{equation}
%From $\mu \in \Lambda_{\mapP}$ we have:
%\begin{equation}
%(I-P_u)(\mu_u-\mu_{vu}\T \bone) = 0;
%\end{equation}
%By chaining, we obtain:
%\begin{equation}
%\begin{aligned}
%& P_u(\mu_u-\mu_{vu}\T \bone) = \mu_u-\mu_{vu}\T \bone = Q_u(\mu_u-\mu_{vu}\T \bone)\\
 %= Q_u & P_u(\mu_u-\mu_{vu}\T \bone).
%\end{aligned}
%\end{equation}
%Or equivalently, 
%\begin{equation}
%(I-Q_u)P_u(\mu_u-\mu_{vu}\T \bone) = 0.
%\end{equation}
%We can now use identity $\bone = P_v\T \bone$ and obtain
%\begin{equation}
%(I-Q_u)(P_u\mu_u-P_u\mu_{vu}\T P_v \bone)  = 0,
%\end{equation}
%which is exactly the reduced marginalization constraint for $\mu' = \mapP \mu$.
%Non-negativity of $\mu'$ follows from non-negativity of components of $\mu$ and $\mapP$. Constraint $\mu'_0 = 1$ holds by definition. Normalization constraints follow as
%\begin{equation}
%1\T \mu'_v = 1\T P_v \mu_v  = 1\T \mu_v  = 1;
%\end{equation}
%Statement $\mapP \mu \in \Lambda_Q$ is proven. 
%%\qed
%\end{proof}
%{\red *} In fact we have a rellation $\Lambda\subset \Lambda_P \subset \Lambda_Q$ for $\mapp\leq \mapq$.
%%Whe have now a necessary condition that any strictly $\Lambda$-improving map $$
%We can replace now the verification problem in step~\ref{alg1:test-\mapp} of \Algorithm{alg:iterative-LP} with
%\begin{equation}\label{test-problem-r1}
%\min_{\mu\in\Lambda_{\mapQ}} \<g,\mu\>.
%\end{equation}
%If the value is zero, by characterization theorem $\mapq$ is strictly $\Lambda$-improving. If the value is negative, then the refined necessary condition tells that all maps $\mapp\in\BS_f$ such that $\mapp\leq \mapq$ must satisfy $[\mapp]\mu = \mu$. And hence all labels $\{(v,i) \mid \mu_{v}(i)>0\}$ can be pruned from the sets $\Y_v$.
%marked as immovable.
Up to now we achieved the following. Suppose that we solve the reduced verification LP with polytope $\Lambda_P$. If there holds $p_v(O_v) = O_v$ for all $v$, then $p\in\BS_f$ by \Theorem{reduced-SI}. In the opposite case, by \Theorem{T:nested++} with $\Lambda'=\Lambda_P$, all strictly relaxed-improving mappings $q<p$ must satisfy $q_v(O_v) = O_v$. Therefore the reduced verification LP is valid to be used in the step~\ref{alg1:test-p} of \Algorithm{alg:iterative-LP}.
% in the step~\ref{alg1:test-\mapp} of \Algorithm{alg:iterative-LP}

==> tex/extra/trws_finate.tex <==
Lastly, we propose a weaker result applicable to a non-reduced version of the verification problem. This result is redundant for the present work, but is not fully obsolete.
\begin{theorem}\label{T:TRW-S-terminates}
Consider the problem $g = (I-[p]\T)f$ with integer costs. Let TRW-S build sequence of reparametrizations $(\varphi_i)_{i=1}^\infty$. After some finite number of steps at least one of the two conditions is satisfied:
\begin{itemize}
\item[(a)] $LB(\varphi_i)>-1/2$;
%\item[(b)] exists $s\in\SV$ and $i \in O_s^{\varepsilon}(g^{\varphi_i})$ such that $p_{s}(i) \neq i$.
\item[(b)] exists $s\in\SV$ and $i \in O_s(g^{\varphi_i})$ such that $p_{s}(i) \neq i$.
\end{itemize}
\end{theorem}
\par
\begin{proof}
Recall the definition of the set of immovable labels $U_s = \{i\in\L_s \mid p_s(i)=i\}$.
\par
Assume for contradiction that %TRW-S builds an infinite sequence of reparametrizations $\varphi_i$, $i=1,\dots$ such that $LB_i<-1/2$ 
for all $i=1,\dots \infty$ holds $LB(\varphi_i)\leq -1/2$ (negation of (a)) and $(\forall s\in\SV)$ $O_s(g^{\varphi_i}) \subset U_s$ (negation of (b)). By properties of TRW-S algorithm~\cite{Kolmogorov-06-convergent-pami} there is a converging subsequence ${\varphi_{i_j}} \rightarrow \varphi$ such that $g^{\varphi}$ satisfies weak tree agreement (WTA). 
%Because $\varepsilon>0$ 
In the limit it must also be $O_s(g^{\varphi}) \subset U_s$. From WTA each tree minimizer takes only the labels in $O_s(g^{\varphi}) \subset U_s$. Since all unary and pairwise costs of $g$ for immovable labels are zero:
\begin{subequations}
\begin{align}
(\forall s\in\SV,\ \forall i\in U_s)\tab & g_{s}(i)=0,\\
(\forall st\in\SE,\ \forall i\in U_s,\ \forall j\in U_t)\tab &g_{st}(i,j)=0,
\end{align}
\end{subequations}
the TRW-S lower bound $LB(\varphi)$ must be zero. Since $LB(\varphi_i) \rightarrow LB(\varphi)$, from the assumption it follows that $LB(\varphi)\leq-1/2$, a contradiction.
\end{proof}

==> tex/extra/trws_potts.tex <==
\myparagraph{Potts model}
We assume $f_{uv}(i,j) = -\gamma_{uv}\leftbb i{=}j\rightbb$. Step 3, for the Potts model simplifies as
\begin{equation}
\varphi_{vu}(j) = 
\begin{cases}
\min\big\{ m_2, a(j)-\gamma_{uv}\big\},& j\in\Y_u,\\
m_2, & j\notin\Y_u,
\end{cases}
\end{equation}
where $m_2 = \min\limits_{i\in \Y_u}a(i)$. So the computation can be implemented in two passes as \Algorithm{Alg:msg-potts}.
\begin{algorithm}
\KwIn{Unary term $a \colon \Y_u \cup\{y_u\} \to \Real$\;}% such that $a(\overline \Y_u) = a(y_u)$\;}
\KwOut{Message $\varphi_{vu} \colon \Y_v \cup\{y_v\} \to \Real$\;}
\For{$i\in \Y_u$}{
	$m_1 := \min\{m_1, a(i)+\Delta_{uv}(i)\}$\;
	$m_2 := \min\{m_2, a(i)\}$\;
}
$m_1 := \min\{m_1,a_u(y_u)\}$\;
$c_1 := m_2-c$\;
$c_2 := -\gamma_{uv}-c$\;
\For{$j\in \Y_v$}{
\eIf{$j\in\Y_u$}{
$\varphi_{vu}(j) := \min\{c_1,a(j)+c_2,\Delta_{vu}(j)+m_1\}$\;
}
{
$\varphi_{vu}(j) := \min\{c_1,\Delta_{vu}(j)+m_1\}$\;
}
}
For $j=y_v$\;
\eIf{$j\in\Y_u$}{
$\varphi_{vu}(j) := \min\{c_1,a(j)+c_2,m_1\}$\;
}
{
$\varphi_{vu}(j) := \min\{c_1,m_1\}$\;
}
\caption{Message Passing for Pruning / Potts\label{Alg:msg-potts}}
\end{algorithm}

Furthermore, for $i \in \Y_u$
\begin{align}
\Delta_{uv}(i) = \min_{j'\in\X_v \backslash \Y_v}[f_{uv}(i,j') - f_{uv}(y_u,j')]\\
= \begin{cases}
%0, & y_u = i \\
-\gamma_{uv}, & i \notin \Y_v\\
\beta_{uv}, & i \in \Y_v,
%0, & \mbox{otherwise}.
\end{cases}
\end{align}
where $\beta_{uv} = \gamma_{uv}\leftbb \X_v\backslash \Y_v = \{y_u\} \rightbb$. Numbers $\Delta$ can be expanded. Then expression
\begin{subequations}
\begin{align}
& \min_{\i\in\Y_u}(a(i)+\Delta_{uv}(i))\\
& = \min\{\min_{\i\in\Y_u \cup \Y_v}a(i)+\beta_{uv},\min_{\i\in\Y_u \cup \overline \Y_v}a(i)-\gamma_{uv}\}\\
& = \min\{v_1+\beta_{uv},v_2-\gamma_{uv}\},
\end{align}
\end{subequations}
where numbers $v_1$ and $v_2$ are defined as the inner minima above. Using these expressions and simplifying further, the computation expresses efficiently as \Algorithm{Alg:msg-potts-2}. So we do not store the precomputed offsets $\Delta$ and can calculate the message directly from sets $\Y_u$, $\Y_v$.
\begin{algorithm}
\KwIn{Unary term $a \colon \Y_u \cup\{y_u\} \to \Real$\;}% such that $a(\overline \Y_u) = a(y_u)$\;}
\KwOut{Message $\varphi_{vu} \colon \Y_v \cup\{y_v\} \to \Real$\;}
%$m_1 := m_2 := m_3 := \infty$\;
$v_1 := v_2 := \infty$\;
\For{$i\in \Y_u$}{
\eIf{$i\in\Y_v$}{
	$v_1 := \min\{v_1, a(i)\}$\;
	}
	{
	$v_2 := \min\{v_2, a(i)\}$\;
	}
}
$m_1 := \min\{v_1+\beta_{uv},v_2-\gamma,a(y_u)\}$\;
$c_1 := \min\{v_1,v_2\}-c$\;
%$c_3 := \min\{\beta+m_1,c_1,a-\gamma_{uv}-c\}$\;
$c_2 := -\gamma_{uv}-c$\;
$c_3 := \min\{\beta_{vu}+m_1,c_1\}$\;
$c_4 := \min\{c_1,-\gamma+m_1\}$\;
%\For{$j\in \Y_v \cup\{y_v\}$}{
%\For{$j\in \Y_v$}{
%\eIf{$j\in\Y_u$}{
%$\varphi_{vu}(j) := c_3$\;
%}
%{
%$\varphi_{vu}(j) := c_4$\;
%}
%}
%Calculate $\varphi_{vu}(y_v)$.
\For{$j\in \Y_v$}{
\eIf{$j\in\Y_u$}{
$\varphi_{vu}(j) := \min\{c_3,a(j)+c_2\}$\;
}
{
$\varphi_{vu}(j) := c_4$\;
}
}
\eIf{$y_v\in\Y_u$}{
$\varphi_{vu}(y_v) := \min\{c_1,a(y_v)+c_2,m_1\}$\;
}
{
$\varphi_{vu}(y_v) := \min\{c_1,m_1\}$\;
}
\caption{Message Passing for Pruning / Potts\label{Alg:msg-potts-2}}
\end{algorithm}

%\par
%Suppose that some pairwise potentials are specially structured, so that messages in message passing algorithms can be computed in linear time in the number of labels instead of quadratic time, see~\cite{FelsenszwalbHuttenlocherEfficientBeliefPropagation}.
%This is the case for many potentials with a linear ordering, e.g. absolute differences, squared distance and truncated versions thereof, which covers Potts-terms.
%\subsection{Message Passing for Potts Model}
%In this case we additionally expand terms $\Delta$ as follows. We assume $f_{uv}(i,j) = -\gamma\leftbb i{=}j\rightbb$. Then
%\begin{align}
%\Delta_{uv}(i) = \min_{j'\in\X_v \backslash \Y_v}[f_{uv}(i,j') - f_{uv}(y_u,j')]\\
%= \begin{cases}
%%0, & y_u = i \\
%-\gamma, & y_u \neq i,\ i \notin \Y_v\\
%\gamma, & y_u \neq i,\ i \in \Y_v,\ \{y_u\} = \overline \Y_v \\
%0, & \mbox{otherwise}.
%\end{cases}
%\end{align}
%
%\begin{align}
%\varphi_{vu}(j) = & \min\limits_{i\in \X_u}\Big[a(i)+\Delta_{uv}(i)\Big]\\
%= & \min\limits_{i\in \X_u}\Big[a(i)+\Delta_{uv}(i)\Big]+\Delta_{vu}(j),
%\end{align}

==> tex/myspace.tex <==
\usepackage{aliascnt}
\newlength{\myskip}
\setlength{\myskip}{\baselineskip}
\def\skipalgomyskip{\vspace{0\myskip}}

\renewcommand{\theenumi}{(\alph{enumi})}
\renewcommand{\labelenumi}{\theenumi}

\newcounter{itemi}	

\renewenvironment{itemize}
  {\begin{list}{$\bullet$}
     {\topsep=0in\itemsep=0pt\parsep=0pt\partopsep=0in\usecounter{itemi}}
   }{\end{list}\addvspace{0pt}}

\raggedbottom
\topsep=0pt 
\partopsep=0pt 
\itemsep=0pt 

\setlength{\tabcolsep}{0pt}
\arraycolsep = 1.2\arraycolsep
\floatsep = 0.5\myskip 
\textfloatsep = 3mm 
\intextsep = 3mm 
\raggedbottom
\abovecaptionskip = 0pt
\belowcaptionskip = 0pt
\itemsep=0pt 
\renewcommand\floatpagefraction{1}
\renewcommand\topfraction{1}
\renewcommand\bottomfraction{1}
\renewcommand\textfraction{0}   
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}

\SetAlgoSkip{skipalgomyskip}
\SetAlgoInsideSkip{}

\makeatletter
\let\corollary\@undefined
\let\c@corollary\@undefined
\let\endcorollary\@undefined
\let\definition\@undefined
\let\c@definition\@undefined
\let\enddefinition\@undefined
\let\theorem\@undefined
\let\c@theorem\@undefined
\let\endtheorem\@undefined
\let\lemma\@undefined
\let\c@lemma\@undefined
\let\endlemma\@undefined
\makeatother

\newtheoremstyle{tightItalic}
  {0.5\myskip}
  {0.5\myskip}
  {}
  {}
  {\itshape}
  {.}
  { }
  {}

\newtheoremstyle{tightBf}
  {0.5\myskip}
  {0.5\myskip}
  {}
  {}
  {\bf}
  {.}
  {.5em}
  {}

\theoremstyle{tightBf}
\newtheorem{theorem}{Theorem}[section]
\providecommand*{\theoremautorefname}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\providecommand*{\corollaryautorefname}{Corollary}
\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\providecommand*{\definitionautorefname}{Definition}
\newaliascnt{statement}{theorem}
\newtheorem{statement}[statement]{Statement}
\aliascntresetthe{statement}
\providecommand*{\statementautorefname}{Statement}
\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\providecommand*{\lemmaautorefname}{Lemma}
\newaliascnt{example}{theorem}
\newtheorem{example}[example]{Example}
\aliascntresetthe{example}
\providecommand*{\exampleautorefname}{Example}
\newaliascnt{remark}{theorem}
\newtheorem*{remark*}{Remark}
\aliascntresetthe{remark}
\providecommand*{\remarkautorefname}{Remark}
\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\providecommand*{\propositionautorefname}{Proposition}
\newaliascnt{property}{theorem}
\newtheorem*{property}{Property}
\aliascntresetthe{property}
\providecommand*{\propertyautorefname}{Property}

\newtheorem*{discussion}{Discussion}

\theoremstyle{tightItalic}

\makeatletter
\setlength{\@fptop}{0pt}
\makeatother


==> tex/old.tex <==
\clearpage
\section{OLD}
\subsection{Intro/Contribution}
 and on the other hand it can be implemented using any existing solvers to solve the standard local polytope relaxation of the MAP-inference problems~\eqref{equ:energyMinimization} as a subroutine

~\cite{SwobodaPersistencyCVPR2014} it is efficient and well-scalable, because it requires only to solve the standard local polytope relaxation of the MAP-inference problems~\eqref{equ:energyMinimization} as a subroutine. Approximate solvers for the relaxed inference problem can be used as well.

We propose an algorithm which possesses advantages of both approaches~\cite{shekhovtsov-14} and~\cite{SwobodaPersistencyCVPR2014} and is free from their drawbacks:
\begin{itemize}
 \item Like~\cite{SwobodaPersistencyCVPR2014} it is efficient and well-scalable, because it requires only to solve the standard local polytope relaxation of the MAP-inference problems~\eqref{equ:energyMinimization} as a subroutine. Approximate solvers for the relaxed inference problem can be used as well.
 \item It has better theoretical guarantees than~\cite{SwobodaPersistencyCVPR2014} and matches the maximum persistency of~\cite{shekhovtsov-14} in the case when an exact LP solver is used.
\end{itemize}
We further propose several speed-up %(\textcolor{red}{use only one term everywhere: speeding up techniques or speed-up techniques}) 
techniques, which are guaranteed {\em not to affect optimality} of the solution and make our method up to several orders of magnitude faster. These techniques are:
 \begin{itemize}
 \item[-] reduction (simplification) of linear programs that need to be solved iteratively.
 \item[-] sufficient conditions to stop an (approximate) inference solver sooner.
 \item[-] computation of fast message passing updates for reduced problems.
\end{itemize}

\par
We demonstrate efficiency of our approach on benchmark problems from machine learning and computer vision. We outperform {\em all} competing methods in terms of the number of persistent labels and method~\cite{shekhovtsov-14} in speed and scalability.
On randomly generated small problems, where an exact method is computationally feasible, the persistency found by our implementation based on an approximate LP solver is close to the maximum one.
\par


\subsection{Outline} \revisit In \Section{sec:preliminaries} we give basic definitions and introduce an alternative formulation of the maximum persistency problem~\cite{shekhovtsov-14}. In \Section{sec:GenerilAlgorithm} we propose a novel generic polynomial algorithm for this problem. 
In \Section{sec:ApproximativeDualAlgorithm} we discuss practical aspects of the method, including its use with approximate solvers for LP relaxations. %for the local polytope relaxation of~\eqref{equ:energyMinimization}. 
In \Section{sec:problemReduction} we introduce the reduction, which enables our final efficient algorithm in~\Section{sec:any-dual} and some of the speed-ups in \Section{sec:speedups}. Experiments and conclusion are found in~\Section{sec:experiments} and \Section{sec:conclusions}.

\par\noindent{\bf Quick Glossary} $\Lambda$ - local polytope. $\BS_{ f}$ -  the set of strict $\Lambda$-improving substitutions for $f$, see~\Definition{def:linearStrictLPImprovingMapping}. $\SP^{2,y}$ - the set of {\em subset-to-one} substitutions, see~\eqref{equ:pixelWiseMapping}. $[p]$ denotes the linear extension of a substitution $p$ as in~\autoref{Pro:P-transpose}.


\myparagraph{Notation}
%{\small
We use the following notation: $\subsetneq$, $\subseteq$ - strict and non-strict set inclusions; $\Real_+$ -  the set of non-negative real numbers; $\Boolean$ - the set of Booleans, identified with $\{0,1\}$; $\leftbb \cdot \rightbb$ is the Iverson bracket, \ie, $\leftbb A \rightbb$ equals $1$ if $A$ is true and $0$ otherwise. LHS and RHS are the left-hand and right-hand sides of an (in)equality.

\subsection{Alg Primal}

The current feasible set of improving substitutions consists of all $q\in \SP^{2,y}$ such that $q \leq p$ where $p\in \SP^{2,y}$ is a substitution maintained by the algorithm and is the current maximum by construction. %is defined by~\eqref{equ:pixelWiseMapping}. Hence $p$ is the maximum of 


We first propose a general algorithm to find the maximum strictly $\Lambda$-improving substitution in $\SP^{2,y}$ that relies on the exact solution of the verification LP~\eqref{equ:linearStrictLPImprovingMapping}. 
It will set the general design and the reference point for the later approximation. \Algorithm{alg:iterative-LP} is a cutting plane method in the discrete space of substitutions. It starts with a feasible set equal to $\SP^{2,y}$. 
In each iteration it computes the maximum substitution $p$ in the current feasible set and verifies whether $p\in\BS_ f$. If it is so, then $p$ is the solution. Otherwise, the feasible set is refined such that it still contains all substitutions in $\BS_ f \cap \SP^{2,y}$ but does not contain the previous maximum $p$.
The algorithm operates with the following reformulation of condition~\eqref{equ:linearStrictLPImprovingMapping}.

the current feasible set.
In line~\ref{alg1:init-p} the verification cost vector $g = (I-[p]\T)f$ is constructed so that $E_g$ quantifies energy improvement $E_g(x) = E_f(x) - E_f(p(x))$ of any labeling~$x$ under substitution~$p$.
In lines~\ref{alg1:test-p}-\ref{alg1:check-condition} the algorithm verifies whether $p$ already belongs to $\BS_f$ by using \autoref{prop:linearStrictLPImprovingMapping} and if not, it {\em prunes} (line~\ref{alg1:update-U}) the sets $\Y_v$ by removing labels corresponding to 
the support set $\O_v^*$ of all optimal solutions of the verification LP. The labels pruned from $\Y_v$ will {\em not} be eliminated. The set $\O^*$ appearing in line 5, which is the facet of all optimal solutions, need not be computed explicitly. 
Given a solution $\mu^*$ in a general configuration, \ie, in the relative interior of the optimal facet, as typically found by interior point methods or algorithms based on smoothing~\cite{Savchynskyy11,AdaptiveDiminishingSmoothing}, support sets $\O_v^*$ can be computed as
\begin{align}
\O_v^* = \{ i\in\X_v \mid \mu^*_v(i) > 0 \},
\end{align}
\ie, if in any optimal solution $\mu$ the component $\mu_u(i)$ is positive then it is so in $\mu^*$, see~\cite{Vanderbei2001}. % (strict complementarity implies that all optimal solution have support in these sets).
%The support sets $\O_v^*$ can be computed from a {\em single} relative interior optimal solution $\mu$, typically found by interior point methods or algorithms based on smoothing~\cite{Savchynskyy11,AdaptiveDiminishingSmoothing}. 





==> tex/tex_defs.tex <==
\newcommand{\myparagraph}[1]{\par\vspace{0.15cm} \noindent \textbf{#1}}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\SG}{{\cal G}}
\newcommand{\SA}{{\cal A}}
\newcommand{\SB}{{\cal B}}
\newcommand{\SE}{{\cal E}}
\newcommand{\SF}{{\cal F}}
\newcommand{\SX}{{\cal X}}
\newcommand{\SCX}{\overline{\cal X}}
\newcommand{\SFX}{\tilde{\cal X}}
\newcommand{\SIsv}{{{\cal I}_{\emptyset}}}
\newcommand{\SY}{{\cal Y}}
\newcommand{\SZ}{{\cal Z}}
\newcommand{\ST}{{\cal T}}
\newcommand{\SH}{{\cal H}}
\newcommand{\SK}{{\cal K}}
\newcommand{\SM}{{\cal M}}
\newcommand{\SC}{{\cal C}}
\newcommand{\SN}{{\cal N}}
\newcommand{\SW}{{\cal W}}
\newcommand{\Ssv}{{\cal S}}
\newcommand{\Ss}{{\cal S}}
\newcommand{\SQ}{{\cal Q}}
\newcommand{\SR}{\Re^n}
\newcommand{\SI}{{\cal I}}
\newcommand{\SO}{{\cal O}}
\newcommand{\SP}{{\cal P}}
\newcommand{\SJ}{{\cal J}}
\newcommand{\SL}{{\cal L}}
\newcommand{\SD}{{\cal D}}
\newcommand{\SV}{{\cal V}}
\newcommand{\V}{{\mathcal V}}
\newcommand{\SU}{{\cal U}}
\newcommand{\BR}{\mathbb R}
\newcommand{\BI}{\mathbb I}
\newcommand{\BS}{\mathbb S}
\newcommand{\BW}{\mathbb W}
\newcommand{\WI}{\mathbb W}

\newcommand{\DA}{{\partial A}}
\newcommand{\DB}{{\partial B}}
\newcommand{\OA}{{\overline A}}
\newcommand{\Nb}{{\rm nb}}

\def\equ#1{(\ref{#1})}
\newcommand{\lan}{\left\langle}
\newcommand{\ran}{\right\rangle}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\T}{^{\mathsf T}}

\newcommand{\X}{{\SX}}
\newcommand{\Y}{{\SY}}
\renewcommand{\O}{{\SO}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Boolean}{\mathbb{B}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\U}{\mathcal{U}}

\newcommand{\lsub}[1]{\limits_{\begin{subarray}{l}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}
\newcommand{\csub}[1]{\limits_{\begin{subarray}{c}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}
\newcommand{\clim}[1]{\limits_{\begin{subarray}{c}\setlength{\arraycolsep}{0.2em}#1\end{subarray}}}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\coni}{coni}
\newcommand{\bone}{1}
\newcommand{\Algorithm}[1]{{Algorithm\,\ref{#1}}}
\newcommand{\Proposition}[1]{{Proposition\,\ref{#1}}}
\newcommand{\tab}{{\hphantom{bla}}}
\def\N{{\bf \rm nb}}

\def\mathrlap{\mathpalette\mathrlapinternal} 
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathllapinternal#1#2{\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{\rlap{$\mathsurround=0pt#1{#2}$}}
\def\leftbb{\mathrlap{[}\hskip1.3pt[}
\def\rightbb{]\hskip1.36pt\mathllap{]}}
\def\bbleft{\leftbb}
\def\bbright{\rightbb}

\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\Argmin}{Arg\,min}
\DeclareMathOperator*{\Argmax}{Arg\,max}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\argmin}{\mathop{\rm argmin}}
\DeclareMathOperator*{\Aff}{Aff}
\def\defeq{\buildrel \text{d{}ef}\over =}	

\newcommand{\Section}[1]{\S\ref{#1}}
\newcommand{\Figure}[1]{\autoref{#1}}
\newcommand{\Theorem}[1]{\autoref{#1}}
\newcommand{\Lemma}[1]{\autoref{#1}}
\newcommand{\Definition}[1]{\autoref{#1}}
\newcommand{\Corollary}[1]{\autoref{#1}}

\let\emptyset\varnothing
\def\revisit{\ensuremath{\red \triangle}\xspace}

\newcommand{\gray}{\color[rgb]{0.5,0.5,0.5}}
\newcommand{\red}{\color[rgb]{1,0,0}}
\newcommand{\cyan}{\color[rgb]{0,0.5,1}}
\newcommand{\blue}{\color[rgb]{0,0.0,1}}
\newcommand{\white}{\color[rgb]{1,1,1}}

\def\subset{\subseteq}
\def\supset{\supseteq}

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\definecolor{Gray}{gray}{0.9}
\newcolumntype{g}{>{\columncolor{Gray}}r}
\newcolumntype{G}{>{\columncolor{Gray}}c}



==> tex/trws_margin.tex <==
\subsection{Properties of TRW-S}\label{sec:TRWS-margin}
{\gray
We give several theoretical guarantees for TRW-S when it is applied to solve the verification problem $(I-[p]\T)f$ or to its reduced version~\eqref{equ:reductionTheorem}.
\par
{TRW-S} algorithm, though observed to always converge in practice to a fixed point, has very weak theoretical convergence guarantees. It is known that there is a convergent subsequence who's limit satisfies Week Tree Agreement (WTA)~\cite{TRWSKolmogorov}. A finite iteration epsilon-variant of this statement exists~\cite{Schlesinger-diffusion} for a related max-sum diffusion algorithm. In either case we have no guarantee to obtain an arc consistent solution required to prove \Proposition{prop:correctnessAlg2}. The major obstacles are: (i) WTA is achieved only in the limit and (ii) there is no guarantee that the set of labels which are in WTA (let alone its arc consistent subset) converges as well.
\par
Fortunately, TRW-S enjoys properties very useful for us especially when it is applied to the reduced verification problem. 
}
\myparagraph{A Convergence Measure for Verification LP} \revisit
Let us introduce a measure of how ``far'' the dual solver is from a fixed integer solution $y$. For a node $u$ we define the {\em node margin} of $u$  as the value 
\begin{equation}
m_u(\varphi) = \min_{i\in\X_u}(f^{\varphi}_{u}(i)-f^{\varphi}_{u}(y_u)).
\end{equation}
The margin is related to the set $\O_u(\varphi)$ of local minimizers. If it is negative, $\O_u(\varphi)$ does not contain $y_u$ and the negative value measures how well it is separated. We define the {\em problem margin} as the value
\begin{equation}
m(\varphi) = \min_{u\in\SV} m_u(\varphi).
\end{equation}
For the verification problem $g = (I-[p]\T)f$, if the problem margin is negative then there exists $u\in\V$ such that $\O_u(\varphi) \cap \Y_u \neq \emptyset$ and therefore set $\Y_u$ will strictly shrink in the pruning \autoref{trws-mark-step} if the later is executed.
The following theorem asserts that in TRW-S the margin is always negative unless it has converged to a point satisfying complementarity with $\delta(y)$ and hence fond the optimal solution. 
\begin{theorem}[Margin for TRW-S]\label{T:margin} 
Let $\bar g$ be the reduced verification problem, $\varphi$ a dual point after one or more iterations of TRW-S and $LB_{\rm T}(\varphi)$ the lower bound of TRW-S. Then
\begin{equation}
LB_{\rm T}(\varphi) = 0 \ \ \mbox{iff}\ \ m_u(\varphi) \geq 0.
\end{equation}
\end{theorem}
For the purpose of the proof we need to give a short specification of TRW-S. Previously, we assumed that $(\V,\E)$ is a directed graph but the orientation of edges was not essential. Let us assume that $(\V,\E)$ is a directed acyclic graph.
With this assumption the dependency in TRW-S updates can be fully specified by the orientation of edges in $\SE$: for $uv\in\E$ the update for $u$ must be computed before the update of $v$. For a serial implementation, this partial order can be completed to a total order on $\SV$ satisfying $u<v$ if $uv\in \SE$. We specify only the forward pass of TRW-S as \autoref{Alg:trws} (\cf \cite[Fig.~3]{TRWSKolmogorov}) and note that the backward pass is obtained by reversing all edges. 
\begin{procedure}
\KwIn{Problem $f\in\Real^\SI$, reparametrization $\varphi$\;}
\KwOut{Updated reparametrization $\varphi$, $LB_T$, best labeling $x$, locally optimal labels $\O_u(\varphi)$\;}
\For{$u\in\SV$}{
\For{$v \mid uv\in\SE$}{
$\varphi_{vu}(j) := \min\limits_{i}\Big[ \frac{1}{n_u} f^{\varphi}_{u}(i)-\varphi_{uv}(i) +f_{uv}(i,j) \Big]$\;
}
}
$\O_u(\varphi) := \argmin_{i} f^{\varphi}_u(i)$; $x_u \in \O_u(\varphi)$\;
$LB_{\rm T}(\varphi) := \sum_{u\in\SV} \frac{n_{\rm term}(u)}{n_u} \min\limits_{i} f^{\varphi}_u(i)$\;
\caption{TRW-S Forward Pass($f$,$\varphi$)\label{Alg:trws}}
\end{procedure}
In \autoref{Alg:trws}, $n_u$ is the number of chains that meet in node $u$ and $n_{\rm term}(u)$ is the number of chains that terminate in $u$.

\par
Viewed as computing the division of costs between the chains, TRW-S has the following properties. To a chain $\tau$ there is associated its oriented graph $(\V^\tau, \SE^\tau)$ and its share of the unary terms in the decomposition, $f^{\tau}$. 
We assume thet each pairwise term $f_{uv}$ is associated to exactly one chain passing through edge $uv$.
\par
After the first backward pass, the algorithm maintains the following invariants. Consider the step of processing vertex $u^* \in \SV$. For a chain $\tau$ which passes through edge $uv\in\SE$ there holds:
\newline\noindent$\bullet$
If $u^* < u$, message $\varphi_{uv}(i)$ is equal to the {\em right} min-marginals of the chain:
\begin{equation}
\varphi_{uv}(i) = \min\lsub{(x_{w}\mid w > v)\\ x_u = i}(\sum\lsub{u\in\SV^{\tau} \\ w > u}f^{\tau}_{w}(x_w) + \sum\lsub{u'v' \in \SE^{\tau} \\ u' \leq u} f_{u'v'}(x_{u'},x_{v'})).
\end{equation}
\newline\noindent$\bullet$ If $u^* > u$, message $\varphi_{vu}(j)$ is equal to the {\em left} min-marginals of the chain:
\begin{equation}
\varphi_{vu}(j) = \min\lsub{(x_{w}\mid w <v)\\ x_v = j}(\sum\lsub{w \in\SV^{\tau} \\ w < v}f^{\tau}_{w}(x_w) + \sum\lsub{u'v' \in \SE^{\tau} \\ u' \leq u} f_{u'v'}(x_{u'},x_{v'})).
\end{equation}
\par
Weak tree agreement is the condition when the lower bound cannot be improved further by TRW-S~\cite{TRWSKolmogorov}. It requires that among all optimal assignments of the chains there is a consistent subset. \revisit Connection to AC
\par

\begin{proof}[Proof of \Theorem{T:margin}]
For the convenience of analysis, we continue to denote the cost vector to which \autoref{Alg:trws} is applied as $f$. In the context of \Algorithm{Alg:iterative-AC}, we temporarily let $f:=\bar g$. 
\par
($\Rightarrow$) Let $LB_T(\varphi) = 0$. By construction, $E_{f}(y) = 0$ so the duality gap is zero and therefore $\varphi$ is dual optimal and $\delta(y)$ is primal optimal. By complementary slackness it must be that $(\forall u\in\SV)\ f^\varphi_u(y_u)$ is locally minimal. Therefore problem margin is exactly zero. This part of the proof holds also for non-reduced verification problem and any reparametrization such that $LB_T(\varphi) = 0$.
\par
($\Leftarrow$) Let now the problem margin be non-negative. Let us consider edge $uv\in\SE$ and let $f^{\tau}$ be the cost vector of the monotonic chain $\tau$ passing through edge $uv$ at the beginning of iteration processing node $v$. Since $u$ was already processed, the value $f^{\varphi}_u$ is proportional to min-marginals of chain $\tau$ in $u$ and we have $m_u(\varphi) \geq 0$. It follows that there is a minimizer $x \in \min_{x} \< f^{\tau}, \delta(x)\>$ such that $x_u = y_u$. For this minimizer there holds 
\begin{equation}\label{partial-y}
x \in \argmin_{\tilde x \mid \tilde x_v = x_v} \< f^{\tau}, \delta(\tilde x)\>.
\end{equation}
This is because we constrained $\tilde x$ to coincide with the global chain minimizer in $v$. This conditional minimizer however clearly does not depend on $f_{v}^{\tau}$, the unary term associated to chain $\tau$.
\par
Consider the operation of averaging min-marginals over node $v$. By assumption, after averaging operation, $m_v \geq 0$ and therefore the local minimum over each chain is attained in $y_v$. The averaging operation only changes the value $f^{\tau}_v$. 
The conditional minimizer 
\begin{equation}\label{partial-x}
x' \in \argmin_{\tilde x \mid \tilde x_v = y_v} \< f^{\tau}, \delta(\tilde x)\>
\end{equation}
does not depend on $f^{\tau}_v$.
\par
Let $r$ precede $u$ in $\tau$. Assume for contradiction that $x'_u \neq y_u$. Because $u$ has been processed, the value $\varphi_{ur}(i)$ is the left-min-marginal for chain $\tau$ in node $u$ and label $i\in\X_u$.
Denote $\overrightarrow{f^{\tau}_u} = \varphi_{ur}(i) + f_u^{\tau}(i)$. 
The relations~\eqref{partial-y} and \eqref{partial-x} can be expressed as
\begin{subequations}
\begin{align}
\label{trws-ch-1}
y_u \in \argmin_{i}\big( \overrightarrow{f^{\tau}_u} + f_{uv}(i,x_v) \big); \\
\label{trws-ch-2}
x'_u \in \argmin_{i}\big( \overrightarrow{f^{\tau}_u} + f_{uv}(i,y_v) \big).
\end{align}
\end{subequations}
From~\eqref{trws-ch-1} we have that $\overrightarrow{f^{\tau}_u}(y_u)+f_{uv}(y_u,x_v) \leq \overrightarrow{f^{\tau}_u}(x'_u) + f_{uv}(x'_u,x_v)$.
We use now the partial submodularity fulfilled for $f$,
\begin{equation}
f_{uv}(y_u,x_v) + f_{uv}(x'_u,y_v) \geq f_{uv}(x'_u,x_v)
\end{equation}
and obtain that
\begin{equation}
\overrightarrow{f^{\tau}_u}(y_u) \leq \overrightarrow{f^{\tau}_u}(x'_u) + f_{uv}(x'_u,y_v).
\end{equation}
Adding on the LHS the term $f_{uv}(y_u,y_v) = 0$, we get
\begin{equation}
\overrightarrow{f^{\tau}_u}(y_u)+f_{uv}(y_u,y_v) \leq \overrightarrow{f^{\tau}_u}(x'_u) + f_{uv}(x'_u,y_v).
\end{equation}
This inequality allows to conclude that $y_u$ is a also a minimizer to~\eqref{trws-ch-2}. Therefore either $x'_u = y_u$ or $y_u$ is an equally good substitute.
\par
We have shown that as soon as there is zero margin, for each chain the part of the minimizer over already processed nodes can be selected equal to $y$. By induction, at the end of the sweep, $y$ is a minimizer for each chain. Hence WTA is achieved. In this case, there is zero integrality gap and $LB_T=E_f(y)=0$.
\par
The termination condition in \autoref{trws-return-step} indicates that $y$ is an optimal primal solution and in this case it must be that $LB = 0$, therefore current $\varphi$ is an optimal dual point. In this case $\O_u^* \subset \O_u$, where set $\O_u^*$ is the support set of all primal optimal solutions (see \Algorithm{alg:iterative-LP}). We therefore have $\O_u^* \subset \O_u \subset \X_u \backslash \Y_u$ for all $u$. It follows that stopping condition of generic \Algorithm{alg:iterative-LP} is satisfied as well and hence $p\in\BS_f$.
\end{proof}
It follows that on {\em every} iteration (but the first initializing one) of TRW-S either the problem margin is negative and therefore $(\exists u)\ \O_u(\varphi) \cap \Y_u \neq \emptyset$ (there is always something to prune) or WTA is achieved and the algorithm terminates with $y$ being optimal integer solution. 

